The interplay between AGN feedback and precipitation of the intracluster medium in simulations of galaxy groups and clusters

Using high-resolution hydrodynamical simulations of galaxy clusters, we study the interaction between the brightest cluster galaxy, its supermassive black hole (BH) and the intracluster medium (ICM). We create initial conditions for which the ICM is in hydrostatic equilibrium within the gravitational potential from the galaxy and an NFW dark matter halo. Two free parameters associated with the thermodynamic profiles determine the cluster gas fraction and the central temperature, where the latter can be used to create cool-core or non-cool-core systems. Our simulations include radiative cooling, star formation, BH accretion, and stellar and active galactic nucleus (AGN) feedback. Even though the energy of AGN feedback is injected thermally and isotropically, it leads to anisotropic outflows and buoyantly rising bubbles. We find that the BH accretion rate (BHAR) is highly variable and only correlates strongly with the star formation rate (SFR) and the ICM when it is averaged over more than $1~\rm Myr$. We generally find good agreement with the theoretical precipitation framework. In $10^{13}~\rm M_\odot$ haloes, AGN feedback quenches the central galaxy and converts cool-core systems into non-cool-core systems. In contrast, higher-mass, cool-core clusters evolve cyclically. Episodes of high BHAR raise the entropy of the ICM out to the radius where the ratio of the cooling time and the local dynamical time $t_{\rm cool}/t_{\rm dyn} > 10$, thus suppressing condensation and, after a delay, the BHAR. The corresponding reduction in AGN feedback allows the ICM to cool and become unstable to precipitation, thus initiating a new episode of high SFR and BHAR.

==> Paper idealised elliptical/IC.tex <==
\defcitealias{navarro1997}{NFW}

Our simulation set-up consists of a \citet{navarro1997} dark matter halo (hereafter \citetalias{navarro1997}), a central elliptical galaxy with a \citet{hernquist1990} stellar profile, a single BH at the centre, and a gaseous halo in hydrostatic equilibrium as described below, that is simulated using smoothed-particle hydrodynamics (SPH). We limit our study to halo masses of $M_{200}=10^{13}~\rm M_\odot$, $10^{13.5}~\rm M_\odot$ and $10^{14}~\rm M_\odot$, spanning the range from groups to low-mass clusters, which offers the best compromise between computational feasibility and available observations \citep[see][for a review]{oppenheimer2021}. We achieve a very high resolution ($10^5~\rm M_\odot$ in mass for the gas and stars, $300~\rm pc$ for the gravitational softening) in the central 100 kpc of our simulation. This is comparable to the studies of \citet{qiu2019} or \citet{meece2017}, and at least an order of magnitude higher than in \citet{li2015}, \citet{gaspari2014}, and in state-of-the-art cosmological galaxy formation simulations like EAGLE \citep{schaye2015} and TNG100 \citep{weinberger2017,pillepich2018}. Recently the TNG50 \citep{nelson2019, pillepich2019} and RomulusC \citep{tremmel2019} simulations have modelled comparable massive haloes at similar resolution but as discussed above, our idealised set-up allows a cleaner and more straightforward interpretation of the simulation results.


\subsection{Dark matter halo}
For the collisionless dark matter and stars we follow closely the approach of \citet{hernquist1993} and \citet{springel1999}. To limit computational expense, the dark matter halo is represented by a static external potential corresponding to an \citetalias{navarro1997} profile,
\begin{equation}
    \Phi_{\rm DM}(r) = - \frac{4\pi G \rho_0 R_{\rm 200}^3}{c^3 r} \ln \left( 1 + \frac{c r}{R_{\rm 200}} \right).
\end{equation}
where $G$ is the gravitational constant and $r$ the cluster-centric radius. The characteristic density $\rho_0$ depends on the radius $R_{200}$, its enclosed mass $M_{200}$, and its concentration $c$ as $\rho_0 = M_{200} \,c^3/4 \pi R_{200}^3 \left[ \ln(1+c) - \frac{c}{1+c} \right]$. For each halo mass the concentration-mass relation of \citet{correa2015} is used to calculate $c$ with the \citet{planck2016} cosmology.

\subsection{Stars}
To generate the stars, we use a modified version of \texttt{MakeNewDisk} \citep[][]{springel2005}. The stellar component of our elliptical galaxy is modelled as a radially symmetric sphere corresponding to a \citet{hernquist1990} density profile,
%\begin{align}
%    \Phi_{\star} (r) &= - \frac{G M_\star}{r+r_\star}.
%\end{align}
\begin{align}
    \rho_{\star} &= \frac{M_\star}{2 \pi} \frac{r_\star}{r(r_\star + r)^3}.
\end{align}
This distribution has two free parameters, the total stellar mass $M_\star$ and scale length $r_\star$, where the latter is set by hand to a specific value depending on the halo mass (see Table \ref{tbl:extra_params}). We do not include any satellite galaxies in our simulations.


While it is straightforward to sample the positions of star particles\footnote{This can be done analytically and requires no artificial truncation, 90 (95) per cent of the mass is within $18 r_\star$ ($38 r_\star$).}, assigning particle velocities such that the system is in dynamical equilibrium requires more care. Following the approach of \citet{hernquist1993} and \citet{springel1999}, we assume that at a specific position the velocity distribution corresponds to the solution of the collisionless Boltzmann equation, and can be approximated sufficiently accurately by a multivariate Gaussian. We can then obtain the moments by using the generalized Jeans equations derived by \citet{magorrian1994} for an axisymmetric system (since we include angular momentum in the gas, see below). These equations constrain the velocity structure such that most first and second moments of the multivariate Gaussian are equal to zero. The only non-zero components are $\langle v_{\rm z}^2 \rangle$, $\langle v_{\rm R}^2 \rangle$, $\langle v_\phi^2 \rangle$ and $\langle v_\phi \rangle$:
\begin{align}
 \langle v_{\rm z}^2 \rangle = \langle v_{\rm R}^2 \rangle = \frac{1}{\rho} \int\limits_z^\infty \rho_\star (z', R) \frac{\partial \Phi_{\rm{total}}}{\partial z'} \mathrm{d} z', \label{eq:vz2}
\end{align}
where $\rho_\star$ is the stellar density, $R$ the radius perpendicular to the $z$-axis and $\Phi_{\rm{total}}$ the total gravitational potential of the system;
\begin{align}
 \langle v_{\rm \phi}^2 \rangle = \langle v_{\rm R}^2 \rangle + \frac{R}{\rho} \frac{\partial (\rho \langle v_{\rm R}^2 \rangle )}{\partial R} + v_{\rm c}^2, \label{eq:vphi}
\end{align}
where $v_{\rm c}^2 = R \partial \Phi_{\rm total}/\partial R$ and $\langle v_\phi \rangle$ is the mean angular streaming component, which can be freely chosen in principle but is set to zero in our models such that the galaxy has no net rotation. Each stellar particle is assigned an initial metallicity of $Z_\star = 1/3 ~Z_\odot$ (where $Z_\odot=0.0134$, \citealt{asplund2009}), a stellar mass of $m_\star=10^5~\rm M_\odot$, and a stellar age of $9 ~\rm Gyr$.

\subsection{Intracluster gas}
After constructing the stellar and dark matter components, the next step is determining the structure of the gas component. We assume that the gas is initially in hydrostatic equilibrium,
\begin{align}
    \frac{{\rm d} P}{{\rm d} r} &= - \frac{G M_{\rm encl}(r) \rho(r)}{r^2}. \label{eq:he}
\end{align}
For simplicity, we neglect the contribution of the gas to the gravitational potential given its subdominant density \citep[e.g.][]{schaller2015}, i.e. $M_{\rm encl}(r)=M_{\rm DM, \rm encl} (r) + M_{\star, \rm encl} (r)$. It is convenient to rewrite equation (\ref{eq:he}) in terms of the circular velocity $v_{\rm c}$ and sound speed $c_{\rm s}$ \citep[e.g.][]{stern2019}:
\begin{equation}
    \frac{{\rm d} \ln P}{\mathrm{d} \ln r} = - \gamma \frac{v_{\rm c}^2}{c_{\rm s}^2}, \label{eq:hydrostatic}
\end{equation}
where $\gamma=5/3$ is the adiabatic index of the gas. Under the assumption of constant $v_{\rm c}/c_{\rm s}$ this corresponds to
\begin{align}
    P = P_{0} \left(\frac{r}{r_{0}}\right)^{-\gamma}, \label{eq:pressure-large-radii}
\end{align}
where $P_{0}$ is a free normalisation pressure at radius $r_{0}$. Gravitationally bound solutions have $v_{\rm c} \sim c_{\rm s}$ \citep[e.g.][]{stern2019}. Assuming that $v_{\rm c}=c_{\rm s}$, the definitions of $v_{\rm c}$ and $c_{\rm s}$ yield a temperature profile 
\begin{align}
   T_{\rm circ} &= \frac{\mu m_{\rm p}}{k_{\rm B} \gamma}  \frac{G M_{\rm encl} (r)}{r}, \label{eq:temp-rotation}
\end{align}
where $m_{\rm p}$ is the proton mass, $k_{\rm B}$ is the Boltzmann constant and $\mu=0.6$ is the mean particle mass for fully ionized gas with a metallicity of $Z=1/3 Z_\odot$. However, the assumption that $v_{\rm c} =c_{\rm s}$ breaks down in the centre of most galaxies because the gas is heated by feedback. To make our initial gas component more realistic, we therefore impose a temperature floor near the halo centre with the gas temperature given by
\begin{align}
    T_{\rm total} &= T_{\rm circ} + \frac{T_{\rm 0}}{1 + \exp\left(\frac{r-2 r_{\rm 0}}{r_{\rm 0}}\right)},
\end{align}
with two free parameters $T_0$ and $r_0$ (see below). We choose this functional form as it asymptotes smoothly to $T_{\rm circ}$ at large radii and to a constant value of $T_{\rm min} \approx 0.9 T_{\rm 0}$ at $r \ll r_0$. With this modified temperature profile, it is no longer possible to solve equation (\ref{eq:hydrostatic}) analytically but we solve it numerically, and as expected the solution approaches equation (\ref{eq:pressure-large-radii}) at large radii. Our gaseous halo extends out to $3 R_{200}$. 



\begin{comment}
it is clear that equation (\ref{eq:hydrostatic}) implies that the normalisation of the pressure and therefore also the gas density are free to choose. The assumption that $v_{\rm c}= c_{\rm s}$, means that the temperature profile is given by:
\begin{align}
   T_{\rm circ} &= \frac{\mu m_{\rm p}}{k_{\rm B} \gamma}  \frac{G M_{\rm encl} (r)}{r}, \label{eq:temp-rotation}
\end{align}
where $m_{\rm p}$ is the proton mass, $k_{\rm B}$ is the Boltzmann constant and $\mu$ is the mean particle mass, which we set to the value for fully ionized gas ($\mu = 0.6$). This means that the temperature profile of the ICM is directly determined by the density distribution of the dark matter and stars. Using equation (\ref{eq:temp-rotation}) it is straightforward to calculate the solution of equation (\ref{eq:hydrostatic}):
\begin{equation}
    P = P_0 \left(\frac{r}{r_0}\right)^{-\gamma}, \label{eq:pressure-large-radii}
\end{equation}
where $P_0$ is the pressure at a radius $r_0$, which is determined by a specified boundary condition. However, the assumption that $v_{\rm c} =c_{\rm s}$ is unrealistic in the centre of most galaxies. To have a more realistic temperature and density profile we impose a minimum temperature in the centre of the cluster. This temperature is than added to the temperature based on the circular velocity:
\begin{align}
    T_{\rm total} &= T_{\rm circ} + T_{\rm additional},
\end{align}
with:
\begin{equation}
 T_{\rm additional} = \frac{T_{\rm 0}}{1 + \exp\left(\frac{r-2 \cdot r_{\rm 0}}{r_{\rm 0}}\right)}.
\end{equation}
The respective values for  $T_0$ and $r_\text{0}$ are free parameters and depend on the halo mass. we set $r_\text{0}$ to 10\% of the virial radius. We chose this functional form as it is maximal in the centre and the contribution decays continuously and asymptotes to 0. At small radii this function imposes a minimum temperature given by $T_{\rm additional} \approx 0.9 T_{\rm min}$.

Given that the pressure and temperature profile are then fully determined, it is possible to calculate the density profile using equations (\ref{eq:temp-rotation}) and (\ref{eq:pressure-large-radii}):
\begin{align}
    \rho(r) &= \frac{\gamma r_0 P_0}{G M_{\rm encl}(r)} \left( \frac{r}{r_0} \right)^{1-\gamma}. 
\end{align}
As our boundary condition we use the gas fraction at $R_{500}$ (i.e. the radius at which the average density is 500 times $\rho_{\rm crit}$), $M_{\rm gas}(R_{500}) = f_{\rm gas, 500} M_{500}$, which allows us to solve for $P_0$:
%In order to constrain the density we impose a fixed gas fraction at $R_{500}$, $M_0 = f_{\rm gas, 500} M_{500}$, which allows us to constrain the pressure to:
%\begin{align}
%    P_0 &= \frac{280}{3} f_{\rm gas, 500} \frac{G M_{500}}{r_{500}} \rho_{\rm crit}.
%\end{align}
\begin{align}
    P_0 &= \frac{500}{3} f_{\rm gas, 500} \frac{G M_{500}}{\gamma r_{500}} \rho_{\rm crit} I_1,
\end{align}
where $I_1$ is an integral of order unity given by:
\begin{align}
    I_1^{-1} &= \int \limits_0^{R_{500}} \frac{M_{500}}{M_{\rm encl}(r)} \left( \frac{r}{R_{500}} \right)^{3-\gamma} {\rm d} \left( \frac{r}{R_{500}} \right).
\end{align}
It is therefore possible to constrain the gas profile by either using gas fraction from observations or by matching the enclosed mass at $R_{500}$ for matched haloes from cosmological hydrodynamical simulations. We choose to set the gas fractions to haloes with the same mass taken from the BAHAMAS simulation \citep{mccarthy2017}, which were calibrated to reproduce observed stellar masses and cluster gas fractions.

\end{comment}

The gas distribution in our initial conditions depends on a free parameter $T_0$ which specifies the temperature plateau near the halo centre and can be used to create a CC or NCC system. We calibrate  its value by comparing our initial gas profile against the BAHAMAS simulation \citep{mccarthy2017}, a self-consistent cosmological hydrodynamical simulation at much lower resolution ($m_{\rm gas} \approx 10^9~\rm M_\odot$), as described in \S \ref{sec:BAHAMAS}. As shown by \citet{mccarthy2017}, BAHAMAS matches the radial density and pressure profiles of observed galaxy clusters very well and therefore provides an ideal reference for our idealised simulations. To set the normalisation of our gas density profile, we find the median gas fraction $f_{500} = M_{\rm gas}/M_{500}$ at $z=0$ and adjust $P_{0}$ to match $f_{500}$. 

To set the initial (bulk) velocity of the ICM, we make the simplifying assumption that the angular momentum of the gas traces that of the dark matter halo, with the rotation vector aligned with the $z$-axis. We use the DM angular momentum distribution and radial dependence within $R_{200}$ from \citet{bullock2001}, but with a slightly different spin parameter of the gas ($\lambda = 0.05$) based on \citet{oppenheimer2018}. As we did for stars, we assign each gas particle an initial metallicity of $1/3~{\rm Z_\odot}$ \citep[e.g.][]{werner2013, mcdonald2016}.


\begin{comment}
\subsection{Angular momentum distribution of the gas}
For the angular momentum distribution in the galaxy we follow \citet{bullock2001}.
According to \citet{bullock2001} the normalisation of the angular momentum at the virial
radius is given by:
\begin{equation}
    j_0 = \sqrt{2} V_{200} R_{200} \frac{\lambda}{- \mu \ln(1 - 1/\mu) - 1 },
\end{equation}
in which $\lambda$ is the spin parameter, $\mu$ is a property of the angular 
momentum profile which is on average $\mu = 1.25$. Using this we assume that 
the specific angular momentum is lower closer to the centre because otherwise
we do get velocities that increase by $1/r$ when we get closer to the centre:
\begin{equation}
    M(r) = M_{200} \mu \frac{j(r)}{j_0 + j(r)}.
\end{equation}
Rewriting to find $j(r)$:
\begin{equation}
    j(r) = j_0 \frac{M(<r)}{M_{200}} \frac{1}{ \mu - M(<r)/M_{200}}.
\end{equation}
This then gives us the specific angular momentum inside $R_{200}$, because \citet{bullock2001} does not go farther than $R_{200}$. For radii larger than $R_{200}$,
we assume that the specific angular momentum remains constant, implying the 
velocity will decrease as $1/r$.

Now that we know the angular momentum for each particle it is possible to 
calculate the velocity as ($j = v \cdot r$):
\begin{equation}
    v = \frac{j}{\sqrt{x^2+y^2}}.
\end{equation}
We give each particle their corresponding velocity in the x-y plane. For the exact value of the spin parameter $\lambda$, we follow \citet{oppenheimer2018} and set $\lambda=0.05$.
\end{comment}

\subsubsection{Radially degrading mass resolution} \label{subsubsec:degrading}
Most of the gas mass is at $r \gg 100~\rm kpc$ and is therefore not directly involved in the interplay between gas cooling and feedback. However, our model becomes increasingly unrealistic at these large radii due to the absence of cosmological accretion and satellites. To minimize the computational expense, we therefore only sample the gas at our target resolution ($m_{\rm gas}=m_\star=10^5~\rm M_\odot$ for our fiducial resolution) within $r_{\rm highres} =100~\rm kpc$. At larger radii, the gas particle mass increases as $m_\star ( r/r_{\rm highres} )^2$, reaching $9 \times 10^5~\rm M_\odot$ at $r=300~\rm kpc$ and $4.2 \times 10^6~\rm M_\odot$ at $r=650~\rm kpc$ (corresponding to $R_{500}$ for our most massive halo). This approach is similar to what has been done on smaller scales \citep[e.g.][]{vdvoort2019}. We have verified that using this gradually degrading resolution does not influence the evolution within $r_{\rm highres}$, by running a set of non-radiative simulations with different resolution profiles. Low-resolution particles do not enter the inner $\approx90~\rm kpc$ for the entire duration of our simulations. 

\subsection{The central supermassive black hole}
A single BH is placed in the centre of the galaxy, with a mass given by the BH mass-stellar mass relation from \citet{mcconnell2013}. To avoid an unrealistically high accretion and feedback at the very start of the simulation, we reduce its ambient gas density by removing any gas particles within $1~\rm kpc$\footnote{This corresponds to less than $10^{-4}$ of the gas within $R_{500}$.} of the BH but still keep the total gas mass within $R_{500}$ fixed by placing the removed gas particles randomly between $1~\rm kpc$ and $R_{500}$. 


\begin{figure*}
	\includegraphics[width=.97\linewidth]{./images/density_entropy_temperature_runs_best.pdf}
    \caption{Comparison of the initial median mass-weighted thermodynamic radial profiles to the results from the BAHAMAS cosmological simulation at $z=0$. Different columns correspond to different halo masses (from left to right: $M_{200}/\rm M_\odot = 10^{13}$, $10^{13.5}$ and $10^{14}$). Row (a) shows the density for all gas, row (b) the temperature of hot gas ($T>10^{5.5}~\rm K$), row (c) shows the entropy of the hot gas ($T>10^{5.5}~\rm K$), row (d) the radiative cooling time, row (e) the ratio $t_{\rm cool}/t_{\rm dyn}$, and row (f) the entropy slope as continuous lines and $(t_{\rm dyn}/t_{\rm cool})^2$ as the dashed lines, the point at which the solid and dashed lines intersect is marked by a dot and the corresponding triangle indicates the radius at which this happens. In each column, different colours correspond to different central temperatures. The black dashed line and grey area indicate the mass-weighted median and 1$\sigma$ spread in the BAHAMAS simulation for haloes with the same mass. The vertical grey line indicates $r=100~\rm kpc$. The green points with error bars in the right column show the observations of \citet{sun2009} and the vertical dotted and dash-dotted lines show 1, 3 and 6 times the gravitational softening of the BAHAMAS simulation ($5.7 ~\rm kpc, 17~\rm kpc$ and $34~\rm kpc$). In row (d) the black dashed line indicates the Hubble time ($t_{\rm H}$) and in row (e) the black dashed line shows the value of $t_{\rm cool}/t_{\rm dyn}=10$.}
    \label{fig:BAHAMAS-comparison}
\end{figure*}

\subsection{Calibration against the BAHAMAS simulations}
\label{sec:BAHAMAS}

We use the BAHAMAS simulation to calibrate the two free parameters of our model. For each halo mass the total amount of gas is set by the BAHAMAS gas fraction within $R_{500}$, $f_{500}$ for each halo (see Table \ref{tbl:extra_params}). Determining $T_0$ is less straightforward since it predominantly affects the centre of the halo where the resolution of BAHAMAS becomes a limiting factor. We therefore generated a range of haloes with different values of $T_0$ for each $M_{200}$ and compare these to BAHAMAS in Fig.~\ref{fig:BAHAMAS-comparison}. Specifically, we compare the radial density, temperature, and entropy profiles, where the entropy is defined as $K\equiv k_{\rm B} T / n_{\rm e}^{2/3}$. For clarity, we normalised the temperature and entropy profiles to their analytic virial values within $R_{500}$, namely $T_{500} = GM_{500} \mu m_{\rm p}/2 k_{\rm B} r_{500}$ and $K_{500} = k_{\rm B} T_{500}/[ 500 f_{\rm b} (\rho_{\rm crit}/\mu_{\rm e} m_{\rm p} ) ]^{2/3}$, where $\mu_{\rm e}=1.14$ is the mean atomic weight per free electron and $f_{\rm b}$ the cosmic baryon fraction. To reduce the dynamic range in Fig.~\ref{fig:BAHAMAS-comparison}, the density profile is normalised to $\rho_{\rm crit}$ and multiplied by $(r/R_{500})^2$. The three columns of Fig.~\ref{fig:BAHAMAS-comparison} show the normalised profiles for haloes with $M_{200}=10^{13}$, $10^{13.5}$ and $10^{14}~\rm M_\odot$ respectively, as solid lines coloured according to $T_0$. Black dashed lines show the corresponding mass-weighted median stacked profiles of BAHAMAS haloes with mass within $\Delta \log_{10} M_{500} = 0.01$ at $z=0$, with the 16th and 84th percentiles of the gas particle distribution represented by grey bands. For both the entropy and temperature profiles we only select gas that has a temperature of $T>10^{5.5}~\rm K$ in order to crudely mimic the X-ray observations that were used to calibrate BAHAMAS. For the density profile we select all gas because we want to compare the BAHAMAS total gas density profile\footnote{This means that the profile includes the contribution from satellite galaxies.} with the density profile from the idealised set-up.

Because the density profiles are normalised to $f_{500}$ for BAHAMAS the normalisation agrees for different values of $T_0$, but the shape is different. The temperature and entropy agree with BAHAMAS in the inner region. At large radii there is however a disagreement between the idealised profiles and BAHAMAS, most clearly in the temperature and entropy profiles for higher halo masses. This disagreement is probably because the idealised profiles do not take the cosmological environment into account, namely that gas is accreted and/or a significant amount of gas is in satellite galaxies.  

Keeping these discrepancies in mind, for the $10^{13}~\rm M_\odot$ haloes $T_{0}=0~\rm K$ matches the BAHAMAS profiles most closely. For $M_{200}=10^{13.5}~\rm M_\odot$, $T_{\rm 0} = 10^{6.5}~\rm K$ is the best model. Although $T_{\rm 0} = 10^{6.75}~\rm K$ matches the entropy profile better, it underpredicts the central density by up to a factor 3. For the $10^{14}~\rm M_\odot$ halo the optimal value of $T_{\rm 0}$ is $10^7~\rm K$. It also matches with the observations of \citet{sun2009}. $T_{\rm 0} = 10^{7.25}~\rm K$ matches the entropy better, but has a large cooling time ($t_{\rm cool}>1~\rm Gyr$) making it less ideal to study the BH/ICM connection (see below).

The initial conditions presented in this section are made publicly available as examples distributed with the \texttt{SWIFT} code\footnote{\texttt{swift} is available at \url{http://www.swiftsim.com}.}.  


==> Paper idealised elliptical/abstract.tex <==
\noindent Using high-resolution hydrodynamical simulations of galaxy clusters, we study the interaction between the brightest cluster galaxy, its supermassive black hole (BH) and the intracluster medium (ICM). We create initial conditions for which the ICM is in hydrostatic equilibrium within the gravitational potential from the galaxy and an NFW dark matter halo. Two free parameters associated with the thermodynamic profiles determine the cluster gas fraction and the central temperature, where the latter can be used to create cool-core or non-cool-core systems. Our simulations include radiative cooling, star formation, BH accretion, and stellar and active galactic nucleus (AGN) feedback. Even though the energy of AGN feedback is injected thermally and isotropically, it leads to anisotropic outflows and buoyantly rising bubbles. We find that the BH accretion rate (BHAR) is highly variable and only correlates strongly with the star formation rate (SFR) and the ICM when it is averaged over more than $1~\rm Myr$. We generally find good agreement with the theoretical precipitation framework. In $10^{13}~\rm M_\odot$ haloes, AGN feedback quenches the central galaxy and converts cool-core systems into non-cool-core systems. In contrast, higher-mass, cool-core clusters evolve cyclically. Episodes of high BHAR raise the entropy of the ICM out to the radius where the ratio of the cooling time and the local dynamical time $t_{\rm cool}/t_{\rm dyn} > 10$, thus suppressing condensation and, after a delay, the BHAR. The corresponding reduction in AGN feedback allows the ICM to cool and become unstable to precipitation, thus initiating a new episode of high SFR and BHAR.

==> Paper idealised elliptical/comparison.tex <==
\subsection{Comparison with previous simulations} \label{subsec:previous-sims}
%In this subsection we compare our results with previous simulations. 

%\subsubsection{The variability of the BHAR and the SFR}
\subsubsection{Different AGN feedback models}
We have shown that our simulations do not have a persistent cooling flow. The BH limits its own growth as well as that of the galaxy by regulating the properties of the ICM. This is accumplished with AGN feedback injected in purely isotropic and thermal form. We now compare these results with previous findings in the literature that used different AGN feedback models. \citet{gaspari2011} showed that an AGN model that uses Bondi-Hoyle accretion and mechanical AGN feedback is able to prevent the formation of a cooling flow in haloes of mass $\approx 4 \times 10^{13}~\rm M_\odot$. They find that this is also true for a model in which AGN feedback is triggered by the accretion of cold gas within $3~\rm kpc$ from the BH. \citet{gaspari2013} find that their cold gas triggered AGN feedback model produces chaotic accretion of gas onto the BH. \citet{gaspari2014} find that self-regulated mechanical jets produce both a realistic cooling time and $L_{\rm X} - T_{500}$ relation, while thermal blast models that are not self-regulated cause excessively long cooling times in the centres of galaxy cluster and too low $L_X$ for $T_{500} \la 1~\rm keV$. Our study agrees with these results in that self-regulated simulations are able to produce realistic cooling times in the centres of galaxy clusters, but also highlights that this can be achieved with purely thermal feedback. 

\citet{meece2017} show that in general the precise implementation of AGN feedback is unimportant and that AGN will self-regulate except for the case of purely thermal AGN feedback. At first sight this appears to contradict our findings. Like us, \citet{meece2017} use a variant of the \citet{booth2009} implementation of thermal AGN feedback. However, \citet{meece2017} use a heating temperature of only $10^7~\rm K$, which is significantly below the virial temperature of their halo and which does not satisfy the \citet{dalla-vecchia2012} criterion for preventing numerical overcooling. We use a significantly higher heating temperature of $10^{8.5}~\rm K$ to suppress such spurious energy losses. As long as both conditions are satisfied the choice of $\Delta T$ will have a limited impact on the cyclic behaviour of the haloes. However, the exact $t_{\rm cool}$ in the centre and mass loading of the outflows will differ. Altogether this sketches a scenario that if the BH model allows self-regulation and if the feedback implementation does not suffer from excessive numerical overcooling, then the exact implementation of the AGN feedback is not critical. 


\subsubsection{High-mass clusters like Perseus}
In the literature, idealised clusters like Perseus with halo masses of around $6\times 10^{14}~\rm M_\odot$, have been extensively studied \citep{li2014a,li2014b,li2015,li2017}, so far mostly using simulations with adaptive mesh refinement (AMR). E.g. \citet[][]{li2015} show that the cold gas mass is regulated by AGN feedback and that it sets both the SFR and average BHAR, with a cycle between episodes of high and low SFRs. They also show (their fig. 2) that on time scales below $t<10^2~\rm Myr$ the BHAR varies over at least 3 orders of magnitude. These findings are in excellent agreement with ours. However, they predict significantly higher SFRs, implying that on average the BCG is actively forming stars and is only quenched for short periods of time. Following cycles of high SFR, the cold gas mass decreases slower than what we are finding. This is probably linked to the fact that a ring of cold gas is formed around the BH that is difficult to destroy by their jet feedback. The mass of the cold ring therefore decreases almost with the speed at which it is converted into stars. We also obtain a cyclic behaviour with episodes of low and high SFRs/BHARs, but in our case the BCG remains quenched during nearly the complete evolution. Similar to \citet{li2015}, our simulations form a ring of cold gas, but in our case it is quickly disturbed. Note however, that our most massive galaxy cluster is almost $1~\rm dex$ lower in halo mass than that in \citet{li2015}.

Cyclic behaviour is also predicted by the simulations of \citet{prasad2015} who report an increase in the BHAR when $t_{\rm cool}/t_{\rm dyn} \leq 10$ due to the condensation of cold gas that feeds the BH. Similar to our findings, their AGN feedback is not able to convert the CC cluster into an NCC cluster. They also find a rotationally supported cold ring around the centre of the BH. The reason that we do not find such a long-lived cold gas ring is likely because our AGN feedback injection is isotropic. \citet{qiu2019} also find that there is a regulation between the cold gas and the BHAR. They find that $t_{\rm cool}/t_{\rm dyn}$ regulates to values slightly higher than $10$ in both a Perseus-like cluster and lower-mass clusters, which is in agreement with our simulations. 

In addition to idealised cluster simulations there are simulations like C-EAGLE \citep{barnes2017,bahe2017} that model galaxy clusters in a cosmological context using nearly the same model for AGN feedback as used here. \citet{barnes2017} find that clusters in C-EAGLE have too large entropy cores and lack CC systems. \citet{barnes2018} studied the evolution of CC clusters in IllustrisTNG. They find that their CC fraction evolves from mainly CC at low $z$ to mainly NCC at high $z$, and that the evolution of the CC and NCC distribution is too strong in the simulation. 

\subsubsection{Lower-mass clusters}
Besides Perseus-mass clusters, \citet{qiu2021} simulated a group with a mass of $\approx 3 \times 10^{13}~\rm M_\odot$. They predict values of $t_{\rm cool}/t_{\rm dyn}$ similar to ours, such that the BH self-regulates. Contrary to \citet{qiu2021}, we find that clusters with this mass also show periodic behaviour in cold gas. The simulations from \citet{wang2019}, who modelled the  elliptical galaxies of NGC5044 and NGC 4472 show that also at halo masses of $M_{200} = 4\times 10^{13}~\rm M_\odot$ there is a periodic behaviour in the amount of cold gas in the centre, regulated by the ratio $t_{\rm cool}/t_{\rm dyn}$. Another different idealised cluster simulation has been performed by \citet{su2021}, who use the FIRE-2 model \citep{hopkins2018} and a dark matter halo mass of $8.5\times 10^{13}~\rm M_\odot$. They find that whether galaxies quench or not depends on the amount of energy that is injected through their different AGN feedback channels, which may however be due to the fact that their AGN model is not self-regulating. \citet{prasad2020b} studied the analytic AGN feedback `valve model' for galaxy models from \citet{voit2020} and found that their galaxies are in reasonable agreement with this model. Like us, they find that cyclic variation of the cold gas content are regulated by AGN feedback.


==> Paper idealised elliptical/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
We have analysed the connection between the ICM, star formation and the AGN using hydrodynamical simulations of galaxy groups/clusters. We developed new initial conditions for a spherical equilibrium system comprising a BCG with a \citet{hernquist1990} profile, a dark matter halo with an \citetalias{navarro1997} density profile, and an ICM profile with two free parameters. The free parameter $T_0$, which sets the central temperature plateau, can be used to initialize different hydrostatic equilibrium profiles for the ICM, ranging from cool-core to non-cool-core systems. The second free parameter is used to specify the cluster gas fraction. To obtain realistic thermodynamic profiles, for each halo mass we calibrate the fiducial values for the two ICM parameters against the cosmological BAHAMAS simulation \citep{mccarthy2017}. 
Using a subgrid model similar to that used in the EAGLE simulation \citep{schaye2015}, which includes radiative cooling, star formation, BH accretion, and both stellar and AGN feedback, we simulate the evolution of haloes with $M_{200}=10^{13}~\rm M_\odot, 10^{13.5}~\rm M_\odot$ $10^{14}~\rm M_\odot$. Our main conclusions are as follows:
\begin{itemize}
    \item Low-mass galaxy clusters ($M_{200}=10^{13}\,\rm M_\odot$) behave qualitatively differently from more massive haloes. They are quickly ($t\la 1~\rm Gyr$) converted from cool-core (CC) into non-cool-core (NCC) by AGN feedback. In contrast, their more massive analogues that are initially CC show periodic behaviour in SFR, BHAR, and ICM properties (see Figs.~\ref{fig:entropy-mean},~\ref{fig:SFH-summary} and \ref{fig:thermoproperties-comparison}). The results for low-mass clusters are insensitive to their initial thermodynamic profile (as long as $t_{\rm cool}/t_{\rm dyn}$ remains realistic). A large amount of cool gas condenses towards the centre resulting in a high BHAR and AGN feedback that quickly quenches the galaxy. The evolution of higher-mass clusters is sensitive to their initial thermodynamic profile. A smaller initial $t_{\rm cool}/t_{\rm dyn}$ yields a higher SFRs that persists for most of the simulation, even after the BH has injected energy exceeding the amount needed to compensate for the initial difference.
    
    \item Even though AGN feedback is injected isotropically and thermally, its interaction with the ISM and ICM results in outflows with a biconical structure (Fig.~\ref{fig:phases-temp}). 
    
    \item The instantaneous BHAR is highly variable and has no strong correlation with the SFR. However, when averaged over timescales $t> 1~\rm Myr$, it correlates strongly with the SFR (Figs.~\ref{fig:SFR-BHAR} and \ref{fig:SFR-BHAR-corr}). 
    
    \item Before an episode of high SFR, the ratio between cooling and dynamical time ($t_{\rm cool}/t_{\rm dyn}$) drops below 10 in the centre (Fig.~\ref{fig:thermoproperties-comparison}). Overall, episodes of low entropy and small $t_{\rm cool}/t_{\rm dyn}$ are preceded by episodes of high SFR and (time-averaged) BHAR (Fig.~\ref{fig:thermoproperties-comparison}), and at the same time episodes of high/low SFR and BHAR precede episodes of high/low entropy and $t_{\rm cool}/t_{\rm dyn}$ in the centre. 
    
    \item In higher-mass clusters showing cyclic behaviour, AGN feedback influences mostly the gas within the radius where $t_{\rm cool}/t_{\rm dyn} < 10$ before the feedback episode. In this region the AGN raises the entropy until $t_{\rm cool}/t_{\rm dyn} \approx 10$, thus suppressing precipitation (Fig.~\ref{fig:thermoproperties-comparison}). At that point cold gas is however still present in the centre, which is either removed by AGN feedback or converted into stars. The cooling time just outside the region where the ratio $t_{\rm cool}/t_{\rm dyn}$ was raised to $\approx 10$ (see row d of Fig.~\ref{fig:BAHAMAS-comparison}) sets the time until the following episode of high SFR and BHAR will take place.
    
    \item Using time-shifted correlations, we quantify the delay between on the one hand SFR or BHAR, and on the other hand entropy or $t_{\rm cool}/t_{\rm dyn}$ (Fig.~\ref{fig:correlation-BHAR}). The results are in good agreement with the precipitation framework in which the value of $t_{\rm cool}/t_{\rm dyn}$ and the entropy of the ICM regulate the inflow of gas towards the centre. However, the AGN feedback influences the logarithmic entropy slope therefore it is not a good predictor for precipitation (Fig.~\ref{fig:slope-voit-corr}).  
    
    \item In order for high-entropy ($K \ga 10^2 ~\rm keV~\rm cm^2$) bubbles to obtain $t_{\rm cool}/t_{\rm dyn}<10$ and condense, they are required to reach significantly larger radii than the radius at which their entropy matches that of the surrounding ICM (Fig. \ref{fig:bubble-K}). Our simulations show that high-entropy bubbles bring cold gas to larger radii such that the cold gas can condense, probably due to pushing of cold gas by hot bubbles, afterwinds caused by hot bubbles and/or bubbles overshooting their equilibrium radius.
    
    \item We find good convergence with the numerical resolution over more than four orders of magnitude in gas particle mass (Fig.~\ref{fig:SFH-res}). However, the oscillatory behaviour of the high-mass clusters is no longer reproduced for gas particle masses below $\approx 6 \times 10^6~\rm M_\odot$, when the interaction between the central ICM and the AGN ceases to be adequately resolved.
\end{itemize}

We have demonstrated that a subgrid model for AGN feedback that injects energy in purely thermal form can convert low-mass clusters from CC to NCC systems, while producing cyclic behaviour for higher-mass CC clusters. In the latter case, long periods during which star formation is quenched are followed by short periods of elevated SFRs and BHARs. The precipitation framework can explain the connection between the ICM and the central galaxy found in our simulations. In the future we intend to investigate how sensitive these results are to the models for BH accretion and AGN feedback.   

==> Paper idealised elliptical/cooling.tex <==
\subsection{How far can feedback compensate the cooling?}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_rate.png}
    \caption{Top: SFH of the $10^{14}~\text{M}_\odot$ halo with the BHAR and the injected energy. Bottom: The radii until which the AGN accretion, SNIa and SNII rate can compensate the cooling rate.}
    \label{fig:cooling-rate-vs-BHAR}
\end{figure}

In our simulation we have three sources of feedback, AGN, SNII and SNIa. We would expect that in general AGN feedback is the dominant source of feedback. Given that a large part of the evolution of the halos that we investigated is depending on the ineraction between the feedback and thermodynamic properties of the gas, we want to see until which radii feedback is able to compensate the cooling of gas. In Fig. \ref{fig:cooling-rate-vs-BHAR} we show the energy injection of all feedback channels (AGN, SNII, SNIa), we can clearly see in Fig. \ref{fig:cooling-rate-vs-BHAR} that the AGN feedback in almost all cases is the dominant source of feedback, however we can also see that when the AGN is not dominant, that the SNIa feedback is the most dominant source, the SNII feedback seems to barely dominate the AGN feedback but also seems to be an important source of feedback, but in general seems to follow the AGN energy injection rate quite closely, while the SNIa seems double the energy injected compared to an AGN only model, meaning that during episodes of low energy injection the energy injected by SNIa is helping the galaxy stay quenched slightly longer, besides this SNIa feedback is at larger radii because it comes from old stars, therefore heating gas that will start in-flowing.

If we look at the bottom plot of Fig. \ref{fig:cooling-rate-vs-BHAR}, we can see the radii until which the different feedback channels compensate the instantaneous cooling rate. We can see in Fig. \ref{fig:cooling-rate-vs-BHAR} that during episodes of high BHAR the AGN feedback can compensate the cooling way beyond the virial radius, we can see that in general when we look at the SNIa and SNII radius we can see that the maximum radius the SNe feedbacks reach is around $10~\rm kpc$, meaning it can only compensate for the cooling inside the galaxy or slightly outside of it, but is not really able to compensate the cooling rate from the CGM. In terms of the total impact on the CGM gas it is more interesting to look at the cumulative behaviour, in Fig. \ref{fig:cooling-rate-vs-BHAR-cum} we show the cumulative behaviour. We can see in FIg. \ref{fig:cooling-rate-vs-BHAR-cum} that the AGN will only after a time of around $2~\rm Gyr$ starts to be close to compensating the cooling until a radii of around $30~\rm kpc$, which seems to be consistent with the fact that the AGN is mainly regulating the thermodynamic cycle and compensating low values of heating. In Fig. \ref{fig:cooling-rate-vs-BHAR-cum} we can also see that the cumulative behaviour for both the the SNIa and SNII only can compensate the cumulative cooling rate up to radii of around $6$ - $10~\rm kpc$, which confirms the idea that SNIa and SNII mainly are able to compensate the cooling just in the galaxy.  

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_rate_cumulative2.png}
    \caption{Top: SFH of the $10^{14}~\text{M}_\odot$ halo with the BHAR and the injected energy. Bottom: The radii until which the AGN accretion, SNIa and SNII rate can compensate the cumulative cooling rate.}
    \label{fig:cooling-rate-vs-BHAR-cum}
\end{figure}




==> Paper idealised elliptical/init_profile.tex <==



==> Paper idealised elliptical/initial_phase.tex <==
We begin our analysis by investigating the overall features of the simulated clusters before focusing in detail on the ICM-AGN connection in \S \ref{sec:ICM-AGN}. In particular, we describe the features emerging in the simulated ICM (\S \ref{subsec:spatialscales}, \S \ref{subsec:risebubbles}) and its radially averaged thermodynamical profiles (\S \ref{subsec:thermoprof}) before analysing the evolution of the SFR and its dependence on the parameter $T_0$ (\S \ref{subsec:sensitivity-SFR}).

\begin{figure*}
	\includegraphics[width=.97\linewidth]{./images/projection_gas_temp_masses_0060_slice.pdf}
    \caption{Comparison of the gas surface density (top row, within $\pm 25~\rm kpc$ (left and middle) or $\pm 15~\rm kpc$ (right) along the line of sight), mass-weighted temperature (second row, infinitely thin slice), mass-weighted  pressure (third row, infinitely thin slice) and mass-weighted shock indicator (bottom row, infinitely thin slice, see text for details) at different physical scales for the $M_{200} =10^{14}~{\rm M}_\odot$ halo. The dotted line in the left panels indicates $R_{500}$. In the left and middle panels a dashed white line indicates the extent of the image to its right. The physical scale is indicated with the black or white bar. In the right columns, black dots within a white circle indicate the position of the BH. All images correspond to time $t=3~\rm Gyr$ from the start of the simulation. The image projection is taken in the plane of the rotation (i.e. the angular momentum vector is pointing out of the paper). Note that some small-scale gas clumps have temperatures and densities well below and above our adopted scaling range, respectively. }
    \label{fig:phases}
\end{figure*}

\begin{figure}
    \centering
	\includegraphics[width=.7\columnwidth]{./images/temp_evolution_close_single_0060.pdf}
    \caption{Mass-weighted logarithmic-averaged temperature distribution in the inner $15~\rm kpc$ of the $M_{200}=10^{14}~\rm M_\odot$ halo. The cold gas in the centre of the halo is similar to structures observed in H$\alpha$ emission.}
    \label{fig:clumpy-temperature}
\end{figure}


\begin{figure*}
	\includegraphics[width=.98\linewidth]{./images/temp_evolution_0060.pdf}
    \caption{Projected gas temperature of the fiducial $10^{14}~\rm M_\odot$ halo in infinitely thin slices at three times separated by $100~\rm Myr$ each ($t=$ 2900 Myr, 3000 Myr and 3100 Myr). The first time frame ($t=2900~\rm Myr$) corresponds to a peak in the SFR and BHAR. The line of sight is approximately perpendicular to the motion of the two prominent bubbles. The online supplementary material shows the evolution more clearly with a movie. Despite a purely isotropic implementation of AGN feedback, the interaction of outflows with the ISM and ICM produces a clearly biconical structure with prominent temperature variations at fixed radius.  
    }
    \label{fig:phases-temp}
\end{figure*}


\subsection{The cluster at different spatial scales} \label{subsec:spatialscales}
To give an impression of how different thermodynamic properties vary on different spatial scales, we first inspect the simulation at a fixed time of $3~\rm Gyr$ for the fiducial simulation of the $M_{200} = 10^{14}~\rm M_\odot$ halo with $T_{\rm min}=10^7~\rm K$. Fig.~\ref{fig:phases} shows the gas mass surface density, temperature, pressure and time derivative of the velocity divergence (defined below) in its four rows. The three columns show images at different spatial scales, with diameters of $2~\rm Mpc$, $200~\rm kpc$ and $30~\rm kpc$, the middle column correspond to our high-resolution region. The online supplementary material has videos that show the evolution of the $200~\rm kpc$ spatial scale for each fiducial halo. 

The central density image reveals the existence of $\approx 20~\rm kpc$ regions with lower density (top middle panel), indicative of previous AGN feedback. These low-density regions have higher-than-average temperatures (middle panel of the 2\textsuperscript{nd} row), such that they are in pressure pressure equilibrium (absence of features in the 3\textsuperscript{rd} row). 

The central $\approx 10~\rm kpc$ of the halo contain many high-density clouds and filamentary structures. These form due to large-scale in-situ cooling which produces large clumps that start collapsing and correspondingly lose their pressure support. This causes the clumps to fall into the centre while rotating around the BH. Close to the BH the large clumps of cold gas are shattered and smaller clumps are brought to larger radii due to the hot bubbles produced by AGN feedback. As seen in Fig.~\ref{fig:clumpy-temperature}, the temperature in the clouds is $< 10^4~\rm K$, indicative of ISM that would be observable in e.g. H$\alpha$ or CO emission (e.g. \citealt{olivares2019}; \citealt{russell2019}). Returning to Fig.~\ref{fig:phases}, we note that clouds have higher pressures than their surrounding ICM (indicated by the light yellow, third row, right panel) implying that they are gravitationally bound. We will return to the importance of these cold gas clouds for the ICM-AGN interaction in \S \ref{sec:ICM-AGN}. 

Shocks and sound waves in the ICM provide an observable record of past AGN episodes that complement the bubbles discussed above \citep[see e.g.][]{sanders2016}. The bottom row of Fig.~\ref{fig:phases} shows a shock/sound wave tracer defined as in \citet{borrow2020}:
\begin{equation}
    \mathcal{S} = \left\{
  \begin{array}{ll}
    \left| \frac{\rm d}{{\rm d} t} \nabla \cdot \mathbf{v}\right| & :  \frac{\rm d}{{\rm d} t} \nabla \cdot \mathbf{v} < 0 ~{\rm or} ~ \nabla \cdot \mathbf{v} < 0,\\
    0 & : \rm otherwise.
  \end{array}
\right.
\end{equation}
The high values of $\mathcal{S}$ in the central few kpc are due to ongoing energy injection by the AGN. At radii $\approx 5~\rm kpc$, the values of $\mathcal{S}$ are overall lower, but show clear ring-like features that indicate outflows from previous AGN episodes. As seen in the third row, the pressure is elevated around the edge of this zone, consistent with an AGN-driven shock front. At larger scales ($10-100~\rm kpc$, middle panel of the bottom row) many more of these rings can be seen, tracing successively older AGN feedback episodes. We note that the top left rising bubble produces a signal on its own that makes the wave tracer less clear in this region. As is evident from the bottom row, the waves disappear beyond $\sim 100~\rm kpc$ due to the degrading resolution (see \S \ref{subsubsec:degrading}). By running a uniform-resolution simulation for $4~\rm Gyr$ we have verified that waves extend all the way to the edge of our simulated halo. 


\subsection{The rise of hot buoyant bubbles} \label{subsec:risebubbles}

To investigate the formation of the biconical bubble structure that can be seen in the temperature distribution at radii of $\approx 100~\rm kpc$, Fig.~\ref{fig:phases-temp} shows the temperature map in three consecutive time frames separated by $100~\rm Myr$; the central image (b) corresponds to the time shown in Fig.~\ref{fig:phases}. The left-most image (a) is just slightly after a peak in the SFR and BHAR (see Fig.~\ref{fig:SFR-BHAR-corr} below). Panel (a) shows two large bubbles at an altitude of around $50~\rm kpc$, formed by the resulting AGN feedback, and several smaller bubbles at smaller radii (some of which are in fact moving in a different direction). The online supplementary material shows the time evolution for all three fiducial haloes. The large bubbles move outwards (central panel), in a way reminiscent of an atomic mushroom cloud, in which they push away the gas above them and produce an inflow of colder gas from lower altitudes. The afterwinds of the hot rising bubbles draw in gas that is colder by at least $0.15$ dex, and lift it to altitudes as high as $100~\rm kpc$ (panel c). This demonstrates that AGN feedback is able to produce fluctuations in the ICM at large distances from the BH. In panel (c) the bubble has risen to its maximum altitude, after which the hotter and colder gas start to disperse and the bubble signature fades away (not shown) over the next $400~\rm Myr$.


We remind the reader that this biconical outflow emerges even though we do not use an explicitly biconical model for AGN feedback. The interaction of the intrinsically isotropic AGN feedback with the inhomogeneous ISM and ICM naturally results in the development of biconical structures in a fully self-consistent fashion. This is consistent with what is predicted by the (cosmological) RomulusC simulation \citep{tremmel2019} and highlights that outflow morphologies on scales of tens of kpc are not necessarily indicative of processes occurring close to the BH.

\begin{figure*}
	\includegraphics[width=.98\linewidth]{./images/radial_profiles_entropy_temperature_density_tcool.pdf}
    \caption{Radially-averaged density (top row), temperature (second row), entropy profiles (third row), and cooling time (bottom row) for the three fiducial simulations of halo masses $M_{200}=10^{13}~\rm M_\odot$, $10^{13.5}~\rm M_\odot$ and $10^{14}~\rm M_\odot$ (left, middle, and right column, respectively). The solid black lines show the volume-weighted median profile based on 160 snapshots spanning 8 Gyr; black dashed lines give the corresponding 16\textsuperscript{th} and 84\textsuperscript{th} percentiles, the grey lines correspond to the initial conditions. Background colours indicate the median time that a particular entropy was reached at each radius. The grey region corresponds to $r>100~\rm kpc$. In the third-right panel, we compare our simulations with the observed ACCEPT galaxy cluster sample \citep{cavagnolo2009}, split into CC and NCC by a central entropy of $50~\rm keV ~\rm cm^2$. The low-mass halo ($M_{200}=10^{13}~\rm M_\odot$) is quickly converted from a CC to an NCC profile. While there is significant scatter in the inner $30~\rm kpc$ with values between CC and NCC, at large radii the scatter is negligible. For the massive haloes $t_{\rm cool}$ is always $\la 1~\rm Gyr$ for $r\la 20~\rm kpc$. $t_{\rm cool}$ decreases with time for gas at $r \ga 10~\rm kpc$, this means that it is inevitable to have new episodes of gas cooling that bring cold gas to the centre. 
    }
    \label{fig:entropy-mean}
\end{figure*}

\begin{figure*}
	\includegraphics[width=.97\linewidth]{./images/SFH_short2}
    \caption{Comparison of the star formation history (SFH) for simulations with different initial central minimum temperatures (different colours and thick curves for the fiducial models) for halo masses of $M_{200}=10^{13}~\rm M_\odot$, $10^{13.5}~\rm M_\odot$ and $10^{14}~\rm M_\odot$ (left, middle and right panels, respectively). Solid curves show the instantaneous SFR (left y-axis), while the dashed curves track the cumulative stellar mass formed (right y-axis). The black dash-dotted line indicates the quenching threshold of sSFR $=10^{-2}~\rm Gyr^{-1}$ (see text for details). For the low-mass halo of $M_{200}=10^{13}~\rm M_\odot$, all initial temperatures lead to rapid ($t\la 1~\rm Gyr$) quenching. More massive haloes instead show oscillatory behaviour with cooler (hotter) cores leading to larger (smaller) mean star formation rates. 
    }
    \label{fig:SFH-summary}
\end{figure*}

\subsection{Mean thermodynamic profiles} \label{subsec:thermoprof}
To understand the short-term fluctuations and the long-term evolution of the ICM in a quantitative way, we investigate the thermodynamic ICM profiles. Fig.~\ref{fig:entropy-mean} shows the volume-weighted, radially-averaged median density, temperature, entropy, and cooling time profiles and their scatter based on 160 snapshots spanning $8~\rm Gyr$ for the fiducial simulations of our three halo masses (different columns). We define the cooling time as
\begin{equation}
 t_\text{cool} = \frac{\frac{3}{2} n k_{\rm B} T}{|\Lambda_\text{net}|},
\end{equation}
where $n$ is the gas number density and $\Lambda_{\rm net}$ is the net radiative cooling rate. To construct the profiles, we first compute the volume-weighted median of the particles in radial bins for each halo individually, and then compute the median profile (black solid line, with 16\textsuperscript{th}/84\textsuperscript{th} percentiles of the profiles indicated by dashed lines). The online supplementary material shows videos of the evolution of the radial profiles for all three haloes that show the evolution of the profiles compared to the SFH. 

As is evident from the third row, all haloes initially have a CC entropy profile (grey line), with central values well below the commonly used demarcation line of $50~\rm keV ~\rm cm^{2}$. For the $M_{200}=10^{13}~\rm M_\odot$ halo, AGN feedback subsequently converts this into an NCC entropy profile, with $K \gg 100~\rm keV ~\rm cm^2$ and $t_{\rm cool}>7~\rm Gyr$ down to $\approx 3~\rm kpc$. Correspondingly, the central temperature is increased by an order of magnitude, while the density is decreased by more than a factor of $10^3$. In contrast, both higher-mass haloes retain a CC, with a time-averaged central entropy below $50~\rm keV ~\rm cm^2$, albeit with significant scatter that regularly results in an NCC-like entropy profile. The $t_{\rm cool}$ is regulates to a constant cooling time for $r<20~\rm kpc$. At large radii ($r \ga 30~\rm kpc$, still well below the edge of the high-resolution region), the profiles remain nearly constant over time, plausibly because outflows produced by AGN rarely reach such large radii (except in the low-mass halo at early times), and if they do, they only cover a small fraction of the total volume (see Fig.~\ref{fig:phases-temp}). The temperature profile at $r>100~\rm kpc$ decreases slightly with time, due to a combination of lower resolution and cooling that is not compensated by shock heating from cosmological accretion. 

In the third-right panel of Fig.~\ref{fig:entropy-mean}, we compare these predictions to the observed CC and NCC entropy profiles of the ACCEPT sample of galaxy clusters\footnote{Consistent with our classification, \citet{cavagnolo2009} used a central entropy of $50~\rm keV~\rm cm^2$ to separate CC from NCC clusters.} \citep[green lines,][]{cavagnolo2009}, which are comparable to our most massive halo (typical $T_X \ga 1~\rm keV$). In general, the entropy profile of our simulated halo agrees well with the observed CC clusters, albeit with a slightly higher entropy in the central $\approx 10~\rm kpc$. The upper range of entropies is comparable to the ACCEPT NCC profile. As we discuss in more detail in \S \ref{sec:ICM-AGN}, this suggests a periodic cycling between CC and NCC states for the $10^{14}~\rm M_\odot$ (and $10^{13.5}~\rm M_\odot$) haloes. 

\subsection{Sensitivity of the SFR to the initial central temperature} \label{subsec:sensitivity-SFR}
We now look at the dependence of the SFR on the initial central minimum temperature of the gas profile in the three different mass galaxy clusters.  

\subsubsection{Star formation histories for different initial central temperature} \label{sec:SFH-T0}
Fig.~\ref{fig:SFH-summary} shows the SFH for our simulations, grouped by halo mass (from left to right: $10^{13}$, $10^{13.5}$ and $10^{14}~\rm M_\odot$). Different values of initial central temperature $T_0$ are represented by different colours. For reference, we indicate the commonly adopted criterion for a galaxy to be quenched, $\rm sSFR < 0.01~\rm Gyr^{-1}$ \citep[e.g.][]{weinmann2006}. For this, we convert from sSFR to SFR based on the initial stellar mass of each simulation, the total stellar mass formed during the $8~\rm Gyr$ (dashed lines) is always negligible compared to the initial stellar mass. 

All galaxies with $M_{200} = 10^{13}\,\rm M_\odot$ are quenched quickly ($t\leq 1~\rm Gyr$) and remain quenched at almost all later times\footnote{This also holds for slightly different quenching criteria.}. This implies that AGN feedback is ubiquitously able to quench group-size haloes, independently of the initial temperature profile. The haloes with large $T_0$ (i.e. $T\geq 10^{6.5}\,\rm K$, not shown) do not form stars because they have $t_{\rm cool} \ga 10 \, t_{\rm dyn}$. These haloes do not cool much and their radiative losses are compensated by adiabatic compression that re-heats the gas. 

Higher halo masses display qualitatively different behaviour. The $10^{13.5}~\rm M_\odot$ simulations with higher $T_{\rm 0}$ ($10^{6.5}~\rm K$ and $10^{6.75}~\rm K$) have oscillatory SFHs, with peak SFRs that tend to increase with decreasing $T_{\rm 0}$. This implies that AGN feedback does not erase the initial conditions and therefore the properties of the haloes with different $T_{\rm 0}$ remain distinct. An exception is the lowest-$T_0$ halo ($10^6~\rm K$, orange line) which starts with a strong starburst but is subsequently transformed due to AGN feedback, resulting in SFRs similar to the $10^{6.5}~\rm K$ halo. The halo with $T_0=10^7~\rm K$ is unable to form stars because of its large $t_{\rm cool}$, similar to the high $T_0$ profiles for the $10^{13}~\rm M_\odot$ haloes. 

At even higher halo masses ($10^{14}~\rm M_\odot$), all four simulations retain distinct SFHs throughout, with a strong dependence of SFR on $T_0$. AGN feedback alone is unable to convert haloes with low initial $T_0$ into something resembling those with high initial $T_0$ and low SFR. This indicates that in order to quench SFR in massive haloes with low central temperatures, we need additional processes beyond what is included in these simulations.  In \S \ref{subsec:regul} we will investigate how the oscillatory behaviour in our simulations is regulated.


\subsubsection{Dependence of the initial SFR on the initial central temperature}
The bottom three rows of Fig.~\ref{fig:BAHAMAS-comparison} show the cooling time, the ratio of cooling to dynamical time ($t_{\rm cool}/t_{\rm dyn}$), and the logarithmic entropy slope for the three different halo masses at $t=0~\rm Gyr$. The dynamical time is defined as
\begin{equation}
 t_\text{dyn} =\sqrt{\frac{2 r}{g}}=\sqrt{ \frac{2 r^3}{G M_{\rm encl}(r)} },
\end{equation}
where $g$ is the local gravitational acceleration and $M_{\rm encl}(r)$ is the total enclosed mass at radius $r$. Since $M_{\rm encl}(r)$ is dominated by the stars of the BCG in the centre, and by the dark matter profile at large radii, at a given radius $t_\text{dyn}$ will remain nearly constant during the simulation. 

As expected, a higher $T_{0}$ leads to a longer initial cooling time and a higher ratio $t_{\rm cool} / t_{\rm dyn}$. When $t_{\rm cool} \ga 10\, t_{\rm dyn}$ gas will not start condensing because it cools slowly and the radiative losses can be compensated by adiabatic compression (see \S \ref{sec:SFH-T0}). However, in the runs with $T_0$ resulting in $t_{\rm cool} / t_{\rm dyn} \la 10$, the cooling is faster and adiabatic compression is unable to compensate the cooling. Therefore, the cooling time $t_{\rm cool}$ sets the time scale for gas to cool down and start condensing. Fig.~\ref{fig:SFH-summary} shows that the cooling time in the inner $10~\rm kpc$ depends on the initial $T_0$ so different times for the onset of star formation are expected.

\begin{figure}
	\includegraphics[width=.97\linewidth]{./images/tcool_tdyan_M14_start}
    \caption{Comparison of $t_{\rm cool}/t_{\rm dyn}$ for the $10^{14}~\rm M_\odot$ halo for different $T_0$ (colours) at time $t=0$ (dashed) and $t=t_{\rm sf}$, immediately before the SFR first reaches $10^{-3}~\rm M_\odot ~\rm yr^{-1}$ (solid line); note that the latter happens already at $t=0$ for $T_0=10^{6.5}~\rm K$ and $10^{6.75}~\rm K$. The black dotted line shows $t_{\rm cool}/t_{\rm dyn}=10$, the threshold for gas to precipitate. When star formation stars, $t_{\rm cool}/t_{\rm dyn} \ll 10$ in the inner $\approx 10-50 ~\rm kpc$, indicating that gas precipitation is not the limiting factor for the onset of star formation.
    %d when star formation starts (continuous). For $\log_{10} T_0/K=6.5$ and $6.75$ IC and when SF stars are the same and only the continuous line is shown. When the star formation stars is defined as the snapshot before the SFR exceeded $10^{-3}~\rm M_\odot ~\rm yr^{-1}$. The black dotted line shows $t_{\rm cool}/t_{\rm dyn}=10$ the point at which gas can start precipitate. The arrows indicate the radii where $t_{\rm cool}/t_{\rm dyn}$ goes below 10. When star formation starts $t_{\rm cool}/t_{\rm dyn} \ll 10$ in the inner 10 kpc.
    }
    \label{fig:tcool-tdyn-M14}
\end{figure}

\begin{figure*}
	\includegraphics[width=.97\linewidth]{./images/SFH_BHAR}
    \caption{Comparison of the BHAR and SFR for the different fiducial haloes at the three different halo masses (left $M_{200} = 10^{13}~\rm M_\odot$, centre $10^{13.5}~\rm M_\odot$ and right $10^{14}~\rm M_\odot$). The left axis shows the SFR, which is coloured blue in all panels. In each panel the dashed horizontal line indicates a quenching criterion of ${\rm sSFR} < 0.01~\rm Gyr^{-1}$. The right axis shows the BHAR, the grey line shows the BHAR at very high time resolution and the orange line shows the BHAR averaged over $50~\rm Myr$. The dotted and dash-dotted lines show 1\% and 10\% of the Eddington accretion rate, respectively. The instantaneous BHAR varies over many orders of magnitudes over short times and is uncorrelated with the SFR. The 50 Myr averaged BHAR is correlated with the SFR.}
    \label{fig:SFR-BHAR}
\end{figure*}

In order to determine the link between $t_{\rm cool}/t_{\rm dyn}$ and the onset of star formation, we show in Fig.~\ref{fig:tcool-tdyn-M14} the radial profile of $t_{\rm cool}/t_{\rm dyn}$, for the four $T_0$ variants of the $10^{14}~\rm M_\odot$ halo at $t=0$ and for the snapshot at $t_{\rm sf}$, the first time the SFR exceeds $10^{-3}~\rm M_\odot ~\rm yr^{-1}$. At the onset of star formation the central $t_{\rm cool}/t_{\rm dyn}$ has already dropped far below $10$, which indicates that this is not the limiting factor that determines when star formation starts.
%the limiting factor that determines gas when gas condensation starts. 

%In order to determine how $t_{\rm cool}/t_{\rm dyn}$ looks just before the onset of star formation we show in Fig. \ref{fig:tcool-tdyn-M14} $t_{\rm cool}/t_{\rm dyn}$ in the IC and the snapshot before the SFR exceeded $10^{-3}~\rm M_\odot ~\rm yr^{-1}$. This shows that before the SFR increases rapidly the $t_{\rm cool}/t_{\rm dyn}$ in the centre satisfies $t_{\rm cool}/t_{\rm dyn} \ll 10$ and thus the $t_{\rm cool}$ is the parameter which determines when stars are forming. 

\citet{voit2017} derived another criterion to determine whether gas is unstable against condensation and precipitation to the centre of the halo: entropy perturbations are unstable when the logarithmic entropy slope satisfies
\begin{align}
    \alpha_{\rm K} \equiv \frac{{\rm d} \ln K }{ {\rm d} \ln r} \la \left( \frac{t_{\rm cool}}{t_{\rm dyn}} \right)^{-2}. \label{eq:voit}
\end{align}
From the bottom row of Fig.~\ref{fig:BAHAMAS-comparison} and Fig.~\ref{fig:SFH-summary} it is evident that the correlation of this ratio with SFR is less strong than is the case for $t_{\rm cool} / t_{\rm dyn}$. For both the $M_{200}=10^{13.5}~\rm M_\odot$- $T_0=10^{6.5}~\rm K$ and $M_{200}=10^{14}~\rm M_\odot$-$T_0=10^{6.75}~\rm K$ haloes, the \citet{voit2017} criterion does not predict condensation while the SFH (Fig.~\ref{fig:SFH-summary}) shows that in both simulations considerable star formation begins almost immediately after $t=0$. All of the above suggest that the initial cooling time set by the initial temperature profile (i.e. $T_0$) is the key factor that decides when significant star formation begins in our simulations. 



\begin{comment}
\subsection{Sensitivity of SFR to initial conditions}
To understand the connection between the initial central minimum temperature of a cluster and its star formation behaviour, we compare simulations of clusters with different central temperatures. As shown in Table \ref{tbl:extra_params}, we consider three different halo masses (i.e. $10^{13} ~\rm M_\odot$, $10^{13.5} ~\rm M_\odot$ and $10^{14} ~\rm M_\odot$) and several central temperatures. Recall that all models start out in hydrostatic equilibrium and with a gas fraction inside $R_{500}$ that is independent of the central temperature. The radial profiles of the temperature, density and entropy, and hence the cooling time are directly influenced by the central minimum temperature. Properties depending on the density like the SFH will also be influenced, for the moment we will mainly focus on the first peak in the SFR. As one of the main results of this paper is the oscillatory behaviour of the SFR, we will first look at the importance of the initial phase and the central minimum temperature before we seek to understand the oscillatory behaviour we find. The oscillatory behaviour will be studied in \S \ref{subsec:longterm} and \S \ref{subsec:regul}.


\subsubsection{The cooling time as an indicator}

In Fig.~\ref{fig:SFH-summary} we show the SFH for the three different halo masses (from left to right: $10^{13}$, $10^{13.5}$ and $10^{14}~\rm M_\odot$) compared with the quenching criterion of $\rm sSFR < 0.01~\rm Gyr^{-1}$. The total stellar mass formed is indicated by the dashed lines. In the bottom three rows of Fig.~\ref{fig:BAHAMAS-comparison} we show important physical properties that change when imposing a different minimum central temperature. The first important physical property that changes is the cooling time, shown in panel (d) of Fig.~\ref{fig:BAHAMAS-comparison}, and defined as:
\begin{equation}
 t_\text{cool} = \frac{\frac{3}{2} n k_{\rm B} T}{|\Lambda_\text{net}|},
\end{equation}
where $n$ is the gas number density, $k_{\rm B}$ is the Boltzmann constant, $T$ is the temperature of the gas and $\Lambda_{\rm net}$ is the net cooling rate. In panel (e) of Fig.~\ref{fig:BAHAMAS-comparison} we show the ratio $t_{\rm cool}/t_{\rm dyn}$, for which we calculate the dynamical time as:
\begin{equation}
 t_\text{dyn} =\sqrt{\frac{2 r}{g}}=\sqrt{ \frac{2 r^3}{G M_{\rm encl}(r)} },
\end{equation}
where $g$ is the local gravitational acceleration, $M_{\rm encl}(r)$ is the total enclosed mass at radius $r$. The dynamical time is dominated by the stars of the BCG in the centre and by the dark matter profile at large radii, therefore the dynamical time at a given radius will remain nearly constant during the simulation. This implies that $t_{\rm cool}/t_{\rm dyn}$ is given by:
\begin{align}
    \frac{t_{\rm cool}}{t_{\rm dyn}} &= \frac{\frac{3}{2} n k_{\rm B} T}{|\Lambda_\text{net}|} \sqrt{\frac{G M_{\rm encl}}{2 r^3}},
\end{align}
where $\Lambda_{\rm net}$ is the net radiative cooling rate per unit volume and the proportionality applies in most cases of interest. At relevant $T$, $\Lambda_{\rm net} \propto \rho^2$. In order to understand the influence of the initial $t_{\rm cool}/t_{\rm dyn}$ we expect that there are three different regimes:  
\begin{enumerate}
    \item The ratio $t_{\rm cool}/t_{\rm dyn}$ at small radii is significantly lower than 10, this results in gas that starts to cool down quickly on timescales of the cooling time. While cooling down, the gas will lose pressure support and will precipitate to the BCG and BH, producing an initial burst of star formation and a high BHAR. 
    \item The ratio $t_{\rm cool}/t_{\rm dyn}$ at small radii is around 10. This means that at the start of the simulation, $t_{\rm cool}/t_{\rm dyn}$ is such that the ICM is stable. Small fluctuations in the density due to SNIa and AGN energy feedback or metal enrichment can make the conditions of the gas such that locally the relation $t_{\rm cool}/t_{\rm dyn}$ drops below 10. Gas with a low ratio starts to cool down on the cooling time, while at the same time losing its pressure support, causing the gas to fall to the BCG. This Produces cold gas in the centre, causing an episode of high SFR and BHAR. Depending on the cooling time, this can take a couple of 100 Myr up to a few Gyr. 
    \item  The ratio $t_{\rm cool}/t_{\rm dyn}$ at small radii is significantly higher than 10. Together with a long cooling time this means that the ICM will stay hot for time scales comparable to the Hubble time and that these simulations will never or barely form stars. This category can be subdivided into two categories. In category (a) the ICM is so hot that the cooling times are similar to the Hubble time. In category (b) the effect of AGN + SNIa can extend the cooling times to the Hubble time. 
\end{enumerate}
This means that based on the initial value of $t_{\rm cool}/t_{\rm dyn}$, we can predict the initial behaviour of the SFR. In the first column of Fig.~\ref{fig:SFH-summary} and Fig.~\ref{fig:BAHAMAS-comparison} we see that for the $10^{13}~\rm M_\odot$ halo there are two different cases for the initial starburst. Three models have an initial central temperature that is equal or below $10^6~\rm K$. And a  $t_{\rm cool}/t_{\rm dyn}$ that is significantly below 10, even below 1 in the inner $10~\rm kpc$. This implies that these three haloes are part of type (i) and will almost immediately start forming stars at a high rate, even before the gas has the time to reach the BH. The haloes that have higher initial central temperatures are completely quenched due to their $t_{\rm cool}/t_{\rm dyn} > 10$, their SFR is so low that they disappear from Fig.~\ref{fig:SFH-summary}. The galaxies in these runs are kept quenched by AGN feedback and star formation will not take place, meaning these galaxies remain quenched for long times, i.e. they are of type (iii). 

We see in the second column of Fig.~\ref{fig:SFH-summary} and Fig.~\ref{fig:BAHAMAS-comparison} the SFH, cooling time and $t_{\rm cool}/t_{\rm dyn}$ for the $10^{13.5}~\rm M_\odot$ halo. The haloes with low initial central temperatures, i.e. $T<10^{6.5}~\rm K$, produce initial $t_{\rm cool}/t_{\rm dyn}$ profiles that are significantly below 10 at small radii, which causes these haloes to start forming stars on the cooling time scale, in this case below $100~\rm Myr$. These haloes therefore belong to type (i). For the haloes with higher initial central temperatures we see that the initial $t_{\rm cool}/t_{\rm dyn}$ is equal or above 10, meaning that these haloes will not directly start forming stars, and will take a cooling time to start forming stars. The halo with $T_{\rm min}=10^{6.75}~\rm K$ starts to form stars after $t_{\rm cool} \approx 500~\rm Myr$, and therefore belongs to type (ii). For even higher $T_{\rm min}$ (i.e. $T_{\rm min}\geq 10^7~\rm K$) we find $t_{\rm cool}/t_{\rm dyn}\gg 10$, and the gas is remains hot and therefore will not form stars (type (iii a)). For $T_{\rm min} = 10^7~\rm K$ the galaxy is quenched with a SFR below $10^{-3}~\rm M_\odot~ \rm yr^{-1}$. 

Lastly, in the third column of Fig.~\ref{fig:SFH-summary} and Fig.~\ref{fig:BAHAMAS-comparison} we show the most massive halo, $M_{200}=10^{14}~\rm M_\odot$. We see in Fig.~\ref{fig:BAHAMAS-comparison} that the lower $T_{\rm min}$ haloes (i.e. $T_{\rm min}<10^7~\rm K$) have $t_{\rm cool}/t_{\rm dyn}< 10$. Based on their initial cooling time, these haloes are expected to have an initial starburst. For the halo with $T_{\rm min}=10^{6.5}~\rm K$ star formation starts immediately, while for the halo with $T_{\rm min}=10^{6.75}~\rm K$ we have to wait a few 10s of Myr. Both belong to type (i). The haloes with higher $T_{\rm min}$ have initially $t_{\rm cool}/t_{\rm dyn}\ga 10$ and will cool down at the cooling time. For the $T_{\rm min} = 10^7~\rm K$ halo this means that the first episode of star formation will start after $500~\rm Myr $, for even higher central temperatures this takes even longer ($t > 1 ~\rm Gyr$).

Altogether, based on the initial central temperature in the galaxy cluster we can determine when and how strong the first episode of star formation is. We find that the initial star formation phase depends on the initial central $t_{\rm cool}/t_{\rm dyn}$ and the corresponding cooling time. Haloes with $t_{\rm cool}/t_{\rm dyn} \ga 10$ stay quenched for a cooling time and only at later times produce a star formation phase while galaxy clusters with low $T_{\rm min}$, and hence $t_{\rm cool}/t_{\rm dyn}<10$ produce initial starbursts. 

\subsubsection{The entropy slope as an indicator}
\citet{voit2017} showed another approach to determining if gas is unstable and will condense and precipitate to the centre of the halo. In this case entropy perturbations are unstable when the logarithmic entropy slope satisfies:
\begin{align}
    \alpha_{\rm K} \equiv \frac{\rm d \log K }{ \rm d \log r} \la \left( \frac{t_{\rm cool}}{t_{\rm dyn}} \right)^{-2}. \label{eq:voit}
\end{align}
From this relation it becomes clear that simulations with small initial $t_{\rm cool}/t_{\rm dyn}$ are even unstable for relatively steep entropy profiles. It also implies that all haloes are unstable if their entropy profile is flat ($\alpha_{\rm K} = 0$) or decreasing outwards ($\alpha_{\rm K} < 0$). Fig.~\ref{fig:BAHAMAS-comparison} shows in panel (a) the entropy profile and the logarithmic entropy slope in panel (f). In panel (a) of Fig. \ref{fig:BAHAMAS-comparison} we see that $T_{\rm min}$ increases the entropy in the ICM for all the different halo masses. Combining this with the entropy slope in panel (f) of Fig.~\ref{fig:BAHAMAS-comparison}, we see that the entropy profile becomes flatter in the centre when a higher temperature is imposed. 

In the case of the $10^{13}~\rm M_\odot$ halo equation (\ref{eq:voit}) predicts well whether the halo will have an initial episode of significant star formation. Here a larger radius at which the criterion is satisfied corresponds to a larger gas mass that is unstable and a higher SFR. Although haloes with high central temperatures have small $\alpha_{\rm K}$, their $t_{\rm cool}/t_{\rm dyn}$ is so high that they do not satisfy the criterion. Therefore, the criterion indicates that haloes with high central temperatures will not start condensing gas\footnote{Note that at small radii ($r<3~\rm kpc$), these haloes satisfy $\alpha_{\rm K} < (t_{\rm dyn}/t_{\rm cool})^2$, this has to do with the discretisation of the particles and not that the gas is actually unstable.}. In the second column of panel (a) and (f) of Fig.~\ref{fig:BAHAMAS-comparison} we show the $10^{13.5}~\rm M_\odot$ halo. For the halo with $T_{\rm min}=10^{6.5}~\rm K$ we see that even though the criterion is only satisfied at very small radii ($r<16~\rm kpc$), it produces an initial star burst phase within the first few $100~\rm Myr$ (see Fig.~\ref{fig:SFH-summary}). This gives the idea that this criterion does not tell us  what will happen in the future but only on what happens instantaneously with the gas. The last column of Fig.~\ref{fig:BAHAMAS-comparison} shows the results for the $10^{14}~\rm M_\odot$ halo, which are similar to those for the $10^{13.5}~\rm M_\odot$ halo. We see that for the $T_{\rm min} = 10^{6.5}~\rm K$ halo the criterion on $\alpha_{\rm K}$ is satisfied ($r<14~\rm kpc$), this halo immediately forms stars at a high SFR. However, if we look at a halo with a slightly higher $T_{\rm min}$ (i.e. $T_{\rm min}=10^{6.75}~\rm K$) we see that even though the criterion is not satisfied at the start of the simulation, this run starts forming stars quickly after the simulation starts ($t\approx 100~\rm Myr$). Altogether this means that the $\alpha_{\rm K}$ criterion works, but only constrains the behaviour on short time scales, To get a more complete picture, it is important to consider $t_{\rm cool}/t_{\rm dyn}$ and $t_{\rm cool}$. 


\subsubsection{Long-term behaviour and importance of $T_{\rm min}$}
\label{subsec:longterm}

In Fig.~\ref{fig:SFH-summary} we show the SFH for all $T_{\rm min}$ and the three different halo masses. All haloes with $M_{200} = 10^{13}~\rm M_\odot$ are quenched quickly and remain quenched for almost all time. This implies that independently of the initial central minimum temperature chosen (as long as it is somewhat realistic), AGN are able to quench all group size haloes. 

For the higher halo masses we see a different behaviour. The $10^{13.5}~\rm M_\odot$ with higher $T_{\rm min}$ runs (i.e. $T_{\rm min}=10^{6.5}~\rm K$ and $10^{6.75}~\rm K$) have oscillatory SFHs, with peak SFRs that tend to increase with decreasing $T_{\rm min}$. This implies that AGN feedback does not erase the initial conditions and therefore the properties of the haloes with different $T_{\rm min}$ remain distinct. However the $10^6~\rm K$ halo has been transformed due to AGN feedback, resulting in SFRs similar to the $10^{6.5}~\rm K$ halo. It is apparent from Fig.~\ref{fig:SFH-summary} that the SFH of the $T_{\rm min} = 10^6~\rm K$ halo is initially similar to that of the $10^{13}~\rm M_\odot$ halo with $T_{\rm min}=0~\rm K$.

The $10^{14}~\rm M_\odot$ halo demonstrates that when we go to even higher halo masses, AGN feedback is unable to convert the low $T_{\rm min}$ models into something resembling the high $T_{\rm min}$ models. This indicates that in order to quench SFR in massive haloes with low central temperatures we need additional processes beyond what is included in these simulations. In section \ref{subsec:regul} we will investigate how the oscillatory behaviour in our simulations is regulated.
\end{comment}






==> Paper idealised elliptical/intro.tex <==

Galaxy groups and clusters are the most massive collapsed structures in the Universe and are unique probes of the large-scale structure because the hot gas in the intracluster medium (ICM) can be observed in X-rays and through the Sunyaev-Zel’dovich effect (SZE) \citep[][for a review]{kravtsov2012}. Furthermore, galaxy clusters are extreme environments where star formation in the central galaxy is suppressed by feedback from the supermassive black hole (BH). Therefore, galaxy clusters can be used to study the interplay between the BH and the ICM and to understand its role in galaxy formation more broadly.


X-ray observations indicate that there are two types of galaxy groups and clusters: those with and without a `cool core' of gas with low temperature, low entropy, high density, and short cooling times \citep[e.g.][]{hudson2010}. These two classes are typically referred to as `cool-core' (CC) and `non-cool-core' (NCC) clusters, respectively. The precise ratio of CC to NCC clusters remains a matter of debate, complicated by a bias of X-ray selected samples towards the (X-ray brighter) CC type \citep[e.g.][]{lin2015,rossetti2017}. Samples of SZE-selected massive galaxy clusters indicated that --- $\approx 30-40$ per cent of clusters at redshift $z \leq0.35$ are CC \citep{andrade-santos2017}. For their (statistical) progenitors at $z=0.3-1.3$, \citet{ruppin2021} derived a CC fraction of $\approx 50$ per cent, indicating that the fraction of CC clusters remains almost constant with increasing redshift. 

The observed thermodynamic profiles of CC clusters would suggest the presence of substantial cooling flows, in which large amounts of gas cool (with rates from $10$s to $1000$s $\rm M_\odot ~\rm yr^{-1}$). However, the observed rate at which gas turns into stars is generally much lower, otherwise the brightest cluster galaxies (BCGs) of galaxy groups and clusters would e.g. be far bluer than observed, an inconsistency that has been termed the `cooling flow problem' \citep{fabian1994}. In addition X-ray spectra (see \citealt{gitti2012} for a review) suggest that the amount of gas that is actually able to cool radiatively to low temperatures ($T\la 10^4~\rm K$) is a factor 2-10 lower than expected from the thermodynamic profiles alone. This indicates that the cooling flows in galaxy groups and clusters, where they exist, must typically be truncated close to the BCG\footnote{Note that there are some BCGs with SFRs of 10s to 100s of $\rm M_\odot ~\rm yr^{-1}$, especially at high redshifts.}. It is generally thought that this is accomplished by an active galactic nucleus (AGN) powered by an accreting BH in the centre of the BCG, which heats the gas and thus offsets the radiative cooling \citep[e.g.][]{mcnamara2007, fabian2012,gitti2012,werner2019,eckert2021}. This causes the gas cooling time ($t_{\rm cool}$) to increase and the cooling flow to stop, with the gas regulating to $t_{\rm cool}/t_{\rm dyn} \approx 10$, where $t_{\rm dyn}$ is the dynamical time (i.e. the time in which the gas would fall to the halo centre in the absence of pressure support; \citealt{voit2015,babyk2018}).


Direct observational evidence for AGN feedback is abundant, especially in X-rays: for instance shocks, ripples and cavities have been detected \citep[see][for a review]{eckert2021}, at scales from groups up to massive galaxy clusters. The X-ray cavities, lower surface brightness features caused by higher temperature and lower density, are thought to be formed due to the injection of energy by the AGN \citep[e.g.][]{eckert2021}. This creates high-entropy bubbles that rise buoyantly and expand, giving rise to larger sizes at greater distances from the centre of the BCG \citep[e.g.][]{dong2010}. Deep observations of X-ray cavities indicate that the power expended to inflate them ($P_{\rm cav}$) can balance the cooling-induced gas luminosity ($L_{\rm cool}$), with a very tight $P_{\rm cav}- L_{\rm cool}$ relation ranging from isolated elliptical galaxies to galaxy clusters \citep[e.g.][]{birzan2008,cavagnolo2010,o-sullivan2011,hlavacek-larrondo2012,eckert2021}. 

%\raggedbottom
However, some cold gas is observed close to the centre of most CC galaxy groups and clusters, implying that cooling flows are not stopped completely \citep[e.g.][]{eckert2021}. Observed cold gas masses range from none \citep[e.g.][]{salome2003,pulido2018} to relatively small amounts ($\approx 3\times 10^8~\rm M_\odot$; \citealp{salome2003,pulido2018}) and to substantial reservoirs ($1.8\times 10^{11}~\rm M_\odot$; \citealp{edge2001}). Resolved cold gas observations often reveal a filamentary structure \citep[e.g.][]{salome2006, salome2011, david2014, temi2018, olivares2019, russell2019}, as well as interactions with satellite galaxies that transport cold gas to the centre of the BCG \citep[e.g.][]{dasyra2012}. Observations indicate that most of the cold gas likely cooled from the hot ICM and is similar for isolated elliptical galaxies and galaxy clusters \citep[see][for a review]{werner2019}. 


For lower-mass haloes ($M_{200} \la 3\times 10^{13}~\rm M_\odot$, where $M_{\Delta}$ is the mass within the radius $R_{\Delta}$ where the average internal density $\langle \rho_{} \rangle = \Delta ~\rho_{\rm crit}$ and $\rho_{\rm crit}$ is the critical density of the Universe), detailed X-ray observations are challenging \citep[e.g.][]{eckert2021}. However, even without direct observational constraints on the presence of AGN at these mass scales, cosmological hydrodynamical simulations need to include AGN feedback in order to predict realistic star formation rates (SFR), stellar masses at $M_\star \ga 10^{11}~\rm M_\odot$ and gas fractions inside $R_{500}$ in haloes with mass $M_{200} > 10^{12}~\rm M_\odot$ \citep[e.g.][]{booth2009, mccarthy2010,crain2015, dave2019}. The same holds for non-cosmological simulations of clusters \citep[e.g.][]{li2014a}. 


Simulations of group/cluster haloes have great potential to provide understanding of the interplay between the BH and ICM through AGN feedback. Many theoretical studies have investigated different aspects of this interplay in the past. Simulations without any AGN feedback generally develop stable cooling flows that build up unphysically massive gas disks \citep[e.g.][]{li2012}. \citet{gaspari2011a} and \citet{meece2017} investigated different accretion models like Bondi-Hoyle or cold gas triggered accretion. Subsequently, \citet{gaspari2014} and \citet{meece2017} investigated different implementations of energy injection for AGN feedback. These studies indicate that when AGN feedback is self-regulated, run-away cooling is prevented, and cold masses and radial profiles agree with observations. The exact mechanism of BH accretion is then not important.

Simulations that focused more closely on the interaction between the ICM and the BH found that when thermal instabilities grow, such that $t_{\rm cool}/t_{\rm dyn} \lesssim 10$ locally, gas starts to condense, loses its pressure support, and falls towards the centre of the halo \citep[e.g.][]{mccourt2012,sharma2012,gaspari2012,gaspari2013}; this process is often referred to as `precipitation' \citep{voit2015b}. The perturbations can be seeded by AGN feedback due to the lifting of colder gas to regions of larger $t_{\rm dyn}$ \citep[e.g.][]{gaspari2013, li2014b, li2014a}, or by the accretion of cold gas with $t_{\rm cool}$ below equilibrium. However, when $t_{\rm cool}/t_{\rm dyn} > 10$, any radial oscillations are damped because the gas is cooling slowly and remains in a quasi-steady state. Consequently, the ICM is expected to self-regulate towards $t_{\rm cool}/t_{\rm dyn} \approx 10$ on timescales of $\sim 1~\rm Gyr$. Based on this general framework, \citet{voit2017} concluded that gas starts to precipitate when $\alpha_{\rm K}\equiv \frac{{\rm d} \ln K }{{ \rm d} \ln r} < \left( \frac{t_{\rm dyn}}{t_{\rm cool}} \right)^2$, where $K$ is the entropy.

At the same time, cosmological simulations have given clues to the overall impact of AGN feedback on the baryon content of massive haloes \cite[e.g.][]{lebrun2014,barnes2017,barnes2018,weinberger2017, pillepich2018,henden2018,zinger2018,dave2019,davies2019}. Detailed insight into the ICM-AGN connection, however, necessitates higher resolution than is typically affordable in this set-up, and even when cosmological simulations have reached sub-kpc resolution \citep[e.g.][]{pillepich2019, tremmel2019}, these are limited to small samples run with one particular model only. Simulations of idealised galaxy groups/clusters allow detailed experiments with careful control of individual model parameters and initial conditions. 

In this paper, we study the interaction between the ICM and the central BH in galaxy groups and clusters with a suite of high-resolution ($m_{\rm gas}=10^5~\rm M_\odot$) idealised simulations of haloes in the mass range $M_{200}=10^{13}-10^{14}~\rm M_\odot$. All our simulations include an AGN model based on a modified Bondi-Hoyle accretion prescription, with feedback energy injected in thermal form. For a self-consistent treatment of gas cooling, star formation, stellar and AGN feedback we use a subgrid model similar to that employed in the EAGLE project \citep{schaye2015,crain2015}. As we will show, this set-up yields realistic NCC or CC clusters (depending on the initial central temperature), whose cooling times are regulated around $1~\rm Gyr$ without unrealistic cooling flows.

\raggedbottom
The remainder of this paper is structured as follows. In Section \ref{sec:IC} we explain how we set up our idealised galaxy cluster simulations. This is followed by an overview of our subgrid-physics model in Section \ref{sec:subgrid} and a description of our simulations and the results obtained from them in Section \ref{sec:results}. Our results are compared with other theoretical models and observations in Section \ref{sec:discussion}. In Section \ref{sec:conclusion} we summarise our main conclusions. 


==> Paper idealised elliptical/observation_comp.tex <==
\subsection{Comparison with observations of cool gas}

\subsubsection{Relation between the amount of cold gas and thermodynamic properties}

Observations indicate that the amount of cold gas in clusters similar to our $M_{200}=10^{14}~\rm M_\odot$ is smaller than $4\cdot 10^{10}~\rm M_\odot$ \citep[e.g.][and other works]{edge2001, salome2003, pulido2018}. Moreover, the large variation in the amount of molecular gas in galaxy clusters indicates that the cold gas content of a galaxy cluster should not be constant in time but should vary over at least two orders of magnitude. In Fig. \ref{fig:thermoproperties-comparison} we show the evolution of the cold gas mass for our fiducial simulations. We can see that the amount of cold gas varies from $10^{7}~\rm M_\odot$ to $10^{10}~\rm M_\odot$, which is in a good agreement with the observations at the same halo mass. \citet{pulido2018} found that they are only able to detect molecular gas when they detect a CC cluster that either has a central cooling time $t_{\rm cool} \lesssim 1~\rm Gyr$ or a central entropy profile $K \lesssim 35~\rm cm^2 ~\rm keV$. They however do not detect any clusters with a molecular mass below $10^8~\rm M_\odot$. Fig. \ref{fig:thermoproperties-comparison} shows that when the cooling time is short, the amount of cold gas is large. When the cooling time is larger than $1~\rm Gyr$, the cold gas mass is below $10^8~\rm M_\odot$, in agreement with the findings of \citet{pulido2018}. Similarly, when the entropy falls below  $35~\rm cm^2 ~\rm keV$ the cold gas mass is above $10^8~\rm M_\odot$, which shows that our simulations agree well with \citet{pulido2018}.

\subsubsection{Clumpy structure of the ISM}

In Fig. \ref{fig:clumpy-temperature} we show the temperature distribution in the inner $15~\rm kpc$ of the $M_{200}=10^{14}~\rm M_\odot$ halo at four different times, separated by 100$~\rm Myr$, around one of the peaks in the SFR. We can see that the simulations predict a filamentary and clumpy multiphase medium in the centre of the BCG. Although the average temperature of the gas is between $10^7$ to $10^{7.5}~\rm K$, a large amount of gas has temperatures below $10^6~\rm K$. Most of the gas with $T\la 10^6~\rm K$ quickly cools to our imposed entropy floor, corresponding to have temperatures below $10^4~\rm K$. While we do not attempt in this paper to reproduce H$\alpha$ or CO observations, we note that the main filamentary structures of the cool gas can be observed in H$\alpha$ but only the densest clumps will have substantial CO emission, in qualitative agreement with observations (e.g. \citealt{olivares2019}; \citealt{russell2019})

\begin{figure}
    \centering
	\includegraphics[width=.7\columnwidth]{./images/temp_evolution_close_single_0054.pdf}
    \caption{Mass-weighted temperature distribution in the inner $15~\rm kpc$ of the $M_{200}=10^{14}~\rm M_\odot$ halo. The cold gas in the centre of the halo is similar to filamentary structures observed.}
    \label{fig:clumpy-temperature}
\end{figure}


==> Paper idealised elliptical/old.tex <==
\begin{comment}
To summarize, based on the central temperature in the galaxy cluster we can determine whether the central galaxy while get a star burst, start quenched but gets star forming after a certain time or remains quenched for eternity. This mainly dependents on the cooling time and the $t_{\rm cool}/t_{\rm dyn}$-ratio. To illustrate this further we do a set of simulations in which we re-scaled the cooling rate by $0.2$ and $0.4$ dex up and down in order to see the impact on the star forming history, in Fig. \ref{fig:cooling-rate} we show the cooling time and $t_{\rm cool}/t_{\rm dyn}$-ratio for the modified cooling rate runs. We can see in this figure that the cooling rate for the none-modified cooling rate results in an initial $t_{\rm cool}/t_{\rm dyn}$-ratio that is very close to 10. We can see that when we increase the cooling rate that we get a lower ratio, while for a lower cooling rate we get a higher ratio. As based on the previous result we would expect that the runs with a higher cooling rate will start forming stars earlier. If we look at Fig. \ref{fig:SFH-rate} it seems that indeed the SFH seems to change as expected.
\end{comment}

\section{How is star formation regulated?}
In this section we will take a closer look at the exact way in which star formation and properties of the CGM play together. To understand this we divide star formation in different episodes shown in Fig. \ref{fig:cycle-criterion}, to summarize the different phases are:
\begin{enumerate}
    \item The rapid increase of the SFR.
    \item The flattening of the SFH.
    \item The initial decline of the SFR.
    \item The persistent decline of the SFR.
\end{enumerate}
We define the phases based on the time at which we determine the boundary between the different phases. We firstly detect peaks in the 50 Myr smoothed SFH using \texttt{scipy.signal.find\_peaks}, using this we select only broad and peaks above a SFR of:
\begin{align}
    \log {\rm SFR} = \log {\rm sSFR}_{\rm quenched} \times M_\star -1.5.
\end{align}
Based on finding all the peaks with widths above 500 Myr we are able to determine the peak of the SFH, based on the peaks of the SFH we look than for the 50 Myr smoothed minimum or first time the galaxy reaches a SFR below $10^{-3}~ \rm M_\odot ~ \rm yr^{-1}$. This gives us the end of phase iv or the start of phase i. Than we are interested in other separation of phases, we do this by finding the time at which the 50 Myr smoothed SFH goes below a factor of e compared to the SFH at the peak. We use the 50 Myr smoothed star formation instead of the instantaneous star formation because the 50 Myr smoothed SFH is fluctuating less on very short times, given that we are mainly interested on the long timescale, small timescale fluctuations are not of uttermost interest.

\begin{comment}
\begin{figure}
	\includegraphics[width=\linewidth]{./images/cycle_criterion.png}
    \caption{The division of an episode of star formation in different phases. (i) the phase of rapid increas of the SFR. (ii) The flattening of the SFH. (iii) The initial decline of the SFR. (iv) the persistent decline of the SFR.}
    \label{fig:cycle-criterion}
\end{figure}
\end{comment}

\begin{enumerate}
    \item
    \item In Fig. \ref{fig:cooling-ratio} we can see that in the centre when the cooling time 
\end{enumerate}

\subsection{Central thermal feedback and short cooling times}
 In Fig. \ref{fig:cooling-time} we can see that the cooling time reaches a maximum of around $1~\rm Gyr$ and at larger radii it does not necessary reach even $1~\rm Gyr$. This is different from what \citet{voit2017} claims thermal feedback is able to do, they claim thermal feedback will always cause the gas in the centre to be above several Gyr, which is worse than what thermal feedback will produce. 




\subsection{Central thermal feedback can regulate the ambient medium}
In Fig. \ref{fig:cooling-ratio} we can see that the $t_{\rm cool}/t_{\rm dyn}$-ratio decreases below an episode of star formation and increases again after an episode and star formation and the corresponding BHAR. But in general we can see that when the ratio is around  $t_{\rm cool}/t_{\rm dyn} \approx 10$ the galaxy is quenched, this basically means that the $t_{\rm cool}/t_{\rm dyn}$-ratio of the CGM is regulated to a value of around $t_{\rm cool}/t_{\rm dyn} \approx 10$. 







\subsection{Entropy profiles behave as expected}
In Fig. \ref{fig:entropy-comparison} we can see that the entropy evolution seems to behave as expected:
\begin{enumerate}
    \item Entropy decreases isentropic with the same cooling rate
    \item The central core of the entropy becomes lower due to precipitation
    \item The entropy in the CGM increases after an episode of AGN feedback/SF
\end{enumerate}







\subsection{Which resolution is required to resolve the precipitation behaviour?}
\begin{itemize}
    \item How does the resolution impact the SFH, see Fig. \ref{fig:SFH-res}
    \item SFH is converged until a certain resolution
    \item Entropy profiles
\end{itemize}

\begin{figure*}
	\includegraphics[width=\linewidth]{./images/SFH_res.png}
    \caption{SFH for the $10^{13}~\rm M_\odot$ and $10^{14}~\rm M_\odot$ halo at different resolutions}
    \label{fig:SFH-res}
\end{figure*}

\subsection{The impact of random numbers}
In Fig. \ref{fig:SFH-seed} we can see that having an identical setup but different random events of AGN feedback and SNe feedback can cause significant different time evolution, in terms of the size of the peaks of SFH, they differ also the exact time difference differs, but the trend between entropy and the SFH do not differ. Meaning the exact behaviour is consistent with precipitation but the exact timing is a bit hard to predict.

\begin{figure*}
	\includegraphics[width=\linewidth]{./images/entropy_comparison_seed.png}
    \caption{SFH for the $10^{14}~\rm M_\odot$ halo and the entropy at different radii for different random number seeds.}
    \label{fig:SFH-seed}
\end{figure*}



\subsection{What drives the oscillations in the SFH?}
In the case of a galaxy cluster with a halo mass of $10^{13}~\rm M_\odot$ we can see in Fig. \ref{fig:SFH-13} that the BH is either able to quench an initial star burst phase or puts so much energy in the CGM that the galaxy will stay quenched for always. However for more massive halo masses we can see in Fig. \ref{fig:SFH-135} and \ref{fig:SFH-14}, that both a galaxy cluster with a halo mass of $10^{13.5}$ and $10^{14}~\rm M_\odot$ do not remain quenched, but rather have episodes of high star formation followed by episodes of low star formation. In the case of having periods we want to understand what sets the periods in the SFH. Continueing on the approach in the previous section we expect that the cooling time and the corresponding $t_{\rm cool}/t_{\rm dyn}$-ratio are important in setting in which phase we are in the quenched-non-quenched evolution. In general we can divide the SFH cycle in four different phases:
\begin{enumerate}
    \item The pre-SFH phase: During this phase the SFH goes below the quenched criteria and continues to become lower due to AGN feedback.
    \item The onset of SFH phase: During this phase the SFH starts increasing very rapidly but the SFH is still quenched. 
    \item The flatting of the SFH phase: During this phase the SFH starts to flatten and reaches the maximum SFH during this cycle. 
    \item The quenching SFH phase: During this phase the AGN heats the gas around the BH causing the SFH to start to decrease and goes below the quenching threshold.
\end{enumerate}
In Fig. \ref{fig:volume-cooling-time} we can see that the cooling time and $t_{\rm cool}/t_{\rm dyn}$-ratio are different for the various phases of the star formation cycle. We see that during the pre-SFH phase the cooling ratio just outside of the galaxy is already significantly below a $t_{\rm cool}/t_{\rm dyn}$-ratio of 10. This means that the gas will cool down on the cooling time scale and will flow inwards with the dynamical time entering the onset of SFH phase, after a very short time around $100~\rm Myr$ later the galaxy already surpasses the quenching criterion, because the galaxy at this point even has a lower $t_{\rm cool}/t_{\rm dyn}$-ratio, a further increase of the SFH cannot be prevented, this means that the galaxy enters the flattening of the SFH phase, at the end of this phase the SFH reaches the peak of this cycle and also the $t_{\rm cool}/t_{\rm dyn}$-ratio will be the lowest in the center, this is followed by the quenching phase in which the AGN feedback reduces the cold gas in the galaxy significantly causing the gas in the galaxy to be very hot and having very large cooling times, with a corresponding very large $t_{\rm cool}/t_{\rm dyn}$-ratio in the centre. However the AGN is not able to increase the $t_{\rm cool}/t_{\rm dyn}$-ratio a lot at large radii ($r>30~\rm kpc$), this means that gas is able to cool down at these radii at the cooling time scale which is around $1~\rm Gyr$. After this we enter the pre-SFH phase during which the SFH still gets lower due to AGN feedback, this phase will take around the time it takes for gas to cool down at the radii that were not influenced by AGN feedback.

How long do we expect the different phases of the SFH cylce to take? Purely based on Fig. \ref{fig:volume-cooling-time}, we understand how long the pre-SFH phase and the onset of SFH phase take, they are directly related to the cooling time of the gas with the lowest $t_{\rm cool}/t_{\rm dyn}$-ratio. However for the two other phases the time of these phases are a bit more difficult because they are not solely based on the cooling time but are highly depending on the exact amount of gas that inflows and the exact amount of energy in feedback that is injected in the cold gas. We will first start with the phases in which the SFH decreases. In this phase we can ignore that new gas is cooling down and the only source of feedback is AGN, which mainly heats the cold gas, this means that the evolution of the cold gas is described by:
\begin{align}
     \frac{\rm d M_{\rm cold gas}}{\rm d t} &= -R_{\rm AGN}.
\end{align}
In which $R_{\rm AGN}$ is the mass rate that is heated by AGN feedback, which is given by:
\begin{align}
    R_{\rm AGN} &= \alpha \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm AGN}} \epsilon_f \epsilon_r {\rm BHAR}(t) c^2.
\end{align}
In which $\alpha$ is a factor of order unity, which means when it is unity that only the gas particles that are heated are decreasing the cold gas mass, but if it is higher than unity it means that a fraction of the gas is also heated due to secondary ways (e.g. shocks or conduction). In general the BHAR and the cold gas mass are not directly related to each other. But in the simulation it seems that the cold gas mass and the BHAR are related to each other to something like:
\begin{align}
    \rm BHAR(t) &= \epsilon_{\rm gas-BHAR} \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right). 
\end{align}
In which $\epsilon_{\rm gas-BHAR}$ is the relation factor that is between 10\% to 0.1\%. Combining the above relations means that we can calculate the e-folding time for the AGN feedback as:
\begin{align}
    t_{\rm AGN} &= \frac{k_B T_{\rm AGN} \cdot 10^9}{\alpha (\gamma -1)\mu m_H \epsilon_f \epsilon_r \epsilon_{\rm gas-BHAR} c^2} \rm yr, \\
    &= 440 ~\rm Myr \left( \frac{T_{\rm AGN}}{10^{8.5}~\rm K} \right) \left( \frac{\alpha \epsilon_{\rm gas-BHAR}}{0.01} \right)^{-1}. \label{eq:e-folding}
\end{align}
Looking at Fig. \ref{fig:cooling-dyn-ratio}, we can see that in the SFH cycle that starts at $2\rm Gyr$, that the e-folding time in the decreasing SFH phase has 3 different slopes, the first phase is starting with a BHAR that is more than 2 orders lower, meaning the e-folding time is around $700\rm Myr$ (following Eq. (\ref{eq:e-folding})), while in the central second phase the BHAR is much higher than $0.01$ and therefore e-folding times decrease to shorter times around $200~\rm Myr$, while after that the e-folding times is around $300~\rm Myr$. This means that the BHAR is important in determining how quick the SFH decreases. 


However the BHAR is not the only thing that determines the exact slope of the decreasing SFH. It is also important to realize that the factor $\alpha$ needs to play some role in setting how fast the SFH decreases, because only based on the BHAR is not enough. This means that gas that is heated also needs to take away part of the gas that is not directly heated by AGN feedback. Especially during episodes of high star formation, the secondary heating of gas is not important because gas that is heated secondary will have severe over-cooling.  In general the density at which thermal feedback is efficient is given by (following Eq. (18) of \citet{dalla-vecchia2012}):
\begin{align}
    n_{H,t_c} &= 23~\rm cm^{-3} \left( \frac{T}{10^{7.5}\rm K} \right)^{3/2} \left( \frac{\langle m \rangle}{10^5 \rm M_\odot} \right)^{-1/2}.
\end{align}

The flattening of the SFH phase is partly chaotic instead of purely determined by timescales, instead of gas falling completely to the center, it is possible that the gas starts forming a stable ring, that is rotating around the BH, keeping the density around the BH low causing a lower BHAR that takes longer for the galaxy to heat the cold gas, at the same time the formation of a disk also means that more gas can form stars while keeping the ring away from the BH. 

\begin{comment}
\subsection{The entropy and the $t_{\rm cool}/t_{\rm dyn}$-ratio}
\begin{itemize}
    \item Entropy is to some way related to the $t_{\rm cool}/t_{\rm dyn}$-ratio, but it seems to be more related to the amount of energy that is injected by feedback.
\end{itemize}

\subsection{The X-ray luminosity}
\begin{itemize}
    \item Small radii are only changing (r<30 kpc)
    \item Higher $t_{\rm cool}/t_{\rm dyn}$ means that the run has a lower X-ray luminosity in the centre. 
\end{itemize}

\subsection{Until which radii can feedback influence the CGM?}
\begin{itemize}
    \item Fig. \ref{fig:coupling:BHARandSFR}
    \item Figure of the cumulative radii, would be interesting
\end{itemize}

\subsection{What is the impact of different realizations of the same galaxy?}
\begin{itemize}
    \item Similar periods?
\end{itemize}
\end{comment}


\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_episodes_of_SFH_mass_weighted.png}
    \caption{Top: Mass weighted cooling time for different phases of the SFH cycle of the galaxy. Bottom: The mass weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_and_entropy_episodes_of_SFH_mass_weighted.png}
    \caption{Top: Mass weighted entropy profile for different phases of the SFH cycle of the galaxy. Bottom: The mass weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_and_Xray_lum_episodes_of_SFH.png}
    \caption{Top: X-ray profile for different phases of the SFH cycle of the galaxy. Bottom: The mass weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_and_Xray_flux_episodes_of_SFH.png}
    \caption{Top: Volume weighted entropy profile for different phases of the SFH cycle of the galaxy. Bottom: The volume weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/SFH_cooling_time_volume.png}
    \caption{The SFH compared with the cooling time at different radii.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/SFH_cooling_time_over_dynamical_time_volume.png}
    \caption{The SFH compared with the $t_{\rm cool}/t_{\rm dyn}$-ratio at different radii.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/SFH_entropy_volume_weighted.png}
    \caption{The SFH compared with the entropy at different radii.}
    \label{fig:SFH-14}
\end{figure}

\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_time_M14_Lambda_dex.png}
    \caption{Top: the cooling time for the $10^{14}~\rm M_\odot$ halo based on the central temperature. Bottom: the $t_{\rm cool}/t_{\rm dyn}$-ratio for the $10^{14}~\rm M_\odot$ halo based on the central temperature.}
    \label{fig:cooling-rate}
\end{figure}


\begin{figure}
	\includegraphics[width=\columnwidth]{./images/Lambda_change.png}
    \caption{SFH of the $10^{14}~\text{M}_\odot$ halo with different cooling rates}
    \label{fig:SFH-rate}
\end{figure}
\end{comment}

\end{comment}

\begin{comment}
A closer look at Fig. \ref{fig:SFH-rate}, lets us realize that the cooling rate is not only important in setting when the initial burst of star formation will take place, but also is important in setting the oscillatory behaviour of the simulation. If we change the cooling rate, this will inversely change the cooling time, so a smaller cooling rate by 0.4 dex, will increase the cooling time by a factor of 0.4 dex. This means that a smaller cooling rate will imply that the same timescales will be at smaller radii. Given that a change in the cooling rate will not influence the dynamical time, this means that the $t_{\rm cool}/t_{\rm dyn}$-ratio will increase at all radii, which means that the radius at which the ratio is around 10, will move inwards (or will even stay above 10).  This will imply a few things:
\begin{enumerate}
    \item The total gas that is within the radius at which we have a  $t_{\rm cool}/t_{\rm dyn}$-ratio of 10 is smaller if the cooling rate is smaller and larger if the cooling rate is larger. Therefore runs that have a smaller cooling rate only have a smaller amount of gas accessible for star formation, this means peaks in star formation will be smaller.
    \item Given that the radius at which the $t_{\rm cool}/t_{\rm dyn}$-ratio is 10 is smaller, this also means that the dynamical time within this region is smaller, therefore the maximal oscillation time in simulations with a smaller cooling rate will be shorter and longer if the cooling rate is larger. 
\end{enumerate}

But this basically only explains half of the picture, after the first burst the SFR decreases due to feedback which is not directly related to the cooling time. In the top panel of Fig. \ref{fig:cooling-dyn-ratio} we show the SFH, BHAR and gas mass and see that the gas mass and SFH are almost perfectly correlated, implying the amount of cold gas sets the SFR, this means that the amount of cold gas needs to decrease. In order to decrease the amount of cold gas we need to look at the impact of the feedback on the cold gas. In general the evolution of cold gas can be described by:
\begin{align}
    \frac{\rm d M_{\rm cold gas}}{\rm d t} &= -R_{\rm AGN} - R_{\rm SNII} - R_{\rm SNIa} - SFR + R_{\rm cooling}. \label{eq:rates}
\end{align}
In which $R_{\rm i}$ with $i=(\rm AGN, \rm SNII, \rm SNIa)$ are the mass rates for the different components and $R_{\rm cooling}$ is the inflow of cold gas produced by cooling. Based on this we can see that the source of a decrease of the amount of cold gas is mainly AGN feedback given that the amount of energy available in SNII and SNIa are lower than in AGN feedback. Based on Fig. \ref{fig:cooling-dyn-ratio} the BHAR can be roughly described as:
\begin{align}
    \rm BHAR(t) &= \epsilon_{\rm gas-BHAR} \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right). \label{eq:BHAR}
\end{align}
In which $\epsilon_{\rm gas-BHAR}$ is a constant close to $0.01$, but in the case of the BHAR, this constant seems to be time dependent, but for now we assume it to be around constant. The mass heating rate of the AGN is given by:
\begin{align}
    R_{\rm AGN} &= \frac{(\gamma - 1) \mu m_H}{k_B T_{\rm AGN}} \epsilon_f \epsilon_r {\rm BHAR}(t) c^2,
\end{align}
In which $T_{\rm AGN}$ is the average temperature to which the AGN needs to heat the gas in order for the gas to produce outflows and remove the cold gas from the center, filling in Eq. (\ref{eq:BHAR}) we obtain:
\begin{align}
    R_{\rm AGN} &= \frac{(\gamma - 1) \mu m_H}{k_B T_{\rm AGN}} \epsilon_f \epsilon_r c^2 \epsilon_{\rm gas-BHAR} \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 } \right).
\end{align}
Ignoring the SNIa and SNII feedback, we obtain an e-folding timescale for the cold gas of around:
\begin{align}
    t_{\rm AGN} &= \frac{k_B T_{\rm AGN} \cdot 10^9}{(\gamma -1)\mu m_H \epsilon_f \epsilon_r \epsilon_{\rm gas-BHAR} c^2} \rm yr, \\
    &= 440 ~\rm Myr \left( \frac{T_{\rm AGN}}{10^{8.5}~\rm K} \right) \left( \frac{\epsilon_{\rm gas-BHAR}}{0.01} \right)^{-1}.
\end{align}
In general when the SFH is very high, this also translates to very high densities in the center of the galaxy, this means that low injection temperatures in the high density cold gas will produce drastic overcooling. In order to overcome this, the gas needs to be heated to sufficiently high average temperatures. The overcooling of feedback is given by Eq. (18) of \citet{dalla-vecchia2012}, which in simplified form is given by:
\begin{align}
    n_{H,t_c} &= 23~\rm cm^{-3} \left( \frac{T}{10^{7.5}\rm K} \right)^{3/2} \left( \frac{\langle m \rangle}{10^5 \rm M_\odot} \right)^{-1/2}.
\end{align}
This means that for SNe feedback we will already have a problem of overcooling at a density of $n_{H,t_c}=23~\rm cm^{-3}$, this implies that when we have a high density in the galaxy, SNe feedback will not help in quenching the galaxy. SNe feedback will only start helping once the density has decreased enough to fall below $n_{H,t_c}=23~\rm cm^{-3}$. In the case of AGN feedback we still have efficient feedback all the way up to densities of $n_{H,t_c}=750~\rm cm^{-3}$. This means that in the high density region only AGN can help quench the galaxy. This basically means that the temperature to which we need to heat the gas in the center in order to quench the galaxy efficient is dependent on the density in the center. Besides getting high temperatures due to feedback it is also possible that gas gets shock heated due to other gas that was heated of energy diffusion heats neighbouring gas particles, this means that it is not necessary to heat all the gas to the injection temperature but an average high temperature will be enough, for example at densities of $n_{H}=130~\rm cm^{-3}$ a average temperature of $10^8 \rm K$ will be enough to heat the gas. This means that the e-folding time scale of AGN feedback basically depends on the exact density. 
\end{comment}


\section{Sketches}
In Fig. \ref{fig:cooling-dyn-ratio} we can see the $t_{\rm cool}/t_{\rm dyn}$-ratio as a function of time for different radii together with the SFH, total cold gas and BHAR. 



In Fig. \ref{fig:cooling-time} we show the SFH of the fiducial simulation and compare it with the cooling time at different radii and different times, we can see that when there is a start of an episode of star formation or when the star formation is still high that the cooling time is relatively short, while when the star formation starts to decrease the gas gets a longer cooling time that is several Gyrs. In Fig. \ref{fig:cooling-dyn-ratio} we can see the  $t_{\rm cool}/t_{\rm dyn}$-ratio as a function of time. Here we can see that the gas initially has a low $t_{\rm cool}/t_{\rm dyn}$-ratio which coincide with an increase in SFH while at large ratios above 10, we see that the the SFH is decreasing rapidly. This basically means that we seem to have a regulated loop between the SFH, gas mass, AGN accretion rate and the $t_{\rm cool}/t_{\rm dyn}$-ratio. 



\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/evolution/Xray_profile_2D.png}
    \caption{SFH of the $10^{13}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/evolution/Xray_profile_2D.png}
    \caption{SFH of the $10^{13}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}
\end{comment}



In Fig. \ref{fig:different-curves} we can see the different curves for the cold gas reservoir for gas below a temperature of $10^5~\rm K$, the SFH and the BHAR. It seems that the cold gas predicts the value for the SFH very well, this means that we can assume in general that the SFH is directly given by the cold gas reservoir available in our simulation, which implies that:
\begin{align}
    \rm SFH(t) = 1 \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right).
\end{align}
Looking more closely at Fig. \ref{fig:different-curves}, it also seems that the BHAR seems to follow on average on timescales of around 50 Myr the cold gas mass quite closely, it however seems that the BHAR is delayed, but for here we assume they are directly related to understand the physics. This means that the accretion rate is given by:
\begin{align}
    \rm BHAR(t) &= \epsilon_{\rm gas-BHAR} \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right). 
\end{align}
In which $\epsilon_{\rm gas-BHAR}$ is a constant close to $0.01$, but in the case of the BHAR, this constant seems to be time dependent, but for now we assume it is exactly $0.01$. 

Given that the amount of cold gas is important in setting both the SFH and the BHAR we look at how the cold gas mass changes as a function of time:
\begin{align}
    \frac{\rm d M_{\rm cold gas}}{\rm d t} &= -R_{\rm AGN} - R_{\rm SNII} - R_{\rm SNIa} + R_{\rm cooling}. \label{eq:rates}
\end{align}
in which $R_{\rm i}$, $i=AGN, SNII, SNIa$ are the mass heating rates that are produced by AGN, SNII and SNIa feedback. $R_{\rm cooling}$ is the mass cooling rate, the amount of mass that cools down per time scale. In the case that we have no cooling flow we can calculate the e-folding time in which the cold gas mass is decreased by a factor of $e^{-1}$, in the case of only taking into account the AGN, we obtain an AGN mass heating rate of:
\begin{align}
    R_{\rm AGN} &= \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm AGN}} \epsilon_f \epsilon_r {\rm BHAR}(t) c^2, \\
    &= \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm AGN}} \epsilon_f \epsilon_r c^2 \epsilon_{\rm gas-BHAR} \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 } \right).
\end{align}
If we fill this in Eq. (\ref{eq:rates}), we obtain a e-folding time for the AGN feedback off:
\begin{align}
    t_{\rm AGN} &= \frac{k_B \Delta T_{\rm AGN} \cdot 10^9}{(\gamma -1)\mu m_H \epsilon_f \epsilon_r \epsilon_{\rm gas-BHAR} c^2} \rm yr, \\
    &= 440 ~\rm Myr.
\end{align}
In a similar approach the mass heating rate for the SNIIs can be calculated as:
\begin{align}
    R_{\rm SNII} &=  \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm SNII}} SFR \eta_{SNII} E_{SNII}, \\
    &=  \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm SNII}} \frac{M_{\rm cold gas}}{10^9} \eta_{SNII} E_{SNII} \rm yr^{-1}.
\end{align}
Meaning the e-folding time for SNII is:
\begin{align}
    t_{\rm SNII} &= \frac{k_B \Delta T_{\rm SNII} \cdot 10^9 \rm yr}{(\gamma -1)\mu m_H \eta_{SNII} E_{SNII}}.
\end{align}
In which $\eta_{SNII}$ is the fraction of stars that produce a SNII, for stars in the range of 8-100 $M_\odot$, this gives $\eta_{SNII}=1.736 \times 10^{-2} \rm M_\odot^{-1}$.
In the case of a heating temperature of $10^{7.5}~\text{K}$, this reduces to $660~\rm Myr$ and for a heating temperature of $10^{8.5}~\rm K$ reduces to $6.6 \rm Gyr$.

The rate of the SNIa however is constant and does not depend directly on the cold gas reservoir but depends on all the old stars that are available in the simulation. This means that the SNIa rate is approximately constant over the whole evolution of the simulation and is given by:
\begin{align}
    R_{\rm SNIa} &= \frac{(\gamma - 1) \mu m_H}{k_B \Delta T} \frac{M_\star \eta_{SNIa} E_{SNIa}}{t_H},
\end{align}
In which $\epsilon_{SNIa}$ is given by $\eta_{SNIa}=4 \times 10^{-3} \rm M_\odot^{-1}$.

To understand a bit more we can  write out de expression in Eq. \ref{eq:rates} to calculate how the system will behave:
\begin{align}
    \frac{\rm d M_{cold gas}}{\rm d t} &= -\left( \frac{1}{t_{\rm AGN}} + \frac{1}{t_{\rm SNII}} \right) M_{\rm cold gas} - R_{\rm SNIa} + R_{\rm cooling} (t),\\
    &= - \frac{M_{\rm cold gas}}{t_{\rm FB}} - R_{\rm SNIa} + R_{\rm cooling} (t),
\end{align}
This means that the solution for this equation will be given by:
\begin{align}
    M_{\rm cold gas}(t) &= M_0 -R_{\rm SNIa} t + e^{-\frac{t}{t_{\rm FB}}} \int R_{\rm cooling} (t') e^{\frac{t'}{t_{\rm FB}}} \rm d t'
\end{align}


\begin{comment}
\begin{align}
    M_{\rm cold gas}(t) &= M_0 -R_{\rm SNIa} t_{\rm FB} + e^{-\frac{t}{t_{\rm FB}}} \int R_{\rm cooling} (t') e^{\frac{t'}{t_{\rm FB}}} \rm d t'
\end{align}
We can see in this expression that the total amount of cold gas in the galaxy depends mainly on the cooling rate, to better understand the exact behaviour we can fill in a dummy function to see how the behaviour would depend on the the period and the amplitude of a sine wave:
\begin{align}
    R_{\rm cooling} (t) &= M_{inf.} \left( \sin \left(\frac{2\pi t}{P}\right) + 1 \right). 
\end{align}
Which will results in a total cold gas as a function of time given by:
\begin{align}
    M_{\rm cold gas}(t) =& M_0 + (M_{inf.}-R_{\rm SNIa}) t_{\rm FB} +\\ &M_{inf.} P t_{FB} \frac{P \sin\left( \frac{2\pi t}{P} \right) + 2\pi t_{FB} \cos\left( \frac{2\pi t}{P} \right) }{P^2 + (2\pi t_{FB})^2}, \\
    =& M_0 + (M_{inf.}-R_{\rm SNIa}) t_{\rm FB} + \\
    & M_{inf.} P t_{FB} \frac{P \sin\left( \frac{2\pi t}{P} \right) + 2\pi t_{FB} \sin\left( \frac{2\pi t}{P} - \frac{\pi}{2} \right) }{P^2 + (2\pi t_{FB})^2},
\end{align}


At which density do we get overcooling of feedback?
The overcooling of feedback is given by Eq. (18) of \citet{dalla-vecchia2012}:
\begin{align}
    n_{H,t_c} &= 23~\rm cm^{-3} \left( \frac{T}{10^{7.5}\rm K} \right)^{3/2} \left( \frac{\langle m \rangle}{10^5 \rm M_\odot} \right)^{-1/2}.
\end{align}
This means that for SNe feedback we will already have a problem of overcooling at a density of $n_{H,t_c}=23~\rm cm^{-3}$, this implies that when we have a high density in the galaxy, SNe feedback will not help in quenching the galaxy. SNe feedback will only start helping once the density has decreased enough to fall below $n_{H,t_c}=23~\rm cm^{-3}$. In the case of AGN feedback we still have efficient feedback all the way up to densities of $n_{H,t_c}=750~\rm cm^{-3}$. This means that in the high density region only AGN can help quench the galaxy. This basically means that the temperature to which we need to heat the gas in the center in order to quench the galaxy efficient is dependent on the density in the center. 
\end{comment}



\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/metallicity_M13_SFR_pure.png}
    \caption{SFH of the $10^{13}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/metallicity_M14_SFR_pure.png}
    \caption{SFH of the $10^{14}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}
\end{comment}

%\subsection{The runs}
%\input{runs.tex}

\subsection{Which channel dominates feedback?}

\subsection{Time scales}
\input{timescales.tex}


\begin{comment}
% Example figure
\begin{figure}
	% To include a figure from a file named example.*
	% Allowable file formats are eps or ps if compiling using latex
	% or pdf, png, jpg if compiling using pdflatex
	\includegraphics[width=\columnwidth]{example}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:example_figure}
\end{figure}

% Example table
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:example_table}
	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		A & B & C & D\\
		\hline
		1 & 2 & 3 & 4\\
		2 & 4 & 6 & 8\\
		3 & 5 & 7 & 9\\
		\hline
	\end{tabular}
\end{table}
\end{comment}

==> Paper idealised elliptical/precipitation.tex <==
\subsection{Comparison with the precipitation framework} \label{subsec:precip}

The causal link between the ICM, AGN and star formation agrees with the precipitation framework \citep[e.g.][]{voit2017}. The evolution of the ratio $t_{\rm cool}/t_{\rm dyn}$ determines the new episodes of star formation as expected.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./images/correlation_combined_SFH_BHAR_slopes.pdf}
    \caption{The Spearman rank correlation coefficient between SFR (BHAR) and volume-weighted $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$ as a function of the delay time $\Delta t$ between the two, for the $M_{200}=10^{14}~\rm M_\odot$ halo. Negative values of $\Delta t$ show how the SFR or BHAR correlate with the past $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$ and vice versa. There is no strong correlation between the past $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$ and the current SFR or BHAR, in disagreement with the precipitation framework.}
    \label{fig:slope-voit-corr}
\end{figure}

\subsubsection{Entropy slope-AGN connection}
One of the predictions of the precipitation framework \citep[e.g.][]{voit2017} is that gas will precipitate when it satisfies inequality (\ref{eq:voit}) for the logarithmic entropy slope $\alpha_{\rm K}$. To check if this is the case in our simulations, we calculate $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$ and show a time-shifted correlation with the BHAR and SFR in Fig.~\ref{fig:slope-voit-corr}. We calculate the volume-weighted entropy slope using all hot gas particles ($T>10^{5.5}~\rm K$) between $3~\rm kpc$ and $30~\rm kpc$. Based on the precipitation framework we expect that BHAR and SFR anti-correlate with past $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$: short cooling times should lead to high BHAR and SFR. Instead, Fig.~\ref{fig:slope-voit-corr} shows the opposite: the peak anti-correlation occurs at slightly positive $\Delta t$. This indicates that the impact of AGN feedback on the entropy slope dominates the correlations. Our picture therefore is that AGN feedback causes a phase of decreased $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$, followed by a decreasing SFR and BHAR on timescales of around $500~\rm Myr$ and  due to the high $t_{\rm cool}/t_{\rm dyn}$ a maximum in  $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$ is reached. This is followed by a period of high SFR and BHAR while the slope is decreasing on timescales of $\Delta t \approx 500~\rm Myr$. %Altogether it seems that $\alpha_{\rm K} (t_{\rm cool}/t_{\rm dyn})^2$ is not a good predictor. 





\begin{figure}
    \centering
    \includegraphics[width=.97\columnwidth]{./images/bubble_rising_reduced.pdf}
    \caption{Adiabatic evolution of a gas bubble rising from the cluster centre ($M_{200}=10^{14}~\rm M_\odot$) with different initial entropies (different colours). In the top panel we compare the initial bubble entropies with the entropy of the ICM and indicate the radii where the two are equal by an arrow and a thin line. The bottom panel shows the cooling time over dynamical time calculated using the \citet{ploeckinger2020} cooling tables. High-entropy bubbles need to rise to radii significantly larger than the radius where their entropy matches that of their environment in order to obtain $t_{\rm cool}/t_{\rm dyn} \ll 10$, as required to condense and precipitate.
    %Comparison at a halo mass of $M_{200}=10^{14}~\rm M_\odot$ of the entropy, density, temperature and the ratio $t_{\rm cool} /t_{\rm dyn}$ of the surrounding gas (solid curve) with gas that has been heated to entropy $K$ (dashed curves) and is rising adiabatically. We calculate the cooling time using the equilibrium cooling tables from \citet{ploeckinger2020} that are used in the simulations. Only when gas rises to significantly higher radii than the radius of their entropy they are able to obtain $t_{\rm cool}/t_{\rm dyn} < 10$ such that they can condense and precipitate.
    }
    \label{fig:bubble-K}
\end{figure}

\subsubsection{Does adiabatically expanding gas become unstable?}
To determine whether gas heated by feedback will start condensing and precipitate back towards the BH, we consider the idealised situation of having a recently heated feedback bubble moving buoyantly to larger radii, until it reaches the radius at which the entropy within the bubble is the same as that of the surrounding medium. The bubble expands until it reaches the pressure of its surroundings. From there on, it will rise buoyantly while satisfying $P_{\rm bubble}=P_{\rm ICM}(r)$, where $P_{\rm bubble}$ is the internal pressure of the bubble and $P_{\rm ICM}(r)$ is the volume-weighted average pressure of the ICM at radius $r$. The entropy injected by AGN (or stellar) feedback is given by
\begin{align}
    K &= 125 ~{\rm keV} ~{\rm cm^2} \left( \frac{\Delta T}{10^{8.5}~\rm K} \right) \left( \frac{n_{\rm H}}{0.1 ~\rm cm^{-3}}\right)^{-2/3},
\end{align}
where $\Delta T$ is the temperature increase due to feedback, $n_{\rm H}$ is the hydrogen number density of the gas that is heated, and we assume $\Delta T \gg T$, the temperature of the gas before heating. Under the assumption that the bubble remains intact, in pressure equilibrium, and rises adiabatically (i.e. the entropy is constant), we can determine its density and temperature at any radius:
\begin{align}
    n_{\rm H} &= \left[ \frac{P_{\rm ICM}(r)}{K} \right]^{3/5}, \\
    T &= \frac{P_{\rm ICM}(r)^{2/5} K^{3/5}}{k_{\rm B}}.
\end{align}
Using these equations, we can compare the ratio $t_{\rm cool}/t_{\rm dyn}$ in the rising feedback bubble with that of the gas at the same radius, using the cooling times from \citet{ploeckinger2020}. Fig.~\ref{fig:bubble-K} shows the entropy and $t_{\rm cool}/t_{\rm dyn}$ for the buoyantly rising gas in the $M_{200}=10^{14}~\rm M_\odot$ halo. We consider bubble entropies in the range $10-300 ~\rm keV~\rm cm^2$ (different colours). After the bubble has risen to the radius corresponding to its own entropy (arrows and vertical thin lines), its $t_{\rm cool}/t_{\rm dyn}$ ratio is almost identical to that of the surrounding gas, which has $t_{\rm cool}/t_{\rm dyn} \ga 10$ (bottom panel). This implies that gas that rises buoyantly to the radius matching its own entropy will not have  $t_{\rm cool}/t_{\rm dyn} \ll10$ and hence will not condense. 

This toy model applies equally to AGN and SN feedback. However, bubbles produced by AGN feedback will typically attain higher entropies because the heating temperature $\Delta T$ is higher. Figs.~\ref{fig:phases} and \ref{fig:phases-temp} show that lower temperature gas ($T\approx 10^{7.2}~\rm K$) can be brought to significantly larger radii than in our toy model ($r\approx 100~\rm kpc$). If gas with entropies around $20~\rm keV~\rm cm^2$ is brought to higher altitude (where $t_{\rm dyn}$ is larger), then this gas will have $t_{\rm cool}/t_{\rm dyn}<10$. This means that cold gas lifted by hotter feedback bubbles, as well as feedback bubbles that overshoot the radius with the same entropy, can produce condensation and the corresponding precipitation.











==> Paper idealised elliptical/regulation.tex <==

\subsection{The ICM-AGN connection} \label{sec:ICM-AGN}

The presence of feedback-induced perturbations in the ICM and the periodicity in the SFR that we have seen above are strongly suggestive of a close interplay between the ICM and the central AGN. We now explore this connection.


\subsubsection{How are star formation and black hole accretion regulated?}
\label{subsec:regul}
As a first step, we show in Fig.~\ref{fig:SFR-BHAR} the evolution of the SFR and the BH accretion rate (BHAR) for our fiducial simulations of the three different halo masses. The light orange curves show the instantaneous BHAR, i.e. computed at each simulation time step. Consistent with previous studies of e.g. the cosmological hydrodynamical EAGLE simulation \citep[][]{mcalpine2017} and of idealised galaxy clusters \citep{li2015, qiu2019}, this shows very strong (orders-of-magnitude) fluctuations on $\la ~\rm Myr$ timescales. When averaged over $50~\rm Myr$, however, slower variations become apparent (dark orange lines): a gradual decrease of the time-averaged BHAR down to almost zero for the $10^{13}~\rm M_\odot$ halo, and oscillations with a period of $\approx 2~\rm Gyr$ for the more massive haloes. The (instantaneous) SFR (blue line) correlates strongly with this time-averaged BHAR, but not with the high-frequency fluctuations. 

The oscillations in the SFR and the BHAR are not perfectly synchronized, however: SFR leads by $\sim 10^2~\rm Myr$. Both the strong correlation and the delay are physically expected: both SFR and BHAR depend on the presence of cold dense gas near the centre of the halo, but they are not co-located. After condensation, cold gas can form stars nearly immediately, but it takes more time for it to flow to the BH at the very centre of the halo. This implies an expected delay of 
\begin{align}
    \Delta t \sim 98 ~{\rm Myr} \left( \frac{r}{10~\rm kpc} \right) \left( \frac{v}{100~\rm km ~\rm s^{-1}} \right)^{-1},
\end{align}
where $r$ is the radius within which gas forms stars ($\sim 10~\rm kpc$) and $v$ its radial velocity ($\sim 10^2~\rm km ~\rm s^{-1}$). 

To quantify the offset and correlation between the SFR and the time-averaged BHAR, we use a time-shifted correlation approach. For a given delay $\Delta t$, we calculate the Spearman rank correlation coefficient of ${\rm BHAR}(t-\Delta t)$ and ${\rm SFR}(t)$, i.e. the correlation strength with the BHAR shifted forward (or equivalently the SFR shifted backward) by $\Delta t$. This approach is non-parametric, so that we can remain agnostic about the exact functional form of ${\rm BHAR}(t)$ and ${\rm SFR}(t)$. Fig.~\ref{fig:SFR-BHAR-corr} shows the resulting Spearman rank correlation coefficient for the $10^{14}~\rm M_\odot$ halo. For averaging timescales $t_{\rm avg} \geq 1~\rm Myr$ there is a very strong peak correlation ($r_{\rm s}\approx 0.8$) between the SFR and BHAR at $\Delta t \approx -50~\rm Myr$,  which is almost independent of the precise value of $t_{\rm avg}$. In other words, the peak (and minimum) SFR is followed by the peak (minimum) BHAR after a delay of $\approx 50~\rm Myr$, in good agreement with our analytic estimate. Results for the $10^{13.5}~\rm M_\odot$ are similar (not shown).

\begin{figure}
	\includegraphics[width=\linewidth]{./images/Spearman_correlation_BHAR_SFH_combined_reduced.pdf}
    \caption{Comparison of the Spearman rank correlation coefficient of SFR and BHAR as a function of delay time $\Delta t$ for different averaging timescales (different colours) for the $M_{200}=10^{14}~\rm M_\odot$ halo. $\Delta t$ is the delay of BHAR with respect to the SFR. The corresponding correlation is calculated as $r_s\left[{\rm BHAR}(t-\Delta t),{\rm SFR}(t) \right]$. We show different values for the time over which the BHAR is averaged (50 Myr to none). When the BHAR is averaged over timescales $t>1~\rm Myr$ there is a strong correlation between the BHAR and SFR, where the past SFR correlates with the current BHAR. There is only a weak correlation when the BHAR is not time-averaged.}
    \label{fig:SFR-BHAR-corr}
\end{figure}



For shorter averaging timescales (i.e. $t_{\rm avg}\ll 10~\rm Myr$) the correlation is significantly weaker, suggesting that BHAR variations on these short timescales are not driven by the global availability of cold gas. Instead, they are plausibly caused by the (stochastic) motion of dense clumps relative to the BH, which do not affect the SFR. This means that it may be challenging to detect correlations between SFR and observational tracers of the (near-)instantaneous BHAR, such as the X-ray luminosity of AGNs. Observables sensitive to the energy injected by AGN over longer timescales, such as radio bubbles, are more promising.


\begin{figure*}
	\includegraphics[width=.97\linewidth]{./images/thermo_evolution_reduced.pdf}
    \caption{Comparison of the SFR and gas properties for the fiducial simulations for the three halo masses ($M_{200} = 10^{13}~\rm M_\odot$, $10^{13.5}~\rm M_\odot$, $10^{14}~\rm M_\odot$). Row (a) shows the SFR as a function of time (blue line); the dashed line corresponds to the quenching criterion of ${\rm sSFR} < 0.01~\rm Gyr^{-1}$. The orange line shows the  cold ($T_{\rm subgrid} < 10^4~\rm K$) gas mass and the mass corresponding to 100 gas particles is indicated by the dotted line. Row (b) shows $t_{\rm cool}/t_{\rm dyn}$ at different radii (differently coloured lines, as indicated in the legend), calculated within concentric shells of $\Delta \log_{10} r = 0.07$ (the dotted line indicates $t_{\rm cool}/t_{\rm dyn}=10$). Row (c) shows the evolution of the entropy (the dotted line indicates $K=50~\rm keV~\rm cm^2$, a common CC/NCC division). The low-mass halo ($M_{200} = 10^{13}~\rm M_\odot$) is quenched quickly and then maintains high entropy and large cooling times in the centre. The higher halo masses instead display oscillatory behaviour in their cooling time, $t_{\rm cool}/t_{\rm dyn}$ and entropy with the same period as the oscillations in the SFR.}
    \label{fig:thermoproperties-comparison}
\end{figure*}


\subsubsection{Central thermal feedback can regulate the ambient medium}
We now show that AGN feedback regulates star formation by raising the ratio $t_{\rm cool}/t_{\rm dyn}$, which stops the supply of cold gas. Fig.~\ref{fig:thermoproperties-comparison} shows the evolution of the SFR and cold gas (top row), $t_{\rm cool}/t_{\rm dyn}$ (middle row) and entropy (bottom row) in the ICM for our fiducial values of $T_0$for the different halo masses. We define as `cold' all gas with\footnote{Defining cold gas as $T_{\rm subgrid} < 10^{4.5}~\rm K$ gives nearly identical results.} $T_{\rm subgrid} < 10^4~\rm K$, i.e. both HI and $\rm H_2$. It is evident that the amount of cold gas directly sets the SFR. For $t_{\rm cool}/t_{\rm dyn}$ and entropy, we select gas particles within 5 narrow radial shells of width $\Delta \log r =0.07$, centred on $\{5.6, 10.0, 17.8, 31.6,56.2\}~\rm kpc$ (different colours).  The $M_{200}=10^{13}~\rm M_\odot$ halo initially has $t_{\rm cool}/t_{\rm dyn} \ll 10$ in its centre and entropies ($\la 10~\rm keV~\rm cm^2$) that are fully consistent with a CC profile. However, the initial cold gas mass in the halo is $\approx 10^{9.5}~\rm M_\odot$ and causes a high initial phase of BH accretion (Fig.~\ref{fig:SFR-BHAR-corr}). Correspondingly, AGN feedback injects a lot of energy such that after less than $2~\rm Gyr$ $t_{\rm cool}$ is raised to $\ga 10^2 \; t_{\rm dyn}$, with $t_{\rm cool} > 7~\rm Gyr$ \citep[a common CC threshold, e.g.][]{gaspari2014}, and $K \approx 10^2~\rm keV~\rm cm^2$. Hence, the initial CC profile is quickly converted into an NCC profile due to AGN feedback. The initial high BHAR produces a long $t_{\rm cool}$ that prevents any further star formation for many Gyr. 


The higher-mass haloes ($10^{13.5}~\rm M_\odot$ and $10^{14}~\rm M_\odot$) on the other hand, show periodic oscillations in their $t_{\rm cool}/t_{\rm dyn}$ ratio and entropy within the inner $30~\rm kpc$, in analogy to the SFR oscillations discussed above. Their central entropy sometimes exceeds $50 ~\rm keV\,\rm cm^2$ and $t_{\rm cool}/t_{\rm dyn}$ regularly drops below $10$. Beyond $\approx 30~\rm kpc$, $t_{\rm cool}/t_{\rm dyn}$ and the entropy remain nearly constant, however. Therefore, they remain a CC cluster over most of their evolution. 

Comparing the oscillations in SFR/cold gas and in the thermodynamic ICM properties, it is apparent that the former have peaks (and troughs) slightly earlier, by a few $100~\rm Myr$. Only after the maximum SFR, when this is already declining again, are the $t_{\rm cool}/t_{\rm dyn}$ and entropy reaching their respective maxima, and analogously for minima. This indicates that the AGN regulates the ICM and induces the periodicity in the SFR. Indeed, simulations without AGN feedback (not shown) show catastrophic cooling and continuously high SFRs. 

The amount of cold gas in the most massive cluster ($M_{200}=10^{14}~\rm M_\odot$) never exceeds $10^{10}~\rm M_\odot$, and regularly drops below $10^8~\rm M_\odot$. Both trends are consistent with observations of molecular gas in BCGs \citep[e.g.][]{edge2001, salome2003, pulido2018}. A connection between cold gas and ICM state was also demonstrated observationally by \citet{pulido2018}. They only detected molecular gas ($M_{\rm mol} > 10^8~\rm M_\odot$) in CC clusters that either have central cooling time $t_{\rm cool} \lesssim 1~\rm Gyr$ or a central entropy $K \lesssim 35 ~\rm keV~\rm cm^2$. This is in good agreement with our simulation, where the cold gas mass drops below $10^8~\rm M_\odot$ only when in the centre we have $t_{\rm cool} \ga 1~\rm Gyr$ or $K \ga 35 ~\rm keV~\rm cm^2$ and vice versa.

A closer look at Fig.~\ref{fig:thermoproperties-comparison} shows that AGN feedback in the simulations raises the cooling time until the ICM is marginally stable, corresponding to $t_{\rm cool} \approx 10\, t_{\rm dyn}$, such that gas is stopped from precipitating and condensing. AGN feedback therefore mainly affects the region $r \ll 10^2$~kpc, where $t_{\rm cool} < 10\, t_{\rm dyn}$ initially. This happens quickly after the SFR and time-averaged BHAR have reached their peak values. After $t_{\rm cool}$ has been raised to $10\, t_{\rm dyn}$, the SFR and BHAR continue to decline until the remainder of the cold gas in the centre has been removed.

Suppressing the precipitation will eventually suppress the fueling of the BH. However, for the high halo masses the cooling time is smaller than $t_\text{H}$ out to $r > 10^2$~kpc (see rows d and e of Fig.~\ref{fig:BAHAMAS-comparison}). Hence, a revival of the cooling flow is unavoidable, leading to feedback cycles. The cooling time at the radius where $t_{\rm cool} \approx 10\, t_{\rm dyn}$ therefore determines the time until the next episode of cold gas condensation. This argument also explains why the cycles get shorter for higher $T_0$ (which can be seen from Fig.~\ref{fig:SFH-summary}). From Fig.~\ref{fig:BAHAMAS-comparison} (rows d and e) we see that for higher $T_0$ the radius at which the condition $t_\text{cool}=10\, t_\text{dyn}$ is reached smaller and that the cooling time at this radius is shorter. While the initial $t_{\rm cool}$ profile is increasing with $r$, after the first episode of high BHAR the $t_{\rm cool}$ profile becomes nearly constant inside $r\la r(t_\text{cool}=10\, t_\text{dyn})$, only after the injection of AGN feedback is significantly lower than its peak the halo will cool with the same $t_{\rm cool}$ for $r\la r(t_\text{cool}=10\, t_\text{dyn})$. As long as AGN feedback is significant, it will keep raising $t_{\rm cool}$ or prevents it from decreasing much in the centre. 



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./images/Spearman_correlation_both_tcool_tdyn_and_entropy_inverted_seed2.pdf}
    \caption{Top: The Spearman rank correlation coefficient for the relation between $t_{\rm cool}/t_{\rm dyn}$ (dashed curves) or ICM entropy (solid curves) and the time-averaged (over $50~\rm Myr$) BHAR (top) or instantaneous SFR (bottom) averaged as a function of the delay $\Delta t$ between the two (see text) for the $M_{200} =10^{14}~\rm M_\odot$ halo. Negative (positive) $\Delta t$ correspond to correlations of entropy and $t_{\rm cool}/t_{\rm dyn}$ with the past (future) BHAR. Different colours indicate different radii. Low $t_{\rm cool}/t_{\rm dyn}$ cause gas to precipitate into cool clouds ($t\sim 3 \times 10^3 ~\rm Myr$) that fall towards the halo centre and increase the SFR and BHAR. The increased BHAR produces outflows that raise the entropy first (within $t\sim 100-250~\rm Myr$) followed by an increase in the cooling time ($t\approx 200~\rm Myr$) that suppresses BHAR and SFR until $t_{\rm cool}$ has decreased enough for the next cycle.
    }
    \label{fig:correlation-BHAR}
\end{figure}


\subsubsection{The causal link between the ICM, AGN, and star formation}

At this point, we have shown that our massive-halo simulations ($10^{13.5}$ and $10^{14} ~\rm M_\odot$) exhibit cyclic variations in the SFR which are strongly correlated (although not perfectly synchronized) with long-term BHAR variations. Likewise, key thermodynamic ICM properties show cyclic variations with a similar period, at least in the central $\la 30 ~\rm kpc$. This naturally raises the question of how these different properties are causally connected: which variations are the drivers, and which are the result of changes in the AGN activity? To address this question, we use the same time-shifted correlation technique that we have already employed for Fig.~\ref{fig:SFR-BHAR-corr}, but now we apply it to the relation between time-averaged BHAR or SFR on the one hand, and the ICM properties $t_{\rm cool}/t_{\rm dyn}$ or entropy on the other.

For each of the four resulting pairs of variables (BHAR-$t_{\rm cool}/t_{\rm dyn}$, BHAR-entropy, SFR-$t_{\rm cool}/t_{\rm dyn}$, SFR-entropy), we plot in Fig.~\ref{fig:correlation-BHAR} the time-shifted Spearman rank correlation coefficient as a function of the shift $\Delta t$ by which we offset the BHAR and SFR evolutions. The correlations with BHAR are shown in the top panel, those with SFR in the bottom one. Since the evolutions of both $t_{\rm cool}/t_{\rm dyn}$ and entropy depend strongly on radial position within the halo (Fig.~\ref{fig:thermoproperties-comparison}), we show four variants of each correlation, with the ICM properties measured within radial shells of width $\Delta \log r = 0.07$ centred on radii $\{5.6, 10.0, 17.8, 31.6\} ~\rm kpc$ (different colours). As in Fig.~\ref{fig:SFR-BHAR-corr}, the feature of key interest is the time shift ($\Delta t$) of the peak (anti-/)correlation as well as its strength: a high - positive or negative - peak at small positive $\Delta t$ indicates that the ICM quantity under consideration will have a strong impact on the BHAR in the near future, whereas a high peak at small negative $\Delta t$ indicates that the ICM quantity has been strongly affected by the recent BHAR. Peaks with a lower amplitude correspond to a weaker connection, whereas peaks at a larger (absolute) $\Delta t$ indicate that the connection has a longer delay time.

Focusing first on the correlation of BHAR with entropy (top panel, solid lines), we see a strong positive correlation coefficient at mildly negative time shifts $\Delta t$. Both the location of the peak and its height vary systematically with radius, in the sense that the ICM closest to the BH ($r=5.6~\rm kpc$, indigo) shows the strongest positive peak correlation with the shortest time offset ($r_{\rm s} \approx 0.75$ and $\Delta t \approx -10^2 ~\rm Myr$, respectively). At larger radii, the correlation is both weaker and has a longer delay ($r_{\rm s} \approx 0.45$ and $\Delta t \approx -250 ~\rm Myr$, respectively, for $r = 31.6 ~\rm kpc$). The peak anti-correlation has a much larger $\Delta t$ ($\approx + 600 ~\rm Myr$), with no strong radial dependence. In other words, an increase in BHAR is rapidly followed by an inside-out increase of the ICM entropy --- consistent with the qualitative picture from Fig.~\ref{fig:phases-temp} --- while the driving effect of low entropy on BHAR takes much longer to develop.

The situation is broadly similar for the correlation between BHAR and $t_{\rm cool}/t_{\rm dyn}$ (top panel, dashed lines). Here, both the positive and negative peaks are offset by approximately $\pm 4\times 10^2 ~\rm Myr$; the former shows the same systematic trend as for entropy (weaker peak correlations at more negative $\Delta t$ for larger radii), with overall larger shifts and lower peak correlation strengths. This implies that AGN feedback affects ICM cooling less directly than it influences entropy, but also that gas cooling has a more significant and faster impact on future BH activity than a decreasing entropy has. 

We note that, contrary to the positive correlation peaks, the $t_{\rm cool}/t_{\rm dyn}$ negative correlation peaks show no strong systematic ordering with radius (except for the largest bin at $\approx 30 ~\rm kpc$, which shows very little cooling time variation in any case; Fig.~\ref{fig:thermoproperties-comparison}). As discussed above, gas cooling only affects the BH after some delay to account for its migration towards the centre, and this delay should be larger for gas cooling from larger radii. The fact that we do not see such a differential delay may imply that only gas cooling from relatively close to the centre (within a few kpc) has a significant impact on the BHAR.

The correlations with SFR (bottom panel of Fig.~\ref{fig:correlation-BHAR}) broadly mirror those for BHAR, with a general shift of all features by $\sim -10^2 ~\rm Myr$, as expected from Fig.~\ref{fig:SFR-BHAR-corr}. This suggests that star formation itself does not significantly influence the ICM (e.g. through SN feedback), and merely acts as an `indicator' of imminent AGN feedback. Also consistent with Fig.~\ref{fig:SFR-BHAR-corr} is the shorter positive time shift of the peak SFR-$t_{\rm cool}/t_{\rm dyn}$ anti-correlation: ICM conditions more conducive to cooling first lead to an increase in SFR (within $\approx 3\times 10^2 ~\rm Myr$), and only later to a higher BHAR.

In summary, we find the following picture of the connection between the ICM, AGN, and SFR in our simulated cluster. Decreasing cooling times lead to low $t_{\rm cool}/t_{\rm dyn}$ causing gas to precipitate into cool clouds (on a timescale of $\sim 3\times 10^2 ~\rm Myr$) that fall towards the halo centre --- mostly from the innermost ICM --- with a further $\sim 10^2~\rm Myr$ delay. There they boost the BHAR, which leads to (anisotropic) outflows of gas that raise the ambient entropy from the inside out (within $\approx 100-250 ~\rm Myr$), and subsequently --- as the bubbles disperse and cover a larger volume fraction --- increase the ICM cooling time. AGN feedback proceeds until $t_{\rm cool}> 10 \, t_{\rm dyn}$ and precipitation is suppressed. Long cooling times suppress both the BHAR and SFR, until $t_{\rm cool}/t_{\rm dyn}$ has dropped sufficiently to initiate the next cycle, which happens after a time similar to the cooling time at the radius out to which precipitation was halted. Any positive feedback effects from the AGN --- i.e. outflows triggering precipitation via a reduction in $t_{\rm cool}$ --- are subdominant and/or occur on much longer time-scales than the negative feedback due to the increase of entropy of the inner ICM. 


Fig.~\ref{fig:thermoproperties-comparison} shows that for the larger halo masses (i.e. $10^{13.5}~\rm M_\odot$ and $10^{14}~\rm M_\odot$) the entropy and cooling time do not evolve much beyond $30~\rm kpc$, which is the precipitation radius $r(t_{\rm cool}\approx 10\, t_{\rm dyn})$. This implies that AGN feedback does not strongly influence gas outside the immediate neighbourhood of the BH. It is natural for the AGN to couple to this region since this is region where condensation occurs. However, AGN feedback could have overshot and affected larger radii, as is the case in the low-mass halo. The fact that this does not occur could be partly because the AGN feedback adopted in our simulations is intrinsically isotropic as opposed to jet-like. However, as demonstrated in Fig.~\ref{fig:entropy-mean}, this feedback still naturally leads to highly anisotropic bubble-like outflows that reach distances as far as $100~\rm kpc$ from the centre. One possibility is therefore that these buoyantly rising bubbles do not significantly impact the mean values of the entropy at $r\ga 30~\rm kpc$. It is possible that our AGN feedback would raise the entropy  out to $r > 30~\rm kpc$ if $t_{\rm cool}/t_{\rm dyn} \la 10$ at these radii, because in that case AGN would need to raise the cooling time at these large radii in order to suppress condensation. Since observed CC and NCC clusters differ in their entropy profiles out to much larger radii (see Fig.~\ref{fig:entropy-mean}), in our current set-up AGN feedback alone does not convert a CC into an NCC cluster. Such a transformation then requires some form of additional input: for example, a major merger may generate significant entropy through shock-heating, and/or may cause the BH to obtain enough fuel to heat the complete core. Unlike the behaviour of the high-mass haloes, AGN feedback is evidently able to convert the low-mass halo ($10^{13}~\rm M_\odot$)  from a CC into an NCC cluster.





==> Paper idealised elliptical/resolution.tex <==
\begin{figure*}
	\includegraphics[width=.97\linewidth]{./images/SFH_res.pdf}
    \caption{Comparison of the star formation history (SFH) for the $M_{200} =10^{13}~\rm M_\odot$ (top row) and $10^{14}~\rm M_\odot$ (bottom row) halo at different resolutions (different columns and colours). The horizontal black dash-dotted line shows the quenching criterion of sSFR $=10^{-2}~\rm Gyr^{-1}$ for the initial stellar mass of the BCG. The low-mass halo ($M_{200}=10^{13}~\rm M_\odot$) is well converged across all resolutions. The highest mass halo ($M_{200}=10^{14}~\rm M_\odot$) converges only up to a resolution of $6.4\times 10^6~\rm M_\odot$; lower resolutions do not show oscillatory behaviour. For the lowest resolutions, the SFR is unresolved during some times; in this case, we set the minimum SFR to $1/8 \times 10^{-2}, 10^{-2}$ and $8 \times 10^{-2} ~\rm M_\odot ~\rm yr^{-1}$ for the resolutions of $m_{\rm gas} = 6.4 \times 10^6, 5.12\times 10^7$ and $4.096\times 10^8~\rm M_\odot$, motivated by equation (\ref{eq:SFRmin}).}
    \label{fig:SFH-res}
\end{figure*}

\begin{comment}
\begin{table}[h!]
  \caption{The runs at different resolutions}
  \label{tab:resolution-runs}
  \centering
  \begin{tabular}{l|r}
   Name & resolution \\ \hline
   high res. 8 & $1.25\cdot 10^4~\rm M_\odot$ \\
   fiducial & $10^5~\rm M_\odot$ \\
   low res. 8 & $8\cdot 10^5~\rm M_\odot$ \\
   low res. 64 & $6.4 \cdot 10^6~\rm M_\odot$ \\
   low res. 512 & $5.12 \cdot 10^7~\rm M_\odot$ \\
   low res. 4096 & $4.096\cdot 10^8~\rm M_\odot$ \\
  \end{tabular}
  %\caption*{A legend, even a table can be used}
\end{table}
\end{comment}

\subsection{What resolution is required?} \label{subsec:resolution}
\begin{comment}
In the literature there is a large variety of cosmological simulations that each have different numerical resolutions, both in terms of their mass and spatial resolution. For example large cosmological simulations like BAHAMAS \citep{mccarthy2017} have numerical resolutions of the order of $10^9~\rm M_\odot$, while state-of-the-art zoom simulations can go as low as $10^3~\rm M_\odot$ (e.g. FIRE2 \citep{hopkins2018}). Between these extreme resolutions there is a large diversity in the literature in the used resolution, motivated predominantly by the goal of the respective simulation. Simulations that have as main goal to study galaxy formation typically have resolutions of around a few $\times 10^6 ~\rm M_\odot$ (e.g. EAGLE \citep{schaye2015,crain2015}). 
\end{comment}

To determine what numerical resolution is required to capture the interaction between the ICM and the BH, we compare sets of simulations for the lowest ($M_{200} = 10^{13}~\rm M_\odot$) and highest ($M_{200} = 10^{14}~\rm M_\odot$) halo mass\footnote{The $10^{14}~\rm M_\odot$ halo at the highest resolution was not run for long due to its computational expense.}. The particle mass is varied by factors of 8 and the gravitational softening by factors of 2. The highest-resolution simulation has a particle mass of $1.25\times 10^4~\rm M_\odot$, 8 times lower than our fiducial simulation and comparable to high-resolution zoom simulations of individual galaxies \citep[e.g.][]{font2020}. The lowest-resolution simulation has a particle mass of $4\times 10^{8}~\rm M_\odot$, which is comparable to the resolution used in cosmological simulations of large samples of galaxy clusters \citep[e.g.][]{mccarthy2017,barnes2017b,cui2018}. % See Tab. \ref{tab:resolution-runs} for the different runs. 

\begin{comment}
\begin{figure}
	\includegraphics[width=\linewidth]{./images/radial_profiles_entropy_res_small.pdf}
    \caption{Comparison of the volume-weighted median entropy profiles for the $M_{200} = 10^{14}~\rm M_\odot$ halo at different resolutions (different colours) averaged over the duration of the simulations. Solid (dashed lines) indicate radii larger (smaller) than three gravitational softening lengths. There is good convergence above three gravitational softening or $5~\rm kpc$. Convergence below $\sim 10~\rm kpc$ produces a SFR with oscillatory behaviour.}
    \label{fig:entropy-res}
\end{figure}
\end{comment}

The top and bottom rows of Fig.~\ref{fig:SFH-res} show the SFH of the $M_{200}=10^{13}~\rm M_\odot$ and the $M_{200}=10^{14}~\rm M_\odot$ haloes, respectively. We do not expect perfect convergence for several reasons. First, the initial density profile is realised using a finite number of particles based on stochastic sampling. Second, stellar and AGN feedback are implemented stochastically. Third, the density threshold for star formation implies the existence of a minimum nonzero SFR,

\begin{equation}
{\rm SFR}_{\rm min} = 3.5 \times 10^{-3} ~ {\rm M_\odot} ~{\rm yr}^{-1} \left( \frac{m_{\rm gas}}{10^7~\rm M_\odot} \right) \left( \frac{n_{\rm H}}{0.1 ~\rm cm^{-3}}\frac{T}{8\times 10^3~\rm K} \right)^{0.2}. \label{eq:SFRmin}
\end{equation}
Taking these considerations into account, we see good convergence for the $10^{13}~\rm M_\odot$ halo. In particular, for all resolutions the SFR declines rapidly to values significantly below the division between star-forming and quenched galaxies (horizontal line). For the $10^{14}~\rm M_\odot$ halo, the convergence is good down to a particle mass of $6.4\times 10^6~\rm M_\odot$. For higher particle masses (i.e. lower resolutions) the SFH no longer shows oscillatory behaviour. This can be understood by the fact that at resolutions of $5.12\times 10^7~\rm M_\odot$ and $\varepsilon=2.4~\rm kpc$ the central region around the BH is not properly resolved and therefore the ICM-AGN connection is no longer modelled correctly. 

Unlike the resolution, randomness in the simulation produced by our random number generator does not qualitatively impact our results (see Appendix \ref{app:random}). 



==> Paper idealised elliptical/runs.tex <==
\subsection{Fiducial run}

\begin{itemize}
    \item We can see in \ref{fig:fid:power-spectrum} that the BHAR accretion rate seems to have a flat power spectrum, this means that the value of the BHAR is mostly random and does not have a significant behaviour in time. This mainly implies that when the BHAR is very high or lower is random. 
    \item It seems that both the SFR and the log of the BHAR behave following pink noise in which the slope of the power spectrum is close to $-1$, this means that the energy of fluctuations is independent of the time in which you look.
    \item If we further look into the curve for the log of the BHAR in Fig. \ref{fig:fid:power-spectrum} we see that on short frequencies the power spectrum is close to $-1$, but at frequencies around $log \nu = -1.5$ there is a peak, this indicates that the behaviour of the BHAR is influenced by a timescale that is around $T=30~\rm Myr$. If we further look at this power spectrum we see that around $\log \nu = -0.8$ the power spectrum still behaves around pink noise. If we go to frequencies of around $\nu = 10^{-0.5} ~\rm Myr^{-1}$ or timescales of $T\sim 3 ~\rm Myr$ we see that the power spectrum becomes almost flat. Meaning the exact value of BHARs is almost white noise while, at smaller times we see that at times off around $T\sim 0.25 \rm Myr$ the power drops again. 
    \item In Fig. \ref{fig:fid:correlation} we show the correlation between the value of the SFR and the BHAR. We can see that when we have a BHAR that is high we expect that the SFR will be anti-correlated and therefore lower after around $300~\rm Myr$. In the case of having a high SFR it seems that the BHAR will than also be high after a while because the SFR correlated with the BHAR.
\end{itemize}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/fid/fid_M14_FFT_summary_binned.png}
    \caption{Power spectrum of the SFR, log SFR, BHAR and log BHAR.}
    \label{fig:fid:power-spectrum}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/fid/fid_M14_Correlation_coefficient.png}
    \caption{Correlation between log SFR and log BHAR.}
    \label{fig:fid:correlation}
\end{figure}

\subsection{The coupling coefficient}

\begin{itemize}
    \item Larger coupling coefficient for the AGN leads to smaller accretion rates on average see Fig. \ref{fig:coupling:BHARandSFR} and \ref{fig:coupling:histogram}, the SFHs seem to be similar, but there seems to a trend that larger coupling coefficients have larger periods between periods of non-quenched and quenched.
    \item When the BHAR is high, this has a delayed negative correlation with the SFR, while if the SFR is high this causes the BHAR to increase in the future. The size of the effect seems to be similar for a coupling coefficient of $0.1$ and $0.01$ and smaller for $1.0$. Furthermore the exact delay seems to be similar between $1.0$ and $0.1$, to be around $350~\rm Myr$ while the delay for the small coupling coefficient of $0.01$ seems to be off the order of around $800~\rm Myr$.
\end{itemize}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/coupling/coupling_SFR_BHAR_25Myr.png}
    \caption{Top panel: Star formation history smoothed over 25 Myr, bottom pannel: BHAR smoothed over 25 Myr.}
    \label{fig:coupling:BHARandSFR}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/coupling/coupling_histogram_BHAR.png}
    \caption{Cumulative histogram of the BHARs}
    \label{fig:coupling:histogram}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/coupling/coupling_SFR_BHAR_correlation.png}
    \caption{Pearson correlation coefficient for a given delay of the BHAR with respect to the SFR.}
    \label{fig:coupling:correlation}
\end{figure}

\subsection{Krumholz vs Bondi-Hoyle}

\begin{itemize}
    \item Bondi-Hoyle has a higher SFR and lower accretion rate than Krumholz, see Fig. \ref{fig:krumBH:BHARandSFR} and \ref{fig:krumBH:hist}.
    \item The power spectrum does not show the same peak at $30~\rm Myr$, instead it seems that at high frequencies the power is much higher and at low frequencies the behaviour is more flat, see Fig. \ref{fig:krumBH:hist}. 
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/krumBH/KrumBH_M14_log_SFR_and_log_BHAR_smoothing25Myr.png}
    \caption{Top panel: Star formation history smoothed over 25 Myr, bottom pannel: BHAR smoothed over 25 Myr.}
    \label{fig:krumBH:BHARandSFR}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/krumBH/KrumBH_M14_histogram_accretion_cumulative.png}
    \caption{Histogram of the accretion rate}
    \label{fig:krumBH:hist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/krumBH/KrumBH_M14_FFT_log_BHAR_binned.png}
    \caption{}
    \label{fig:krumBH:power-spectrum}
\end{figure}

\subsection{Isotropic vs Minimum distance}
\begin{itemize}
    \item Minimum distance feedback is more smooth in the accretion rate than the isotropic feedback, see Fig. \ref{fig:injection:BHARandSFR}
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/injection/injection_M14_SFR_and_BHAR_smoothing25Myr.png}
    \caption{Top panel: Star formation history smoothed over 25 Myr, bottom pannel: BHAR smoothed over 25 Myr.}
    \label{fig:injection:BHARandSFR}
\end{figure}

\begin{enumerate}
    \item Nngb variations
    \item Heating temperature: higher heating temperature quenching takes longer but stay also quenched longer. Also higher accretion rates seem to have 
    \item Bondi-Hoyle and boost: Boost means lower SFR, SFR plot. When
you boost the accretion rate the accretion rate behave more stable on
small scales as compared to without boost in which case it fluctuates
a lot
    \item Krumholz and boost: very similar to the Bondi-Hoyle part, only here
both models quench reasonable.
    \item higher coupling constant means you stay quenched longer after SF
and SF rises less. Ofcourse also the common thing of higher coupling coefficient means
lower accretion rate to reach the same. For this part it is also in-
\end{enumerate}


==> Paper idealised elliptical/seed.tex <==




\section{The impact of random numbers}
\label{app:random}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/evolution_seeds}
    \caption{Comparison of the SFR (top panel) and $t_{\rm cool}/t_{\rm dyn}$ ratio (bottom panel) for the $10^{14}~\rm M_\odot$ halo using three different random seeds (different colours). Although the absolute periods and phases are different for different seeds, the relation between the SFR and $t_{\rm cool}/t_{\rm dyn}$ ratio remains largely unaffected.}
    \label{fig:SFH-seed}
\end{figure}


The subgrid model used in the simulations depends heavily on random numbers because the star formation and SNe/AGN feedback are stochastic. Therefore, to investigate whether our results are qualitatively influenced by different random numbers, we investigate two additional runs that have identical physics and initial conditions but use different random number seeds. Fig. \ref{fig:SFH-seed} shows the SFR and $t_{\rm cool}/t_{\rm dyn}$ ratio at 10 kpc. The exact positions and amplitudes of the peaks is influenced by the random number seeds, but the connection between the SFR and $t_{\rm cool}/t_{\rm dyn}$ ratio remains qualitatively the same. This means that the general results are insensitive to the use of different random numbers. 





==> Paper idealised elliptical/simulations.tex <==
\section{Simulations}
\label{sec:subgrid}

Starting from the initial conditions described above, we have run a suite of simulations with the N-body + hydrodynamics code \texttt{SWIFT} \citep{schaller16,schaller2018}. Self-gravity of the baryons is solved with a fast multipole method \citep{greengard1987} while the external gravitational forces from the dark matter halo is approximated by a static external potential (see \S \ref{sec:IC}). Self-gravity is softened with a Plummer-equivalent softening length of $\varepsilon_{\rm grav} = 300~\rm pc$. Particle time steps are fully adaptive, based on the local acceleration ($\Delta t \propto 1/\sqrt{|\mathbf{a}|}$) and limited to 1 per cent of the circular orbital period at the particle's position. For gas, we additionally apply the Courant–Friedrichs–Lewy (CFL) condition and the \citet{durier2012} time step limiter in the vicinity of recent feedback events. For the hydrodynamics, we use SPHENIX \citep{borrow2020}, a density-energy based SPH scheme that includes artificial conduction and artificial viscosity to capture shocks and contact discontinuities. The smoothing lengths of the high-resolution particles are adaptively set to $1.2348$ times the local inter-particle separation (corresponding to 58 neighbours), limited to a minimum of $0.01 \varepsilon_{\rm grav} = 3~\rm pc$. The gas particles have a maximal smoothing length $h_{\rm max}=250~\rm kpc$, and the high-resolution particles all have $h<5~\rm kpc$.

\subsection{Radiative cooling and star formation}
Radiative gas cooling and heating is implemented using the tables of \citet{ploeckinger2020}, which used \texttt{CLOUDY} \citep{ferland2017} to calculate the individual equilibrium cooling and heating rates for the 11 most important elements (H, He, C, N, O, Ne, Mg, Si, S, Ca, Fe), in the presence of a spatially uniform, time-varying UV background based on the model of \citet{faucher-giguere2020}, interstellar radiation and cosmic rays that depend on local gas properties through the Kennicutt-Schmidt (KS) relation \citep{kennicutt1998}, and dust (assuming a constant dust-to-gas ratio of $(D/G)=5.6\times 10^{-3}$ at high densities and a lower dust-to-gas ratio at lower densities that scales also with the KS relation). The cooling tables account for self-shielding of gas, using a cloud size given by the local Jeans length. 

Our simulations do not model the cold phase ($T \la 10^4~\rm K$) of the ISM. We therefore impose a temperature floor corresponding to a constant Jeans mass as proposed by \citet{schaye2008},
\begin{align}
 T_{\rm floor} &= T_{\rm floor, 0} \left(\frac{\rho_{\rm g}}{\rho_{\rm g,0}}\right)^{1/3},
\end{align}
normalised to $T_0=8000~\rm K$ at a density of $n_{\rm H} =0.1~\rm cm^{-3}$. Numerically, this is implemented as an entropy floor and we convert between entropy and temperature assuming a hydrogen mass fraction $X=0.756$ and mean particle mass $\mu=1.22$ of neutral primordial gas for all gas particles. 


%The floor prevents artificial fragmentation of gas that we do not properly resolve. Instead of imposing the floor as a temperature or pressure floor we directly impose an entropy floor given by:
%\begin{align}
%    K_{\rm floor} &= \frac{k_{\rm B} T_0 X^{2/3}}{\mu m_{\rm H}^{5/3}} \frac{1}{(n_{\rm H} n_{\rm H,0})^{1/3}},
%\end{align}
%where we adopt a value of $T_0=8000~\rm K$ and $n_{\rm H,0}=0.1~\rm cm^{-3}$ for the normalization of the entropy floor. For this floor we assume that every SPH particle has a hydrogen mass fraction (X) and mean particle mass ($\mu$) equal to the value for neutral primordial gas, $X=0.756$ and $\mu = 1.22$. 

Gas with entropy within $0.3~\rm dex$ of the floor is assumed to be multi-phase, with an unresolved cold dense component. We use the tables of \citet{ploeckinger2020} to calculate a subgrid temperature $T_{\rm subgrid}$ of this cold phase, and the corresponding subgrid density $\rho_{\rm subgrid}$, by assuming that the gas is in thermal and pressure equilibrium\footnote{For gas that is more than $0.3~\rm dex$ above the floor, the subgrid temperature and density are identical to the SPH temperature and density.}. Gas with $T_{\rm subgrid}< 8\times 10^3~\rm K$ is considered to be star-forming. This mainly selects gas that is on the temperature floor, with a star formation rate based on its pressure following \citet{schaye2008}.

\subsection{Stellar feedback and chemical enrichment}
Once formed, a star particle is assumed to represent a simple stellar population (SSP) with uniform metallicity and formation time, each following a \citet{chabrier2003} initial mass function (IMF) with a mass range of $0.1-100~\rm M_\odot$. For the stellar enrichment we follow \citet{wiersma2009}, with the modifications described in \citet{schaye2015}, which accounts for stellar winds from AGB and massive stars, core collapse supernovae (SNII) and type Ia supernovae (SNIa). %, which for every particle calculates the fraction of stars that reach the end of their main-sequence phase, based on stellar mass and metallicity dependent yield tables from \citet{portinari1998}, then all neighbouring gas particles get a fraction of mass related to their SPH weighting based on their initial mass and distance from the stellar particle.

We assume that massive stars with $M>8~\rm M_\odot$ end their lives as SNII, corresponding to $n_{\rm SNII} = 1.18\times 10^{-2}~\rm M_\odot^{-1}$ SNe II per unit stellar mass formed, each releasing $10^{51}~\rm erg$ of energy. Instead of a fixed SNII delay \citep[as in][]{schaye2015}, we calculate the expected number of SNII during each time step, $N_{\rm SNII}$, based on the \citet{portinari1998} lifetimes of individual stars within the SSP. 
%\begin{equation}
%    N_{\rm SNII} = \left\{
%    \begin{array}{lr}
%    n_{\rm SNII} m_{\star, \rm init} \dfrac{1-\alpha}{t_{\rm max}} \left( \dfrac{t}{t_{\rm max}}\right)^{-\alpha} & t_{\rm min} <t< t_{\rm max}, \\
%    0 & \text{otherwise},
%    \end{array}
% \right.
%\end{equation}
%where $t$ is the age of the star particle, $m_{\star, \rm init}$ its initial stellar mass, $\alpha=0.48$ is a constant determined by the IMF, $t_{\rm max} \approx 40~\rm Myr$ is the metallicity-dependent SNII delay time for a $8~\rm M_\odot$ star, whereas $t_{\rm min}\approx 3~\rm Myr$ is the life time of the most massive stars in our assumed SSP. 
To prevent numerical overcooling, we follow \citet{dalla-vecchia2012} and use the total energy from these SNe to heat a small number of gas particles by $\Delta T=10^{7.5}~\rm K$. Energy feedback from stars is implemented in stochastic, thermal and isotropic form as described in detail by \citet{chaikin2022}\footnote{In essence, we draw a ray in a random direction and select the SPH gas neighbour that has the smallest angular separation from this ray.}. 

Besides SNII, we also implement SNIa feedback. In clusters and their quenched BCGs, SNIa are considered the second most important energy source after AGN and may help quench the galaxy by heating gas at larger radii \citep[e.g.][]{ciotti2007}. In addition, they contribute significantly to the metal enrichment of the ICM \citep[e.g.][]{simionescu2015}. It is therefore important to prevent numerical overcooling of SNIa feedback --- a subtlety not considered in most simulations. We achieve this with the same implementation as described above for SNII feedback. In contrast to SNII, SNIa can occur long after star formation and the precise delay cannot be predicted theoretically because it depends on poorly constrained parameters such as the binary fraction and separation. We therefore take a statistical approach and sample the SNIa rate from a delay time distribution (DTD) in every time step. In general, the DTD can be written as $ \text{DTD}(t) = \nu \xi(t)$, where $\nu$ is the total number of SNIa per unit formed stellar mass and $\xi(t)$ is a function normalised to
\begin{align}
 \int\limits_0^{t_{\rm u}} \xi(t) \mathrm{d}t &= 1, \label{eq:DTDnorm}
\end{align}
where $t_{\rm u}$ is the age of the Universe\footnote{Because most DTDs do not converge up to infinity, it is a convention to integrate up to the age of the Universe, $t_{\rm u}$, instead.} \citep{maoz2012}. Most commonly, the DTD is assumed to follow a power law, i.e. $\xi(t) \propto t^{-\beta}$. We set the slope of the power law to $\beta=1.0$, as inferred from the cosmic SNIa rate both in the field and in clusters \citep[see][for reviews]{maoz2012b, maoz2014}. Furthermore, we assume that SNIa have a fixed minimum delay time of $t_{\rm delay}=40~\rm Myr$ corresponding to the maximum lifetime of stars that explode as SNII. The properly normalised DTD is therefore given by
\begin{equation}
 \text{DTD}(t) = 
    \nu \frac{1}{\ln(t_{\rm u}) - \ln(t_{\rm delay})}
    t^{-1}\Theta(t-t_{\rm delay}).
\end{equation}
In contrast to the power-law slope $\beta$, the DTD normalisation $\nu$ is observed to differ significantly between the field and clusters. For the former, observations agree very well on a value of $\nu = 1.2\times 10^{-3} \; \rm M_\odot^{-1}$\citep{maoz2011, maoz2012, graur2011, perrett2012, frohmaier2019, strolger2020}, whereas a higher value of $\nu = 4\times 10^{-3} \;\rm M_\odot^{-1}$ is preferred by both observations of SNIa in galaxy clusters \citep{maoz2010b, maoz2012b, freundlich2020, strolger2020} and cluster iron abundances \citep{maoz2010}. Because we are simulating massive haloes, we adopt the latter value in this work.

\begin{table*}
\begin{center}
\caption{Simulation parameters. From left to right, we list the dark matter halo mass within apertures $R_{200}$, $R_{500}$, and $R_{2500}$ and the corresponding radii; 
  the initial black hole mass, $M_{\rm BH}$;
  the stellar-to-halo mass ratio $M_{\star}/M_{\rm h}$; 
  stellar scale length $r_\star$; 
  concentration of the dark matter halo, $c$, based on \citet{correa2015};
  gas fraction within $R_{500}$, $f_{500}$;
  virial temperature at $R_{500}$, $k_{\rm B} T_{500}$;
  virial entropy at $R_{500}$, $K_{500}$; 
  the fiducial imposed central initial temperature, $T_{0,\rm fid}$.
  }
\label{tbl:extra_params}
\begin{tabular}{cccclcccccclcl}

\hline
   $\log_{10} M_{200}$ & $\log_{10} M_{500}$ & $\log_{10} M_{2500}$ & $R_{200}$ & $R_{500}$ & $R_{2500}$ & $\log_{10} M_{\rm BH}$ & $M_{\star}/M_{\rm 200}$ & $r_\star$ & $c$ & $f_{\rm gas, 500}$ & $k_{\rm B} T_{500}$ & $\log_{10} K_{500}$ & $T_{0,\rm fid}$\\
                $\rm M_\odot$  & $\rm M_\odot$& $\rm M_\odot$ & $\rm kpc$ & $\rm kpc$ & $\rm kpc$ & $\rm M_\odot$         &     & $\rm kpc$ & &  &            $\rm keV$ & $\rm keV~\rm cm^2$  & $\rm K$ \\
\hline 
   13.0 & 12.89 & 12.62 & 443 & 305 & 143 & 8.4 & 0.01 & 4.5 & 7.2 & 0.016 & 0.34 & 1.78 & 0 \\

   13.5 & 13.37 & 13.09 & 650 & 438 & 205 & 8.6 & 0.005 & 5.0 & 6.4 & 0.037 & 0.7 & 2.09 & $10^{6.5}$\\

   14.0 & 13.88 & 13.56 & 955 & 651 & 294 & 8.8 & 0.0025 & 6.5 & 5.6 & 0.045 & 1.6 & 2.43 & $10^7$
\end{tabular}
\end{center}
\end{table*}

\subsection{Black holes and AGN feedback}
Finally, our simulations model the growth of supermassive BHs and the associated energy feedback (AGN feedback). Since we are simulating an idealised halo, with a single BH, we fix its position explicitly to the centre of the dark matter halo. This is because even at our comparatively high resolution, our simulations do not properly resolve the processes (such as dynamical friction) that determine the motion of the BH \citep[e.g.][]{tremmel2017, bahe2021}. 

Instead of modeling gas accretion with the standard Bondi-Hoyle approach, we use a modification that accounts for supersonic turbulence around the BH. The accretion rate is given by,
\begin{align}
    \dot{m}_{\rm accr, turb} &= 4 \pi \rho G^2 \frac{m_{\rm BH}^2}{c_{\rm s}^3} \left[ \frac{\lambda^2 + \mathscr{M}^2}{(1+\mathscr{M}^2)^4}\right]^{1/2},
\end{align}
with $\lambda= 1.1$ and Mach number $\mathscr{M}=v/c_{\rm s}$, where $v$ and $c_{\rm s}$ are the bulk velocity and (SPH-smoothed) sound speed of the gas surrounding the BH \citep{krumholz2006, ruffert1994}. This expression reduces to the Bondi-Hoyle accretion rate for $\mathscr{M}\ll 1$, but for highly supersonic gas flows around the BH ($\mathscr{M} \gg 1$), the accretion rate is suppressed by a factor $\mathscr{M}^{-3}$. 

When the gas flow around the BH is vorticity-dominated, we instead use the BH accretion rate of \citet{krumholz2005},
\begin{align}
    \dot{m}_{\rm accr, ang} &= \frac{4 \pi \rho (Gm_{\rm BH})^2}{c_{\rm s}^3} 0.34 f(\omega_\star),
\end{align}
where $\omega_\star = \omega r_{\rm B} / c_{\rm s}$, $r_{\rm B} = G m_{\rm BH}/c_{\rm s}^2$ is the Bondi radius, $\omega = |\nabla \times \mathbf{v}|$ is the vorticity of the ambient gas and the function $f(\omega_\star)$ is given by $f(\omega_\star) = (1+\omega_\star^{0.9})^{-1}$. To combine these two approaches, we interpolate the accretion rate between them as
\begin{align}
    \dot{m}_{\rm accr} &= \left( \dot{m}_{\rm accr, turb}^{-2} + \dot{m}_{\rm accr, ang}^{-2} \right)^{-1/2}.
\end{align}
The gas accretion rate is limited to the Eddington rate,
\begin{align}
    \dot{m}_{\rm accr} &= {\rm min}\left(\dot{m}_{\rm accr}, \dot{m}_{\rm Edd} \right),
\end{align}
where
\begin{align}
    \dot{m}_{\rm Edd} &= \frac{4 \pi G m_{\rm BH} m_{\rm p}}{\epsilon_{\rm r} \sigma_{\rm T} c} = 2.218 ~{\rm M_\odot} \; {\rm yr^{-1}} \left( \frac{m_{\rm BH}}{10^8 ~\rm M_\odot} \right).
\end{align}
Here, $\sigma_{\rm T}$ is the Thomson cross-section, $\epsilon_{\rm r}=0.1$ is the assumed radiative efficiency of the accretion disk \citep{shakura1973} and $c$ is the speed of light. 

The mass growth of the BH is then given by
\begin{align}
    \dot{m}_{\rm BH} &= (1 - \epsilon_{\rm r}) \dot{m}_{\rm accr},
\end{align}
while the rest of the accreted mass is radiated away (see below). The mass gain of the BH during a time step $\Delta t$ is therefore
\begin{align}
    \Delta m_{\rm BH} =  (1-\epsilon_r)\dot{m}_{\rm accr} \Delta t.
\end{align}
To conserve the total mass of our simulation (aside from radiative losses), we follow \citet{bahe2021} and remove small amounts of mass from neighbouring gas particles at each time step, as long as this would not reduce the gas particle mass below half their initial mass\footnote{Since the position of the BH is fixed in our simulation, we do not transfer momentum from gas particles to the BH, which leads to an (insignificant) violation of momentum conservation.}.

AGN feedback is implemented based on \citet{booth2009}. The amount of energy available for AGN feedback is given by
\begin{equation}
    \dot{E}_{\rm BH } = \epsilon_{\rm f} \epsilon_{\rm r} \dot{m}_{\rm accr} c^2 = 1.787 \times 10^{56} {~\rm erg ~\rm Myr^{-1}} \left( \cfrac{\dot{m}_{\rm accr}}{10^{-2}~\rm M_\odot ~\rm yr^{-1}} \right), 
\end{equation}
where we assume $\epsilon_{\rm f}=0.1$ for the coupling coefficient of the AGN energy to the ambient gas. In each time step, the energy released to the surrounding gas is stored in an (initially empty) reservoir $E_{\rm BH, res}$ in which this energy is accumulated until it reaches a threshold $E_{\rm heat}$. The latter corresponds to the energy required to heat a single gas particle by $\Delta T=10^{8.5}~\rm K$. Such a high heating temperature is needed to prevent numerical overcooling. At this point we determine the largest integer number $N$ of gas particles that can be heated by $\Delta T$, which may be $>1$ if the BH has accreted substantial mass in the current time step (but see below). The same procedure as for SN feedback is used to select the particles to heat. The energy used to heat them is then subtracted from the energy reservoir. 


In order to accurately follow the accretion of gas onto the BH, we want to avoid artificially delaying the onset of AGN feedback through too long time steps. We therefore use an additional time step limiter for the BH to prevent an excessive build-up of energy in its reservoir,
\begin{align}
    \Delta t_{\rm BH, accr} &= \frac{E_{\rm heat}}{\dot{E}_{\rm BH}} =  \frac{k_{\rm B} \Delta T_{\rm AGN} m_{\rm gas}}{(\gamma - 1) \mu m_{\rm H} \epsilon_{\rm f} \epsilon_{\rm r} \dot{m}_{\rm accr} c^2}. \label{eq:timestep1}
\end{align}
In other words, at a constant accretion rate $\dot{m}_{\rm accr}$ the energy reservoir should gain at most $E_{\rm heat}$ (the energy needed to heat one gas particle) during the BH time step. However, in particular for simulations of more massive haloes than presented here, very high accretion rates (and hence $\dot{E}$) could require unacceptably small time step ($t \approx 50~\rm yr$ and $t \approx 10~\rm yr$ for $10^{8.8}~\rm M_\odot$ and $10^{9.5} ~\rm M_\odot$ BHs accreting at the Eddington limit, respectively). To prevent such very small time steps, $\Delta t_{\rm BH, \rm accr}$ is restricted to a minimum of $\Delta t_{\rm BH, \rm accr}=100~\rm yr$.


 
\subsection{Simulation runs}
For each of the three different halo masses ($10^{13}~\rm M_\odot$, $10^{13.5}~\rm M_\odot$ and $10^{14}~\rm M_\odot$), we run a suite of simulations that keep the parameters listed in Table \ref{tbl:extra_params} fixed, but adopt different values of the initial central temperature $T_0$. For the $10^{13}~\rm M_\odot$ halo we run five simulations ($T_{\rm 0}=\{ 0, 10^{5.5}, 10^6, 10^{6.5}, 10^{6.7}\}~\rm K$, and four each for $10^{13.5}~\rm M_\odot$ ($T_{\rm 0}=\{ 10^{6}, 10^{6.5}, 10^{6.75}, 10^7 \}~\rm K$) and $10^{14}~\rm M_\odot$ ($T_{\rm 0}=\{ 10^{6.5}, 10^{6.75}, 10^{7}, 10^{7.25}\}~\rm K$). To study the long-term evolution of galaxy clusters each simulation is run for $8~\rm Gyr$, which is approximately equal to the time between $z=1$ and $z=0$.



==> Paper idealised elliptical/timescales.tex <==
\subsubsection{gas timescales}

The gas has several different time scales, the shortest time scale in general is the flow time scale that is the time that it takes gas to reach the centre with their current velocity:
\begin{equation}
 t_\text{flow} = \frac{r}{|\vec{v}|}.
\end{equation}
In which $r$ is the distance to the centre of the cluster/galaxy and $\vec{v}$ is the velocity vector. After that we have that the cooling time is short and given by:
\begin{equation}
 t_\text{cool} = \frac{\frac{3}{2} n k_B T}{|\Lambda_\text{net}|}.
\end{equation}
In which $\Lambda_\text{net}$ is the netto cooling rate, $T$ the gas temperature and $n$ the number density. The dynamical time is given by:
\begin{equation}
 t_\text{dyn} = \frac{\sqrt{2} r}{\sqrt{G M_\text{encl}/r}}.
\end{equation}
In which $M_\text{encl}$ is the enclosed mass at the radius $r$. and the free fall time is given by:
\begin{align}
 t_\text{ff} &= \sqrt{\frac{3\pi }{32 G \rho}}, \\
 &= 145~{\rm Myr} \left( \frac{n_H}{0.1~\rm cm^{-3}} \right)^{-1/2}. 
\end{align}
In which $\rho$ is the gas density.

In the runs the different timescales seem to reach 1 Gyr and 100 Myr at radii of see Tab \ref{tab:gas-time}.
% Example table
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:gas-time}
    \begin{tabular}{l|c|c}
         Time scale & 1 Gyr & 100 Myr \\ \hline  
         Flow time & 10 kpc & 3 kpc \\
         cooling time & 30 kpc & 3 kpc \\
         Dynamical time & 200 kpc & 30 kpc \\
         Free fall time & 100 kpc & - \\
    \end{tabular}
\end{table}


\subsubsection{Time scales close to the black hole}
For the BH there are several time scales, the first is the Salpeter time scale which is the e folding time when the BH accretes at the Eddington limit, this timescale is given by:
\begin{align}
 t_{\rm{Salpeter}} = \frac{\epsilon_r \sigma_T c}{4 \pi G m_p} = 45 \text{Myr}. 
\end{align}
In the simulations that I did we do only occasionally for a short moment in time accrete close the to Eddington limit, so I think this timescale is not of significant importance for the runs. A short time scale that can be off interest is the time between different AGN heating events is given by:
\begin{align}
 \epsilon_f \epsilon_r \langle \dot{M}_\text{BH} \rangle t_\text{AGN heating} c^2 &= \frac{k_B \Delta T}{\gamma -1} \frac{m_{gas}}{\mu m_H} N_\text{target}, 
\end{align}
Which in physical values is given by:
\begin{align}
 t_\text{AGN heating} &= 70~\text{kyr} \left(\frac{\Delta T}{10^{8.5}~\text{K}}\right) \left( \frac{\langle \dot{M}_\text{BH} \rangle}{10^{-2.5~\text{M}_\odot / \text{yr}}} \right)^{-1} \left( N_\text{target} \right).
\end{align}
In terms of the eddington ratio:
\begin{align}
 t_\text{AGN heating} &= 10~\text{kyr} \left(\frac{\Delta T}{10^{8.5}~\text{K}}\right) \left( \frac{R_{\rm Edd}}{0.01} \right)^{-1} \left( \frac{m_{\rm BH}}{10^8 \rm M_\odot} \right)^{-1} \left( N_\text{target} \right).
\end{align}

We can also write it explicitly in terms of the density and temperature around the black hole, than we obtain:
\begin{align}
    t_\text{AGN heating} &= 1.5~\text{kyr} \left(\frac{\Delta T}{10^{8.5}~\text{K}}\right) \left( \frac{M_{BH}}{10^8~\rm M_\odot} \right)^{-2} \left( \frac{n_H}{0.1 \rm cm^{-3}} \right)^{-1} \\
    &~~ \left( \frac{T}{10^5~\rm K} \right)^{3/2} \left( N_\text{target} \right).
\end{align}

For BHs there are also other time scales of interest, small scale times are not resolved in our simulation. The timescale closest related to the BH is the Bondi-Hoyle time scale, given by:
\begin{align}
 t_\text{Bondi} = \frac{r_B}{c_s} = 420 \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-3} ~\text{Myr}. 
\end{align}
Similar we can define a Bondi-Hoyle radius as:
\begin{align}
    r_{\rm Bondi} &= \frac{GM}{c_s^2} = 3.0 ~\rm kpc \left( \frac{M_{\rm BH}}{10^8 \rm M_\odot} \right) \left( \frac{T}{10^4 \rm K} \right)^{-1}. 
\end{align}

In the case that the gas around the BH has supersonic velocities we need to use an other equation given by:
\begin{align}
 t_\text{Krumholz} = \frac{r_B}{(1+M_0^2) M_0 c_s} = 420 \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{(1+M_0^2) M_0 c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-3} ~\text{Myr}. 
\end{align}
This also implies that the Bondi-Hoyle radius is modified to:
\begin{align}
    r_{\rm Krumholz} &= \frac{GM}{(1 + M_0^2) c_s^2} = \frac{3.0 ~\rm kpc}{1 + M_0^2} \left( \frac{M_{\rm BH}}{10^8 \rm M_\odot} \right) \left( \frac{T}{10^4 \rm K} \right)^{-1}. 
\end{align}
This means that when there is turbulence the Bondi-Hoyle radius is decreased compared to the approach in which we do not take into account turbulence.

In the case of Gaspari type of feedback we have that we want to accrete enough mass to heat 1 particle the moment we a particle gets in our inner radius for which we accrete. This means that in order to heat 1 particle we need to nibble a mass of:
\begin{align}
    \epsilon_f \epsilon_r \Delta m_{\rm acc} c^2 &= \frac{k_B \Delta T}{\gamma -1} \frac{m_{gas}}{\mu m_H},
\end{align}
this reduces to:
\begin{align}
    \Delta m_{\rm acc} &= \frac{k_B T}{\gamma - 1} \frac{m_{\rm gas}}{\mu m_H \epsilon_f \epsilon_r c^2}, \\
    &= 726~\rm{M}_\odot \left( \frac{\Delta T}{10^{8.5}K} \right) \left( \frac{m_{\rm gas}}{10^{5} ~\rm M_\odot } \right) \left( \frac{\mu}{0.6} \right)^{-1}.
\end{align}

AGN:
\citet{rosas-guevara2015}, \citet{schaye2015}

The Eddington accretion rate is given by:
\begin{align}
    \dot{m}_{\rm Edd} &= \frac{4 \pi G m_{\rm BH} m_{\rm p}}{\epsilon_r \sigma_T c}, \\
    &= 2.218 ~\rm M_\odot \rm yr^{-1} \left( \frac{m_{\rm BH}}{10^8 ~\rm M_\odot} \right).
\end{align}

Bondi-Hoyle accretion\citep{bondi1944}:
\begin{align}
    \dot{m}_{\rm Bondi} &= \frac{4 \pi G^2 m_{\rm BH}^2 \rho}{(c_s^2 +v^2)^{3/2}}.
\end{align}

\begin{align}
    \dot{m}_{\rm BH} = (1-\epsilon_r) \dot{m}_{\rm accr}. 
\end{align}


\subsubsection{Time scales related to the disk around the BH}
The sound crossing time for the disk:
\begin{align}
 t_\text{cross} = 65 \text{Myr} \left( \frac{\mu}{0.6}\right )^{1/2} \left(\frac{T}{10^4 K}\right)^{-1/2} \left(\frac{d}{1 kpc}\right).
\end{align}
Disk consumption time scale is given by:
\begin{align}
 t_{\rm SFR} &= \frac{M_{\rm gas}}{SFR}, \\
 &= 10~{\rm Myr} \left( \frac{M_{\rm gas}}{10^8~\rm M_\odot} \right) \left( \frac{SFR}{10~ \rm M_\odot ~\rm yr^{-1}} \right)^{-1}.
\end{align}
\subsubsection{Time scales related to stars}
SNII time scale, the time scale within all SNII go off:
\begin{align}
    t_{\rm SNII} &= 30~\rm Myr.
\end{align}

\subsubsection{Angular momentum limiter related time scales}

The viscous Yetli time scale:
\begin{align}
 t_\text{visc} &= 420~ C_\text{visc} \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{V_\phi}{10~\text{km}~\text{s}^{-1}} \right)^3 \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-6} ~\text{Myr}, \\
 &= 2.6\cdot 10^6 \left(\frac{C_\text{visc}}{2\pi \cdot 10^3}\right) \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{V_\phi}{10~\text{km}~\text{s}^{-1}} \right)^3 \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-6} ~\text{Myr}.
\end{align}

A vorticity time scale for the Krumholz model:
\begin{align}
 t_\text{vorticity} &= \frac{1}{|\nabla \times \vec{v}|} = \frac{1}{\omega} = \frac{r}{\tilde{\omega} M_0 c_s}, \\
  &= 19.6 ~\text{Myr} \left( \frac{r}{10~\text{kpc}} \right) \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-1}\left( \frac{\tilde{\omega}}{10.} \right)^{-1}.
\end{align}
This has a corresponding length scale given by:
\begin{align}
    r_{\rm vorticity} =\frac{M_0 c_s}{|\nabla \times \vec{v}|}  &= 1.0~ \rm{kpc}\left( \frac{M_0}{5} \right) \left( \frac{r}{10~\text{kpc}} \right) \left( \frac{\tilde{\omega}}{10.} \right)^{-1}.
\end{align}

\subsubsection{When is gas gravitational bound?}
The total energy of the gas-BH system is given by:
\begin{align}
    E_{tot} &= E_{grav} + E_{kin} + E_{th}.
\end{align}
Filling in the equations we obtain:
\begin{align}
    E_{tot} &= - \frac{G M_{BH} m_{gas}}{r} + \frac{1}{2} m_{gas} v^2 + \frac{k_B T}{(\gamma - 1)} \frac{m_{gas}}{\mu m_H}.
\end{align}
In general gas is bound when we have $E_{tot} < 0$, which means that we obtain:
\begin{align}
    \sqrt{\frac{G M_{BH}}{r}} > \sqrt{\frac{k_B T}{(\gamma -1)\mu m_H} + \frac{1}{2}v^2}.
\end{align}
Which can be expressed as:
\begin{align}
    165~\rm km \rm s^{-1} \left( \frac{r}{100~\rm pc} \right)^{-1/2} \left( \frac{M_{BH}}{10^{8.8}~\rm M_\odot} \right)^{1/2} > \sqrt{95 ~\rm km^2 \rm s^{-2} \left(\frac{T}{10^4~\rm K} \right) + \frac{1}{2} v^2}. 
\end{align}
Which means that if we ignore the thermal term, we obtain:
\begin{align}
    v_{gas} < 230~\rm km \rm s^{-1} \left( \frac{r}{100~\rm pc} \right)^{-1/2} \left( \frac{M_{BH}}{10^{8.8}~\rm M_\odot} \right)^{1/2}
\end{align}
and in the case of thermal dominated we obtain:
\begin{align}
    T < \frac{G M_{BH} (\gamma -1) \mu m_H}{r k_B} = 2.85 \times 10^6 ~\rm K \left( \frac{M_{BH}}{10^{8.8}~\rm M_\odot} \right) \left( \frac{r}{100~\rm pc} \right)^{-1}.
\end{align}

What radius is the enclosed stellar mass smaller than the BH mass?
\begin{align}
    M_{\rm BH} > M_{\star} \frac{r^2}{(r_{\star}^2 + r^2)}.
\end{align}
This results in:
\begin{align}
    \left( M_{\star} - M_{\rm BH} \right) r^2 - 2 r r_\star M_{\rm BH} - M_{\rm BH} r_{\star}^2 < 0.
\end{align}
Which means that we obtain:
\begin{align}
    r < 2 r_{\star} \left( \frac{M_{\rm BH} \pm \sqrt{M_{\rm BH} M_{\star} }}{M_{\star} - M_{\rm BH}} \right).
\end{align}

==> cooling.tex <==
\subsection{How far can feedback compensate the cooling?}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_rate.png}
    \caption{Top: SFH of the $10^{14}~\text{M}_\odot$ halo with the BHAR and the injected energy. Bottom: The radii until which the AGN accretion, SNIa and SNII rate can compensate the cooling rate.}
    \label{fig:cooling-rate-vs-BHAR}
\end{figure}

In our simulation we have three sources of feedback, AGN, SNII and SNIa. We would expect that in general AGN feedback is the dominant source of feedback. Given that a large part of the evolution of the halos that we investigated is depending on the ineraction between the feedback and thermodynamic properties of the gas, we want to see until which radii feedback is able to compensate the cooling of gas. In Fig. \ref{fig:cooling-rate-vs-BHAR} we show the energy injection of all feedback channels (AGN, SNII, SNIa), we can clearly see in Fig. \ref{fig:cooling-rate-vs-BHAR} that the AGN feedback in almost all cases is the dominant source of feedback, however we can also see that when the AGN is not dominant, that the SNIa feedback is the most dominant source, the SNII feedback seems to barely dominate the AGN feedback but also seems to be an important source of feedback, but in general seems to follow the AGN energy injection rate quite closely, while the SNIa seems double the energy injected compared to an AGN only model, meaning that during episodes of low energy injection the energy injected by SNIa is helping the galaxy stay quenched slightly longer, besides this SNIa feedback is at larger radii because it comes from old stars, therefore heating gas that will start in-flowing.

If we look at the bottom plot of Fig. \ref{fig:cooling-rate-vs-BHAR}, we can see the radii until which the different feedback channels compensate the instantaneous cooling rate. We can see in Fig. \ref{fig:cooling-rate-vs-BHAR} that during episodes of high BHAR the AGN feedback can compensate the cooling way beyond the virial radius, we can see that in general when we look at the SNIa and SNII radius we can see that the maximum radius the SNe feedbacks reach is around $10~\rm kpc$, meaning it can only compensate for the cooling inside the galaxy or slightly outside of it, but is not really able to compensate the cooling rate from the CGM. In terms of the total impact on the CGM gas it is more interesting to look at the cumulative behaviour, in Fig. \ref{fig:cooling-rate-vs-BHAR-cum} we show the cumulative behaviour. We can see in FIg. \ref{fig:cooling-rate-vs-BHAR-cum} that the AGN will only after a time of around $2~\rm Gyr$ starts to be close to compensating the cooling until a radii of around $30~\rm kpc$, which seems to be consistent with the fact that the AGN is mainly regulating the thermodynamic cycle and compensating low values of heating. In Fig. \ref{fig:cooling-rate-vs-BHAR-cum} we can also see that the cumulative behaviour for both the the SNIa and SNII only can compensate the cumulative cooling rate up to radii of around $6$ - $10~\rm kpc$, which confirms the idea that SNIa and SNII mainly are able to compensate the cooling just in the galaxy.  

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_rate_cumulative2.png}
    \caption{Top: SFH of the $10^{14}~\text{M}_\odot$ halo with the BHAR and the injected energy. Bottom: The radii until which the AGN accretion, SNIa and SNII rate can compensate the cumulative cooling rate.}
    \label{fig:cooling-rate-vs-BHAR-cum}
\end{figure}




==> observation_comp.tex <==
\subsection{Comparison with observations of cool gas}

\subsubsection{Relation between the amount of cold gas and thermodynamic properties}

Observations indicate that the amount of cold gas in clusters similar to our $M_{200}=10^{14}~\rm M_\odot$ is smaller than $4\cdot 10^{10}~\rm M_\odot$ \citep[e.g.][and other works]{edge2001, salome2003, pulido2018}. Moreover, the large variation in the amount of molecular gas in galaxy clusters indicates that the cold gas content of a galaxy cluster should not be constant in time but should vary over at least two orders of magnitude. In Fig. \ref{fig:thermoproperties-comparison} we show the evolution of the cold gas mass for our fiducial simulations. We can see that the amount of cold gas varies from $10^{7}~\rm M_\odot$ to $10^{10}~\rm M_\odot$, which is in a good agreement with the observations at the same halo mass. \citet{pulido2018} found that they are only able to detect molecular gas when they detect a CC cluster that either has a central cooling time $t_{\rm cool} \lesssim 1~\rm Gyr$ or a central entropy profile $K \lesssim 35~\rm cm^2 ~\rm keV$. They however do not detect any clusters with a molecular mass below $10^8~\rm M_\odot$. Fig. \ref{fig:thermoproperties-comparison} shows that when the cooling time is short, the amount of cold gas is large. When the cooling time is larger than $1~\rm Gyr$, the cold gas mass is below $10^8~\rm M_\odot$, in agreement with the findings of \citet{pulido2018}. Similarly, when the entropy falls below  $35~\rm cm^2 ~\rm keV$ the cold gas mass is above $10^8~\rm M_\odot$, which shows that our simulations agree well with \citet{pulido2018}.

\subsubsection{Clumpy structure of the ISM}

In Fig. \ref{fig:clumpy-temperature} we show the temperature distribution in the inner $15~\rm kpc$ of the $M_{200}=10^{14}~\rm M_\odot$ halo at four different times, separated by 100$~\rm Myr$, around one of the peaks in the SFR. We can see that the simulations predict a filamentary and clumpy multiphase medium in the centre of the BCG. Although the average temperature of the gas is between $10^7$ to $10^{7.5}~\rm K$, a large amount of gas has temperatures below $10^6~\rm K$. Most of the gas with $T\la 10^6~\rm K$ quickly cools to our imposed entropy floor, corresponding to have temperatures below $10^4~\rm K$. While we do not attempt in this paper to reproduce H$\alpha$ or CO observations, we note that the main filamentary structures of the cool gas can be observed in H$\alpha$ but only the densest clumps will have substantial CO emission, in qualitative agreement with observations (e.g. \citealt{olivares2019}; \citealt{russell2019})

\begin{figure}
    \centering
	\includegraphics[width=.7\columnwidth]{./images/temp_evolution_close_single_0054.pdf}
    \caption{Mass-weighted temperature distribution in the inner $15~\rm kpc$ of the $M_{200}=10^{14}~\rm M_\odot$ halo. The cold gas in the centre of the halo is similar to filamentary structures observed.}
    \label{fig:clumpy-temperature}
\end{figure}


==> old.tex <==
\begin{comment}
To summarize, based on the central temperature in the galaxy cluster we can determine whether the central galaxy while get a star burst, start quenched but gets star forming after a certain time or remains quenched for eternity. This mainly dependents on the cooling time and the $t_{\rm cool}/t_{\rm dyn}$-ratio. To illustrate this further we do a set of simulations in which we re-scaled the cooling rate by $0.2$ and $0.4$ dex up and down in order to see the impact on the star forming history, in Fig. \ref{fig:cooling-rate} we show the cooling time and $t_{\rm cool}/t_{\rm dyn}$-ratio for the modified cooling rate runs. We can see in this figure that the cooling rate for the none-modified cooling rate results in an initial $t_{\rm cool}/t_{\rm dyn}$-ratio that is very close to 10. We can see that when we increase the cooling rate that we get a lower ratio, while for a lower cooling rate we get a higher ratio. As based on the previous result we would expect that the runs with a higher cooling rate will start forming stars earlier. If we look at Fig. \ref{fig:SFH-rate} it seems that indeed the SFH seems to change as expected.
\end{comment}

\section{How is star formation regulated?}
In this section we will take a closer look at the exact way in which star formation and properties of the CGM play together. To understand this we divide star formation in different episodes shown in Fig. \ref{fig:cycle-criterion}, to summarize the different phases are:
\begin{enumerate}
    \item The rapid increase of the SFR.
    \item The flattening of the SFH.
    \item The initial decline of the SFR.
    \item The persistent decline of the SFR.
\end{enumerate}
We define the phases based on the time at which we determine the boundary between the different phases. We firstly detect peaks in the 50 Myr smoothed SFH using \texttt{scipy.signal.find\_peaks}, using this we select only broad and peaks above a SFR of:
\begin{align}
    \log {\rm SFR} = \log {\rm sSFR}_{\rm quenched} \times M_\star -1.5.
\end{align}
Based on finding all the peaks with widths above 500 Myr we are able to determine the peak of the SFH, based on the peaks of the SFH we look than for the 50 Myr smoothed minimum or first time the galaxy reaches a SFR below $10^{-3}~ \rm M_\odot ~ \rm yr^{-1}$. This gives us the end of phase iv or the start of phase i. Than we are interested in other separation of phases, we do this by finding the time at which the 50 Myr smoothed SFH goes below a factor of e compared to the SFH at the peak. We use the 50 Myr smoothed star formation instead of the instantaneous star formation because the 50 Myr smoothed SFH is fluctuating less on very short times, given that we are mainly interested on the long timescale, small timescale fluctuations are not of uttermost interest.

\begin{comment}
\begin{figure}
	\includegraphics[width=\linewidth]{./images/cycle_criterion.png}
    \caption{The division of an episode of star formation in different phases. (i) the phase of rapid increas of the SFR. (ii) The flattening of the SFH. (iii) The initial decline of the SFR. (iv) the persistent decline of the SFR.}
    \label{fig:cycle-criterion}
\end{figure}
\end{comment}

\begin{enumerate}
    \item
    \item In Fig. \ref{fig:cooling-ratio} we can see that in the centre when the cooling time 
\end{enumerate}

\subsection{Central thermal feedback and short cooling times}
 In Fig. \ref{fig:cooling-time} we can see that the cooling time reaches a maximum of around $1~\rm Gyr$ and at larger radii it does not necessary reach even $1~\rm Gyr$. This is different from what \citet{voit2017} claims thermal feedback is able to do, they claim thermal feedback will always cause the gas in the centre to be above several Gyr, which is worse than what thermal feedback will produce. 




\subsection{Central thermal feedback can regulate the ambient medium}
In Fig. \ref{fig:cooling-ratio} we can see that the $t_{\rm cool}/t_{\rm dyn}$-ratio decreases below an episode of star formation and increases again after an episode and star formation and the corresponding BHAR. But in general we can see that when the ratio is around  $t_{\rm cool}/t_{\rm dyn} \approx 10$ the galaxy is quenched, this basically means that the $t_{\rm cool}/t_{\rm dyn}$-ratio of the CGM is regulated to a value of around $t_{\rm cool}/t_{\rm dyn} \approx 10$. 







\subsection{Entropy profiles behave as expected}
In Fig. \ref{fig:entropy-comparison} we can see that the entropy evolution seems to behave as expected:
\begin{enumerate}
    \item Entropy decreases isentropic with the same cooling rate
    \item The central core of the entropy becomes lower due to precipitation
    \item The entropy in the CGM increases after an episode of AGN feedback/SF
\end{enumerate}







\subsection{Which resolution is required to resolve the precipitation behaviour?}
\begin{itemize}
    \item How does the resolution impact the SFH, see Fig. \ref{fig:SFH-res}
    \item SFH is converged until a certain resolution
    \item Entropy profiles
\end{itemize}

\begin{figure*}
	\includegraphics[width=\linewidth]{./images/SFH_res.png}
    \caption{SFH for the $10^{13}~\rm M_\odot$ and $10^{14}~\rm M_\odot$ halo at different resolutions}
    \label{fig:SFH-res}
\end{figure*}

\subsection{The impact of random numbers}
In Fig. \ref{fig:SFH-seed} we can see that having an identical setup but different random events of AGN feedback and SNe feedback can cause significant different time evolution, in terms of the size of the peaks of SFH, they differ also the exact time difference differs, but the trend between entropy and the SFH do not differ. Meaning the exact behaviour is consistent with precipitation but the exact timing is a bit hard to predict.

\begin{figure*}
	\includegraphics[width=\linewidth]{./images/entropy_comparison_seed.png}
    \caption{SFH for the $10^{14}~\rm M_\odot$ halo and the entropy at different radii for different random number seeds.}
    \label{fig:SFH-seed}
\end{figure*}



\subsection{What drives the oscillations in the SFH?}
In the case of a galaxy cluster with a halo mass of $10^{13}~\rm M_\odot$ we can see in Fig. \ref{fig:SFH-13} that the BH is either able to quench an initial star burst phase or puts so much energy in the CGM that the galaxy will stay quenched for always. However for more massive halo masses we can see in Fig. \ref{fig:SFH-135} and \ref{fig:SFH-14}, that both a galaxy cluster with a halo mass of $10^{13.5}$ and $10^{14}~\rm M_\odot$ do not remain quenched, but rather have episodes of high star formation followed by episodes of low star formation. In the case of having periods we want to understand what sets the periods in the SFH. Continueing on the approach in the previous section we expect that the cooling time and the corresponding $t_{\rm cool}/t_{\rm dyn}$-ratio are important in setting in which phase we are in the quenched-non-quenched evolution. In general we can divide the SFH cycle in four different phases:
\begin{enumerate}
    \item The pre-SFH phase: During this phase the SFH goes below the quenched criteria and continues to become lower due to AGN feedback.
    \item The onset of SFH phase: During this phase the SFH starts increasing very rapidly but the SFH is still quenched. 
    \item The flatting of the SFH phase: During this phase the SFH starts to flatten and reaches the maximum SFH during this cycle. 
    \item The quenching SFH phase: During this phase the AGN heats the gas around the BH causing the SFH to start to decrease and goes below the quenching threshold.
\end{enumerate}
In Fig. \ref{fig:volume-cooling-time} we can see that the cooling time and $t_{\rm cool}/t_{\rm dyn}$-ratio are different for the various phases of the star formation cycle. We see that during the pre-SFH phase the cooling ratio just outside of the galaxy is already significantly below a $t_{\rm cool}/t_{\rm dyn}$-ratio of 10. This means that the gas will cool down on the cooling time scale and will flow inwards with the dynamical time entering the onset of SFH phase, after a very short time around $100~\rm Myr$ later the galaxy already surpasses the quenching criterion, because the galaxy at this point even has a lower $t_{\rm cool}/t_{\rm dyn}$-ratio, a further increase of the SFH cannot be prevented, this means that the galaxy enters the flattening of the SFH phase, at the end of this phase the SFH reaches the peak of this cycle and also the $t_{\rm cool}/t_{\rm dyn}$-ratio will be the lowest in the center, this is followed by the quenching phase in which the AGN feedback reduces the cold gas in the galaxy significantly causing the gas in the galaxy to be very hot and having very large cooling times, with a corresponding very large $t_{\rm cool}/t_{\rm dyn}$-ratio in the centre. However the AGN is not able to increase the $t_{\rm cool}/t_{\rm dyn}$-ratio a lot at large radii ($r>30~\rm kpc$), this means that gas is able to cool down at these radii at the cooling time scale which is around $1~\rm Gyr$. After this we enter the pre-SFH phase during which the SFH still gets lower due to AGN feedback, this phase will take around the time it takes for gas to cool down at the radii that were not influenced by AGN feedback.

How long do we expect the different phases of the SFH cylce to take? Purely based on Fig. \ref{fig:volume-cooling-time}, we understand how long the pre-SFH phase and the onset of SFH phase take, they are directly related to the cooling time of the gas with the lowest $t_{\rm cool}/t_{\rm dyn}$-ratio. However for the two other phases the time of these phases are a bit more difficult because they are not solely based on the cooling time but are highly depending on the exact amount of gas that inflows and the exact amount of energy in feedback that is injected in the cold gas. We will first start with the phases in which the SFH decreases. In this phase we can ignore that new gas is cooling down and the only source of feedback is AGN, which mainly heats the cold gas, this means that the evolution of the cold gas is described by:
\begin{align}
     \frac{\rm d M_{\rm cold gas}}{\rm d t} &= -R_{\rm AGN}.
\end{align}
In which $R_{\rm AGN}$ is the mass rate that is heated by AGN feedback, which is given by:
\begin{align}
    R_{\rm AGN} &= \alpha \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm AGN}} \epsilon_f \epsilon_r {\rm BHAR}(t) c^2.
\end{align}
In which $\alpha$ is a factor of order unity, which means when it is unity that only the gas particles that are heated are decreasing the cold gas mass, but if it is higher than unity it means that a fraction of the gas is also heated due to secondary ways (e.g. shocks or conduction). In general the BHAR and the cold gas mass are not directly related to each other. But in the simulation it seems that the cold gas mass and the BHAR are related to each other to something like:
\begin{align}
    \rm BHAR(t) &= \epsilon_{\rm gas-BHAR} \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right). 
\end{align}
In which $\epsilon_{\rm gas-BHAR}$ is the relation factor that is between 10\% to 0.1\%. Combining the above relations means that we can calculate the e-folding time for the AGN feedback as:
\begin{align}
    t_{\rm AGN} &= \frac{k_B T_{\rm AGN} \cdot 10^9}{\alpha (\gamma -1)\mu m_H \epsilon_f \epsilon_r \epsilon_{\rm gas-BHAR} c^2} \rm yr, \\
    &= 440 ~\rm Myr \left( \frac{T_{\rm AGN}}{10^{8.5}~\rm K} \right) \left( \frac{\alpha \epsilon_{\rm gas-BHAR}}{0.01} \right)^{-1}. \label{eq:e-folding}
\end{align}
Looking at Fig. \ref{fig:cooling-dyn-ratio}, we can see that in the SFH cycle that starts at $2\rm Gyr$, that the e-folding time in the decreasing SFH phase has 3 different slopes, the first phase is starting with a BHAR that is more than 2 orders lower, meaning the e-folding time is around $700\rm Myr$ (following Eq. (\ref{eq:e-folding})), while in the central second phase the BHAR is much higher than $0.01$ and therefore e-folding times decrease to shorter times around $200~\rm Myr$, while after that the e-folding times is around $300~\rm Myr$. This means that the BHAR is important in determining how quick the SFH decreases. 


However the BHAR is not the only thing that determines the exact slope of the decreasing SFH. It is also important to realize that the factor $\alpha$ needs to play some role in setting how fast the SFH decreases, because only based on the BHAR is not enough. This means that gas that is heated also needs to take away part of the gas that is not directly heated by AGN feedback. Especially during episodes of high star formation, the secondary heating of gas is not important because gas that is heated secondary will have severe over-cooling.  In general the density at which thermal feedback is efficient is given by (following Eq. (18) of \citet{dalla-vecchia2012}):
\begin{align}
    n_{H,t_c} &= 23~\rm cm^{-3} \left( \frac{T}{10^{7.5}\rm K} \right)^{3/2} \left( \frac{\langle m \rangle}{10^5 \rm M_\odot} \right)^{-1/2}.
\end{align}

The flattening of the SFH phase is partly chaotic instead of purely determined by timescales, instead of gas falling completely to the center, it is possible that the gas starts forming a stable ring, that is rotating around the BH, keeping the density around the BH low causing a lower BHAR that takes longer for the galaxy to heat the cold gas, at the same time the formation of a disk also means that more gas can form stars while keeping the ring away from the BH. 

\begin{comment}
\subsection{The entropy and the $t_{\rm cool}/t_{\rm dyn}$-ratio}
\begin{itemize}
    \item Entropy is to some way related to the $t_{\rm cool}/t_{\rm dyn}$-ratio, but it seems to be more related to the amount of energy that is injected by feedback.
\end{itemize}

\subsection{The X-ray luminosity}
\begin{itemize}
    \item Small radii are only changing (r<30 kpc)
    \item Higher $t_{\rm cool}/t_{\rm dyn}$ means that the run has a lower X-ray luminosity in the centre. 
\end{itemize}

\subsection{Until which radii can feedback influence the CGM?}
\begin{itemize}
    \item Fig. \ref{fig:coupling:BHARandSFR}
    \item Figure of the cumulative radii, would be interesting
\end{itemize}

\subsection{What is the impact of different realizations of the same galaxy?}
\begin{itemize}
    \item Similar periods?
\end{itemize}
\end{comment}


\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_episodes_of_SFH_mass_weighted.png}
    \caption{Top: Mass weighted cooling time for different phases of the SFH cycle of the galaxy. Bottom: The mass weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_and_entropy_episodes_of_SFH_mass_weighted.png}
    \caption{Top: Mass weighted entropy profile for different phases of the SFH cycle of the galaxy. Bottom: The mass weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_and_Xray_lum_episodes_of_SFH.png}
    \caption{Top: X-ray profile for different phases of the SFH cycle of the galaxy. Bottom: The mass weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_and_Xray_flux_episodes_of_SFH.png}
    \caption{Top: Volume weighted entropy profile for different phases of the SFH cycle of the galaxy. Bottom: The volume weighted $t_{\rm cool}/t_{\rm dyn}$-ratio for different phases of the SFH cycle of the galaxy.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/SFH_cooling_time_volume.png}
    \caption{The SFH compared with the cooling time at different radii.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/SFH_cooling_time_over_dynamical_time_volume.png}
    \caption{The SFH compared with the $t_{\rm cool}/t_{\rm dyn}$-ratio at different radii.}
    \label{fig:SFH-14}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/SFH_entropy_volume_weighted.png}
    \caption{The SFH compared with the entropy at different radii.}
    \label{fig:SFH-14}
\end{figure}

\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/cooling_time_M14_Lambda_dex.png}
    \caption{Top: the cooling time for the $10^{14}~\rm M_\odot$ halo based on the central temperature. Bottom: the $t_{\rm cool}/t_{\rm dyn}$-ratio for the $10^{14}~\rm M_\odot$ halo based on the central temperature.}
    \label{fig:cooling-rate}
\end{figure}


\begin{figure}
	\includegraphics[width=\columnwidth]{./images/Lambda_change.png}
    \caption{SFH of the $10^{14}~\text{M}_\odot$ halo with different cooling rates}
    \label{fig:SFH-rate}
\end{figure}
\end{comment}

\end{comment}

\begin{comment}
A closer look at Fig. \ref{fig:SFH-rate}, lets us realize that the cooling rate is not only important in setting when the initial burst of star formation will take place, but also is important in setting the oscillatory behaviour of the simulation. If we change the cooling rate, this will inversely change the cooling time, so a smaller cooling rate by 0.4 dex, will increase the cooling time by a factor of 0.4 dex. This means that a smaller cooling rate will imply that the same timescales will be at smaller radii. Given that a change in the cooling rate will not influence the dynamical time, this means that the $t_{\rm cool}/t_{\rm dyn}$-ratio will increase at all radii, which means that the radius at which the ratio is around 10, will move inwards (or will even stay above 10).  This will imply a few things:
\begin{enumerate}
    \item The total gas that is within the radius at which we have a  $t_{\rm cool}/t_{\rm dyn}$-ratio of 10 is smaller if the cooling rate is smaller and larger if the cooling rate is larger. Therefore runs that have a smaller cooling rate only have a smaller amount of gas accessible for star formation, this means peaks in star formation will be smaller.
    \item Given that the radius at which the $t_{\rm cool}/t_{\rm dyn}$-ratio is 10 is smaller, this also means that the dynamical time within this region is smaller, therefore the maximal oscillation time in simulations with a smaller cooling rate will be shorter and longer if the cooling rate is larger. 
\end{enumerate}

But this basically only explains half of the picture, after the first burst the SFR decreases due to feedback which is not directly related to the cooling time. In the top panel of Fig. \ref{fig:cooling-dyn-ratio} we show the SFH, BHAR and gas mass and see that the gas mass and SFH are almost perfectly correlated, implying the amount of cold gas sets the SFR, this means that the amount of cold gas needs to decrease. In order to decrease the amount of cold gas we need to look at the impact of the feedback on the cold gas. In general the evolution of cold gas can be described by:
\begin{align}
    \frac{\rm d M_{\rm cold gas}}{\rm d t} &= -R_{\rm AGN} - R_{\rm SNII} - R_{\rm SNIa} - SFR + R_{\rm cooling}. \label{eq:rates}
\end{align}
In which $R_{\rm i}$ with $i=(\rm AGN, \rm SNII, \rm SNIa)$ are the mass rates for the different components and $R_{\rm cooling}$ is the inflow of cold gas produced by cooling. Based on this we can see that the source of a decrease of the amount of cold gas is mainly AGN feedback given that the amount of energy available in SNII and SNIa are lower than in AGN feedback. Based on Fig. \ref{fig:cooling-dyn-ratio} the BHAR can be roughly described as:
\begin{align}
    \rm BHAR(t) &= \epsilon_{\rm gas-BHAR} \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right). \label{eq:BHAR}
\end{align}
In which $\epsilon_{\rm gas-BHAR}$ is a constant close to $0.01$, but in the case of the BHAR, this constant seems to be time dependent, but for now we assume it to be around constant. The mass heating rate of the AGN is given by:
\begin{align}
    R_{\rm AGN} &= \frac{(\gamma - 1) \mu m_H}{k_B T_{\rm AGN}} \epsilon_f \epsilon_r {\rm BHAR}(t) c^2,
\end{align}
In which $T_{\rm AGN}$ is the average temperature to which the AGN needs to heat the gas in order for the gas to produce outflows and remove the cold gas from the center, filling in Eq. (\ref{eq:BHAR}) we obtain:
\begin{align}
    R_{\rm AGN} &= \frac{(\gamma - 1) \mu m_H}{k_B T_{\rm AGN}} \epsilon_f \epsilon_r c^2 \epsilon_{\rm gas-BHAR} \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 } \right).
\end{align}
Ignoring the SNIa and SNII feedback, we obtain an e-folding timescale for the cold gas of around:
\begin{align}
    t_{\rm AGN} &= \frac{k_B T_{\rm AGN} \cdot 10^9}{(\gamma -1)\mu m_H \epsilon_f \epsilon_r \epsilon_{\rm gas-BHAR} c^2} \rm yr, \\
    &= 440 ~\rm Myr \left( \frac{T_{\rm AGN}}{10^{8.5}~\rm K} \right) \left( \frac{\epsilon_{\rm gas-BHAR}}{0.01} \right)^{-1}.
\end{align}
In general when the SFH is very high, this also translates to very high densities in the center of the galaxy, this means that low injection temperatures in the high density cold gas will produce drastic overcooling. In order to overcome this, the gas needs to be heated to sufficiently high average temperatures. The overcooling of feedback is given by Eq. (18) of \citet{dalla-vecchia2012}, which in simplified form is given by:
\begin{align}
    n_{H,t_c} &= 23~\rm cm^{-3} \left( \frac{T}{10^{7.5}\rm K} \right)^{3/2} \left( \frac{\langle m \rangle}{10^5 \rm M_\odot} \right)^{-1/2}.
\end{align}
This means that for SNe feedback we will already have a problem of overcooling at a density of $n_{H,t_c}=23~\rm cm^{-3}$, this implies that when we have a high density in the galaxy, SNe feedback will not help in quenching the galaxy. SNe feedback will only start helping once the density has decreased enough to fall below $n_{H,t_c}=23~\rm cm^{-3}$. In the case of AGN feedback we still have efficient feedback all the way up to densities of $n_{H,t_c}=750~\rm cm^{-3}$. This means that in the high density region only AGN can help quench the galaxy. This basically means that the temperature to which we need to heat the gas in the center in order to quench the galaxy efficient is dependent on the density in the center. Besides getting high temperatures due to feedback it is also possible that gas gets shock heated due to other gas that was heated of energy diffusion heats neighbouring gas particles, this means that it is not necessary to heat all the gas to the injection temperature but an average high temperature will be enough, for example at densities of $n_{H}=130~\rm cm^{-3}$ a average temperature of $10^8 \rm K$ will be enough to heat the gas. This means that the e-folding time scale of AGN feedback basically depends on the exact density. 
\end{comment}


\section{Sketches}
In Fig. \ref{fig:cooling-dyn-ratio} we can see the $t_{\rm cool}/t_{\rm dyn}$-ratio as a function of time for different radii together with the SFH, total cold gas and BHAR. 



In Fig. \ref{fig:cooling-time} we show the SFH of the fiducial simulation and compare it with the cooling time at different radii and different times, we can see that when there is a start of an episode of star formation or when the star formation is still high that the cooling time is relatively short, while when the star formation starts to decrease the gas gets a longer cooling time that is several Gyrs. In Fig. \ref{fig:cooling-dyn-ratio} we can see the  $t_{\rm cool}/t_{\rm dyn}$-ratio as a function of time. Here we can see that the gas initially has a low $t_{\rm cool}/t_{\rm dyn}$-ratio which coincide with an increase in SFH while at large ratios above 10, we see that the the SFH is decreasing rapidly. This basically means that we seem to have a regulated loop between the SFH, gas mass, AGN accretion rate and the $t_{\rm cool}/t_{\rm dyn}$-ratio. 



\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/evolution/Xray_profile_2D.png}
    \caption{SFH of the $10^{13}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/evolution/Xray_profile_2D.png}
    \caption{SFH of the $10^{13}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}
\end{comment}



In Fig. \ref{fig:different-curves} we can see the different curves for the cold gas reservoir for gas below a temperature of $10^5~\rm K$, the SFH and the BHAR. It seems that the cold gas predicts the value for the SFH very well, this means that we can assume in general that the SFH is directly given by the cold gas reservoir available in our simulation, which implies that:
\begin{align}
    \rm SFH(t) = 1 \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right).
\end{align}
Looking more closely at Fig. \ref{fig:different-curves}, it also seems that the BHAR seems to follow on average on timescales of around 50 Myr the cold gas mass quite closely, it however seems that the BHAR is delayed, but for here we assume they are directly related to understand the physics. This means that the accretion rate is given by:
\begin{align}
    \rm BHAR(t) &= \epsilon_{\rm gas-BHAR} \rm M_\odot \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 \rm M_\odot} \right). 
\end{align}
In which $\epsilon_{\rm gas-BHAR}$ is a constant close to $0.01$, but in the case of the BHAR, this constant seems to be time dependent, but for now we assume it is exactly $0.01$. 

Given that the amount of cold gas is important in setting both the SFH and the BHAR we look at how the cold gas mass changes as a function of time:
\begin{align}
    \frac{\rm d M_{\rm cold gas}}{\rm d t} &= -R_{\rm AGN} - R_{\rm SNII} - R_{\rm SNIa} + R_{\rm cooling}. \label{eq:rates}
\end{align}
in which $R_{\rm i}$, $i=AGN, SNII, SNIa$ are the mass heating rates that are produced by AGN, SNII and SNIa feedback. $R_{\rm cooling}$ is the mass cooling rate, the amount of mass that cools down per time scale. In the case that we have no cooling flow we can calculate the e-folding time in which the cold gas mass is decreased by a factor of $e^{-1}$, in the case of only taking into account the AGN, we obtain an AGN mass heating rate of:
\begin{align}
    R_{\rm AGN} &= \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm AGN}} \epsilon_f \epsilon_r {\rm BHAR}(t) c^2, \\
    &= \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm AGN}} \epsilon_f \epsilon_r c^2 \epsilon_{\rm gas-BHAR} \rm yr^{-1} \left( \frac{M_{\rm cold gas}}{10^9 } \right).
\end{align}
If we fill this in Eq. (\ref{eq:rates}), we obtain a e-folding time for the AGN feedback off:
\begin{align}
    t_{\rm AGN} &= \frac{k_B \Delta T_{\rm AGN} \cdot 10^9}{(\gamma -1)\mu m_H \epsilon_f \epsilon_r \epsilon_{\rm gas-BHAR} c^2} \rm yr, \\
    &= 440 ~\rm Myr.
\end{align}
In a similar approach the mass heating rate for the SNIIs can be calculated as:
\begin{align}
    R_{\rm SNII} &=  \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm SNII}} SFR \eta_{SNII} E_{SNII}, \\
    &=  \frac{(\gamma - 1) \mu m_H}{k_B \Delta T_{\rm SNII}} \frac{M_{\rm cold gas}}{10^9} \eta_{SNII} E_{SNII} \rm yr^{-1}.
\end{align}
Meaning the e-folding time for SNII is:
\begin{align}
    t_{\rm SNII} &= \frac{k_B \Delta T_{\rm SNII} \cdot 10^9 \rm yr}{(\gamma -1)\mu m_H \eta_{SNII} E_{SNII}}.
\end{align}
In which $\eta_{SNII}$ is the fraction of stars that produce a SNII, for stars in the range of 8-100 $M_\odot$, this gives $\eta_{SNII}=1.736 \times 10^{-2} \rm M_\odot^{-1}$.
In the case of a heating temperature of $10^{7.5}~\text{K}$, this reduces to $660~\rm Myr$ and for a heating temperature of $10^{8.5}~\rm K$ reduces to $6.6 \rm Gyr$.

The rate of the SNIa however is constant and does not depend directly on the cold gas reservoir but depends on all the old stars that are available in the simulation. This means that the SNIa rate is approximately constant over the whole evolution of the simulation and is given by:
\begin{align}
    R_{\rm SNIa} &= \frac{(\gamma - 1) \mu m_H}{k_B \Delta T} \frac{M_\star \eta_{SNIa} E_{SNIa}}{t_H},
\end{align}
In which $\epsilon_{SNIa}$ is given by $\eta_{SNIa}=4 \times 10^{-3} \rm M_\odot^{-1}$.

To understand a bit more we can  write out de expression in Eq. \ref{eq:rates} to calculate how the system will behave:
\begin{align}
    \frac{\rm d M_{cold gas}}{\rm d t} &= -\left( \frac{1}{t_{\rm AGN}} + \frac{1}{t_{\rm SNII}} \right) M_{\rm cold gas} - R_{\rm SNIa} + R_{\rm cooling} (t),\\
    &= - \frac{M_{\rm cold gas}}{t_{\rm FB}} - R_{\rm SNIa} + R_{\rm cooling} (t),
\end{align}
This means that the solution for this equation will be given by:
\begin{align}
    M_{\rm cold gas}(t) &= M_0 -R_{\rm SNIa} t + e^{-\frac{t}{t_{\rm FB}}} \int R_{\rm cooling} (t') e^{\frac{t'}{t_{\rm FB}}} \rm d t'
\end{align}


\begin{comment}
\begin{align}
    M_{\rm cold gas}(t) &= M_0 -R_{\rm SNIa} t_{\rm FB} + e^{-\frac{t}{t_{\rm FB}}} \int R_{\rm cooling} (t') e^{\frac{t'}{t_{\rm FB}}} \rm d t'
\end{align}
We can see in this expression that the total amount of cold gas in the galaxy depends mainly on the cooling rate, to better understand the exact behaviour we can fill in a dummy function to see how the behaviour would depend on the the period and the amplitude of a sine wave:
\begin{align}
    R_{\rm cooling} (t) &= M_{inf.} \left( \sin \left(\frac{2\pi t}{P}\right) + 1 \right). 
\end{align}
Which will results in a total cold gas as a function of time given by:
\begin{align}
    M_{\rm cold gas}(t) =& M_0 + (M_{inf.}-R_{\rm SNIa}) t_{\rm FB} +\\ &M_{inf.} P t_{FB} \frac{P \sin\left( \frac{2\pi t}{P} \right) + 2\pi t_{FB} \cos\left( \frac{2\pi t}{P} \right) }{P^2 + (2\pi t_{FB})^2}, \\
    =& M_0 + (M_{inf.}-R_{\rm SNIa}) t_{\rm FB} + \\
    & M_{inf.} P t_{FB} \frac{P \sin\left( \frac{2\pi t}{P} \right) + 2\pi t_{FB} \sin\left( \frac{2\pi t}{P} - \frac{\pi}{2} \right) }{P^2 + (2\pi t_{FB})^2},
\end{align}


At which density do we get overcooling of feedback?
The overcooling of feedback is given by Eq. (18) of \citet{dalla-vecchia2012}:
\begin{align}
    n_{H,t_c} &= 23~\rm cm^{-3} \left( \frac{T}{10^{7.5}\rm K} \right)^{3/2} \left( \frac{\langle m \rangle}{10^5 \rm M_\odot} \right)^{-1/2}.
\end{align}
This means that for SNe feedback we will already have a problem of overcooling at a density of $n_{H,t_c}=23~\rm cm^{-3}$, this implies that when we have a high density in the galaxy, SNe feedback will not help in quenching the galaxy. SNe feedback will only start helping once the density has decreased enough to fall below $n_{H,t_c}=23~\rm cm^{-3}$. In the case of AGN feedback we still have efficient feedback all the way up to densities of $n_{H,t_c}=750~\rm cm^{-3}$. This means that in the high density region only AGN can help quench the galaxy. This basically means that the temperature to which we need to heat the gas in the center in order to quench the galaxy efficient is dependent on the density in the center. 
\end{comment}



\begin{comment}
\begin{figure}
	\includegraphics[width=\columnwidth]{./images/metallicity_M13_SFR_pure.png}
    \caption{SFH of the $10^{13}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/metallicity_M14_SFR_pure.png}
    \caption{SFH of the $10^{14}~\text{M}_\odot$ halo with different initial metallicities}
    \label{fig:coupling:BHARandSFR}
\end{figure}
\end{comment}

%\subsection{The runs}
%\input{runs.tex}

\subsection{Which channel dominates feedback?}

\subsection{Time scales}
\input{timescales.tex}


\begin{comment}
% Example figure
\begin{figure}
	% To include a figure from a file named example.*
	% Allowable file formats are eps or ps if compiling using latex
	% or pdf, png, jpg if compiling using pdflatex
	\includegraphics[width=\columnwidth]{example}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:example_figure}
\end{figure}

% Example table
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:example_table}
	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		A & B & C & D\\
		\hline
		1 & 2 & 3 & 4\\
		2 & 4 & 6 & 8\\
		3 & 5 & 7 & 9\\
		\hline
	\end{tabular}
\end{table}
\end{comment}

==> runs.tex <==
\subsection{Fiducial run}

\begin{itemize}
    \item We can see in \ref{fig:fid:power-spectrum} that the BHAR accretion rate seems to have a flat power spectrum, this means that the value of the BHAR is mostly random and does not have a significant behaviour in time. This mainly implies that when the BHAR is very high or lower is random. 
    \item It seems that both the SFR and the log of the BHAR behave following pink noise in which the slope of the power spectrum is close to $-1$, this means that the energy of fluctuations is independent of the time in which you look.
    \item If we further look into the curve for the log of the BHAR in Fig. \ref{fig:fid:power-spectrum} we see that on short frequencies the power spectrum is close to $-1$, but at frequencies around $log \nu = -1.5$ there is a peak, this indicates that the behaviour of the BHAR is influenced by a timescale that is around $T=30~\rm Myr$. If we further look at this power spectrum we see that around $\log \nu = -0.8$ the power spectrum still behaves around pink noise. If we go to frequencies of around $\nu = 10^{-0.5} ~\rm Myr^{-1}$ or timescales of $T\sim 3 ~\rm Myr$ we see that the power spectrum becomes almost flat. Meaning the exact value of BHARs is almost white noise while, at smaller times we see that at times off around $T\sim 0.25 \rm Myr$ the power drops again. 
    \item In Fig. \ref{fig:fid:correlation} we show the correlation between the value of the SFR and the BHAR. We can see that when we have a BHAR that is high we expect that the SFR will be anti-correlated and therefore lower after around $300~\rm Myr$. In the case of having a high SFR it seems that the BHAR will than also be high after a while because the SFR correlated with the BHAR.
\end{itemize}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/fid/fid_M14_FFT_summary_binned.png}
    \caption{Power spectrum of the SFR, log SFR, BHAR and log BHAR.}
    \label{fig:fid:power-spectrum}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/fid/fid_M14_Correlation_coefficient.png}
    \caption{Correlation between log SFR and log BHAR.}
    \label{fig:fid:correlation}
\end{figure}

\subsection{The coupling coefficient}

\begin{itemize}
    \item Larger coupling coefficient for the AGN leads to smaller accretion rates on average see Fig. \ref{fig:coupling:BHARandSFR} and \ref{fig:coupling:histogram}, the SFHs seem to be similar, but there seems to a trend that larger coupling coefficients have larger periods between periods of non-quenched and quenched.
    \item When the BHAR is high, this has a delayed negative correlation with the SFR, while if the SFR is high this causes the BHAR to increase in the future. The size of the effect seems to be similar for a coupling coefficient of $0.1$ and $0.01$ and smaller for $1.0$. Furthermore the exact delay seems to be similar between $1.0$ and $0.1$, to be around $350~\rm Myr$ while the delay for the small coupling coefficient of $0.01$ seems to be off the order of around $800~\rm Myr$.
\end{itemize}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/coupling/coupling_SFR_BHAR_25Myr.png}
    \caption{Top panel: Star formation history smoothed over 25 Myr, bottom pannel: BHAR smoothed over 25 Myr.}
    \label{fig:coupling:BHARandSFR}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/coupling/coupling_histogram_BHAR.png}
    \caption{Cumulative histogram of the BHARs}
    \label{fig:coupling:histogram}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{./images/coupling/coupling_SFR_BHAR_correlation.png}
    \caption{Pearson correlation coefficient for a given delay of the BHAR with respect to the SFR.}
    \label{fig:coupling:correlation}
\end{figure}

\subsection{Krumholz vs Bondi-Hoyle}

\begin{itemize}
    \item Bondi-Hoyle has a higher SFR and lower accretion rate than Krumholz, see Fig. \ref{fig:krumBH:BHARandSFR} and \ref{fig:krumBH:hist}.
    \item The power spectrum does not show the same peak at $30~\rm Myr$, instead it seems that at high frequencies the power is much higher and at low frequencies the behaviour is more flat, see Fig. \ref{fig:krumBH:hist}. 
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/krumBH/KrumBH_M14_log_SFR_and_log_BHAR_smoothing25Myr.png}
    \caption{Top panel: Star formation history smoothed over 25 Myr, bottom pannel: BHAR smoothed over 25 Myr.}
    \label{fig:krumBH:BHARandSFR}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/krumBH/KrumBH_M14_histogram_accretion_cumulative.png}
    \caption{Histogram of the accretion rate}
    \label{fig:krumBH:hist}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/krumBH/KrumBH_M14_FFT_log_BHAR_binned.png}
    \caption{}
    \label{fig:krumBH:power-spectrum}
\end{figure}

\subsection{Isotropic vs Minimum distance}
\begin{itemize}
    \item Minimum distance feedback is more smooth in the accretion rate than the isotropic feedback, see Fig. \ref{fig:injection:BHARandSFR}
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/injection/injection_M14_SFR_and_BHAR_smoothing25Myr.png}
    \caption{Top panel: Star formation history smoothed over 25 Myr, bottom pannel: BHAR smoothed over 25 Myr.}
    \label{fig:injection:BHARandSFR}
\end{figure}

\begin{enumerate}
    \item Nngb variations
    \item Heating temperature: higher heating temperature quenching takes longer but stay also quenched longer. Also higher accretion rates seem to have 
    \item Bondi-Hoyle and boost: Boost means lower SFR, SFR plot. When
you boost the accretion rate the accretion rate behave more stable on
small scales as compared to without boost in which case it fluctuates
a lot
    \item Krumholz and boost: very similar to the Bondi-Hoyle part, only here
both models quench reasonable.
    \item higher coupling constant means you stay quenched longer after SF
and SF rises less. Ofcourse also the common thing of higher coupling coefficient means
lower accretion rate to reach the same. For this part it is also in-
\end{enumerate}


==> timescales.tex <==
\subsubsection{gas timescales}

The gas has several different time scales, the shortest time scale in general is the flow time scale that is the time that it takes gas to reach the centre with their current velocity:
\begin{equation}
 t_\text{flow} = \frac{r}{|\vec{v}|}.
\end{equation}
In which $r$ is the distance to the centre of the cluster/galaxy and $\vec{v}$ is the velocity vector. After that we have that the cooling time is short and given by:
\begin{equation}
 t_\text{cool} = \frac{\frac{3}{2} n k_B T}{|\Lambda_\text{net}|}.
\end{equation}
In which $\Lambda_\text{net}$ is the netto cooling rate, $T$ the gas temperature and $n$ the number density. The dynamical time is given by:
\begin{equation}
 t_\text{dyn} = \frac{\sqrt{2} r}{\sqrt{G M_\text{encl}/r}}.
\end{equation}
In which $M_\text{encl}$ is the enclosed mass at the radius $r$. and the free fall time is given by:
\begin{align}
 t_\text{ff} &= \sqrt{\frac{3\pi }{32 G \rho}}, \\
 &= 145~{\rm Myr} \left( \frac{n_H}{0.1~\rm cm^{-3}} \right)^{-1/2}. 
\end{align}
In which $\rho$ is the gas density.

In the runs the different timescales seem to reach 1 Gyr and 100 Myr at radii of see Tab \ref{tab:gas-time}.
% Example table
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:gas-time}
    \begin{tabular}{l|c|c}
         Time scale & 1 Gyr & 100 Myr \\ \hline  
         Flow time & 10 kpc & 3 kpc \\
         cooling time & 30 kpc & 3 kpc \\
         Dynamical time & 200 kpc & 30 kpc \\
         Free fall time & 100 kpc & - \\
    \end{tabular}
\end{table}


\subsubsection{Time scales close to the black hole}
For the BH there are several time scales, the first is the Salpeter time scale which is the e folding time when the BH accretes at the Eddington limit, this timescale is given by:
\begin{align}
 t_{\rm{Salpeter}} = \frac{\epsilon_r \sigma_T c}{4 \pi G m_p} = 45 \text{Myr}. 
\end{align}
In the simulations that I did we do only occasionally for a short moment in time accrete close the to Eddington limit, so I think this timescale is not of significant importance for the runs. A short time scale that can be off interest is the time between different AGN heating events is given by:
\begin{align}
 \epsilon_f \epsilon_r \langle \dot{M}_\text{BH} \rangle t_\text{AGN heating} c^2 &= \frac{k_B \Delta T}{\gamma -1} \frac{m_{gas}}{\mu m_H} N_\text{target}, 
\end{align}
Which in physical values is given by:
\begin{align}
 t_\text{AGN heating} &= 70~\text{kyr} \left(\frac{\Delta T}{10^{8.5}~\text{K}}\right) \left( \frac{\langle \dot{M}_\text{BH} \rangle}{10^{-2.5~\text{M}_\odot / \text{yr}}} \right)^{-1} \left( N_\text{target} \right).
\end{align}
In terms of the eddington ratio:
\begin{align}
 t_\text{AGN heating} &= 10~\text{kyr} \left(\frac{\Delta T}{10^{8.5}~\text{K}}\right) \left( \frac{R_{\rm Edd}}{0.01} \right)^{-1} \left( \frac{m_{\rm BH}}{10^8 \rm M_\odot} \right)^{-1} \left( N_\text{target} \right).
\end{align}

We can also write it explicitly in terms of the density and temperature around the black hole, than we obtain:
\begin{align}
    t_\text{AGN heating} &= 1.5~\text{kyr} \left(\frac{\Delta T}{10^{8.5}~\text{K}}\right) \left( \frac{M_{BH}}{10^8~\rm M_\odot} \right)^{-2} \left( \frac{n_H}{0.1 \rm cm^{-3}} \right)^{-1} \\
    &~~ \left( \frac{T}{10^5~\rm K} \right)^{3/2} \left( N_\text{target} \right).
\end{align}

For BHs there are also other time scales of interest, small scale times are not resolved in our simulation. The timescale closest related to the BH is the Bondi-Hoyle time scale, given by:
\begin{align}
 t_\text{Bondi} = \frac{r_B}{c_s} = 420 \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-3} ~\text{Myr}. 
\end{align}
Similar we can define a Bondi-Hoyle radius as:
\begin{align}
    r_{\rm Bondi} &= \frac{GM}{c_s^2} = 3.0 ~\rm kpc \left( \frac{M_{\rm BH}}{10^8 \rm M_\odot} \right) \left( \frac{T}{10^4 \rm K} \right)^{-1}. 
\end{align}

In the case that the gas around the BH has supersonic velocities we need to use an other equation given by:
\begin{align}
 t_\text{Krumholz} = \frac{r_B}{(1+M_0^2) M_0 c_s} = 420 \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{(1+M_0^2) M_0 c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-3} ~\text{Myr}. 
\end{align}
This also implies that the Bondi-Hoyle radius is modified to:
\begin{align}
    r_{\rm Krumholz} &= \frac{GM}{(1 + M_0^2) c_s^2} = \frac{3.0 ~\rm kpc}{1 + M_0^2} \left( \frac{M_{\rm BH}}{10^8 \rm M_\odot} \right) \left( \frac{T}{10^4 \rm K} \right)^{-1}. 
\end{align}
This means that when there is turbulence the Bondi-Hoyle radius is decreased compared to the approach in which we do not take into account turbulence.

In the case of Gaspari type of feedback we have that we want to accrete enough mass to heat 1 particle the moment we a particle gets in our inner radius for which we accrete. This means that in order to heat 1 particle we need to nibble a mass of:
\begin{align}
    \epsilon_f \epsilon_r \Delta m_{\rm acc} c^2 &= \frac{k_B \Delta T}{\gamma -1} \frac{m_{gas}}{\mu m_H},
\end{align}
this reduces to:
\begin{align}
    \Delta m_{\rm acc} &= \frac{k_B T}{\gamma - 1} \frac{m_{\rm gas}}{\mu m_H \epsilon_f \epsilon_r c^2}, \\
    &= 726~\rm{M}_\odot \left( \frac{\Delta T}{10^{8.5}K} \right) \left( \frac{m_{\rm gas}}{10^{5} ~\rm M_\odot } \right) \left( \frac{\mu}{0.6} \right)^{-1}.
\end{align}

AGN:
\citet{rosas-guevara2015}, \citet{schaye2015}

The Eddington accretion rate is given by:
\begin{align}
    \dot{m}_{\rm Edd} &= \frac{4 \pi G m_{\rm BH} m_{\rm p}}{\epsilon_r \sigma_T c}, \\
    &= 2.218 ~\rm M_\odot \rm yr^{-1} \left( \frac{m_{\rm BH}}{10^8 ~\rm M_\odot} \right).
\end{align}

Bondi-Hoyle accretion\citep{bondi1944}:
\begin{align}
    \dot{m}_{\rm Bondi} &= \frac{4 \pi G^2 m_{\rm BH}^2 \rho}{(c_s^2 +v^2)^{3/2}}.
\end{align}

\begin{align}
    \dot{m}_{\rm BH} = (1-\epsilon_r) \dot{m}_{\rm accr}. 
\end{align}


\subsubsection{Time scales related to the disk around the BH}
The sound crossing time for the disk:
\begin{align}
 t_\text{cross} = 65 \text{Myr} \left( \frac{\mu}{0.6}\right )^{1/2} \left(\frac{T}{10^4 K}\right)^{-1/2} \left(\frac{d}{1 kpc}\right).
\end{align}
Disk consumption time scale is given by:
\begin{align}
 t_{\rm SFR} &= \frac{M_{\rm gas}}{SFR}, \\
 &= 10~{\rm Myr} \left( \frac{M_{\rm gas}}{10^8~\rm M_\odot} \right) \left( \frac{SFR}{10~ \rm M_\odot ~\rm yr^{-1}} \right)^{-1}.
\end{align}
\subsubsection{Time scales related to stars}
SNII time scale, the time scale within all SNII go off:
\begin{align}
    t_{\rm SNII} &= 30~\rm Myr.
\end{align}

\subsubsection{Angular momentum limiter related time scales}

The viscous Yetli time scale:
\begin{align}
 t_\text{visc} &= 420~ C_\text{visc} \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{V_\phi}{10~\text{km}~\text{s}^{-1}} \right)^3 \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-6} ~\text{Myr}, \\
 &= 2.6\cdot 10^6 \left(\frac{C_\text{visc}}{2\pi \cdot 10^3}\right) \left( \frac{M_\text{BH}}{10^8~\text{M}_\odot} \right) \left( \frac{V_\phi}{10~\text{km}~\text{s}^{-1}} \right)^3 \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-6} ~\text{Myr}.
\end{align}

A vorticity time scale for the Krumholz model:
\begin{align}
 t_\text{vorticity} &= \frac{1}{|\nabla \times \vec{v}|} = \frac{1}{\omega} = \frac{r}{\tilde{\omega} M_0 c_s}, \\
  &= 19.6 ~\text{Myr} \left( \frac{r}{10~\text{kpc}} \right) \left( \frac{c_s}{10~\text{km}~\text{s}^{-1}} \right)^{-1}\left( \frac{\tilde{\omega}}{10.} \right)^{-1}.
\end{align}
This has a corresponding length scale given by:
\begin{align}
    r_{\rm vorticity} =\frac{M_0 c_s}{|\nabla \times \vec{v}|}  &= 1.0~ \rm{kpc}\left( \frac{M_0}{5} \right) \left( \frac{r}{10~\text{kpc}} \right) \left( \frac{\tilde{\omega}}{10.} \right)^{-1}.
\end{align}

\subsubsection{When is gas gravitational bound?}
The total energy of the gas-BH system is given by:
\begin{align}
    E_{tot} &= E_{grav} + E_{kin} + E_{th}.
\end{align}
Filling in the equations we obtain:
\begin{align}
    E_{tot} &= - \frac{G M_{BH} m_{gas}}{r} + \frac{1}{2} m_{gas} v^2 + \frac{k_B T}{(\gamma - 1)} \frac{m_{gas}}{\mu m_H}.
\end{align}
In general gas is bound when we have $E_{tot} < 0$, which means that we obtain:
\begin{align}
    \sqrt{\frac{G M_{BH}}{r}} > \sqrt{\frac{k_B T}{(\gamma -1)\mu m_H} + \frac{1}{2}v^2}.
\end{align}
Which can be expressed as:
\begin{align}
    165~\rm km \rm s^{-1} \left( \frac{r}{100~\rm pc} \right)^{-1/2} \left( \frac{M_{BH}}{10^{8.8}~\rm M_\odot} \right)^{1/2} > \sqrt{95 ~\rm km^2 \rm s^{-2} \left(\frac{T}{10^4~\rm K} \right) + \frac{1}{2} v^2}. 
\end{align}
Which means that if we ignore the thermal term, we obtain:
\begin{align}
    v_{gas} < 230~\rm km \rm s^{-1} \left( \frac{r}{100~\rm pc} \right)^{-1/2} \left( \frac{M_{BH}}{10^{8.8}~\rm M_\odot} \right)^{1/2}
\end{align}
and in the case of thermal dominated we obtain:
\begin{align}
    T < \frac{G M_{BH} (\gamma -1) \mu m_H}{r k_B} = 2.85 \times 10^6 ~\rm K \left( \frac{M_{BH}}{10^{8.8}~\rm M_\odot} \right) \left( \frac{r}{100~\rm pc} \right)^{-1}.
\end{align}

What radius is the enclosed stellar mass smaller than the BH mass?
\begin{align}
    M_{\rm BH} > M_{\star} \frac{r^2}{(r_{\star}^2 + r^2)}.
\end{align}
This results in:
\begin{align}
    \left( M_{\star} - M_{\rm BH} \right) r^2 - 2 r r_\star M_{\rm BH} - M_{\rm BH} r_{\star}^2 < 0.
\end{align}
Which means that we obtain:
\begin{align}
    r < 2 r_{\star} \left( \frac{M_{\rm BH} \pm \sqrt{M_{\rm BH} M_{\star} }}{M_{\star} - M_{\rm BH}} \right).
\end{align}
